Dynamic Hypergames for Synthesis of Deceptive Strategies with Temporal Logic Objectives

In this paper, we study the use of deception for strategic planning in adversarial environments. We model the interaction between the agent (player 1) and the adversary (player 2) as a two-player concurrent game in which the adversary has incomplete information about the agent's task specification in temporal logic. During the online interaction, the adversary can infer the agent's intention from observations and adapt its strategy so as to prevent the agent from satisfying the task. To plan against such an adaptive opponent, the agent must leverage its knowledge about the adversary's incomplete information to influence the behavior of the opponent, and thereby being deceptive. To synthesize a deceptive strategy, we introduce a class of hypergame models that capture the interaction between the agent and its adversary given asymmetric, incomplete information. A hypergame is a hierarchy of games, perceived differently by the agent and its adversary. We develop the solution concept of this class of hypergames and show that the subjectively rationalizable strategy for the agent is deceptive and maximizes the probability of satisfying the task in temporal logic. This deceptive strategy is obtained by modeling the opponent evolving perception of the interaction and integrating the opponent model into proactive planning. Following the deceptive strategy, the agent chooses actions to influence the game history as well as to manipulate the adversary's perception so that it takes actions that benefit the goal of the agent. We demonstrate the correctness of our deceptive planning algorithm using robot motion planning examples with temporal logic objectives and design a detection mechanism to notify the agent of potential errors in modeling of the adversary's behavior.

==> Archived/Archived/Problem_formulation.tex <==
We consider the problem of computing optimal strategies for a controllable player, Alice (P1), in a game where P1 plays against an adversarial uncontrollable player, Bob (P2), who has partial information about P1's objective in the game. We assume that (a) P1 and P2 are bounded-rational players, (b) P1 knows what P2 believes to be her objective at the beginning of the game, (c) P1 knows how P2 updates his belief after observing the game play, and (d) P1 and P2 have complete observability of the game. Under assumptions (b) and (c), we note that the above game is a two-player zero-sum game under information asymmetry \cite{}. 


We, now, describe the formalism used to characterize the interaction between P1 and P2. The game between P1 and P2 is said to be played over a game arena (hereby referred to as simply, arena). 


{\definition[Arena] An arena is a digraph, $G = \langle V, E \rangle$. The set $V$ denotes the set of vertices (interchangeably also called as ``states") of arena and $E \subseteq V \times V$ denotes the edges of arena. 
}

An arena represents: (a) a superset all the states that any player can take, and (b) a superset of all the edges that are accessible to any player, during the game. It is noted that, some states and/or edges in the arena may not be accessible to some players.


Every player in the game is defined by its characteristics. These characteristics define what action capabilities does the player have, what sensing modalities does the player have, or how the player reasons about thinks and reasons about his environment and other players. 


{\definition[Player] Let $G = \langle V, E \rangle$ be an arena. Then, a player in an arena, $G$, is defined as a following tuple, 
\[
    P = \langle G, A, \alpha, AP, L, \varphi, \mu, \eta, B \rangle 
\]
where every element (except $G$) is said to be a characteristic of the player and is defined as, 
\begin{itemize}
    \item $A$ is a set of actions that the player can perform.
    
    \item $\alpha \subseteq E \times A$ represents the accessibility relation for the player. Given an edge $(u, v) \in E$ and an action $a \in A$, we abuse the notation and write $(u, a, v) \in \alpha$ to denote that the player reaches the state $v$ by performing an action $a$ at state $u$. 
    
    \item $AP$ is the set of atomic propositions, also called the alphabet of the player. 
    
    \item $L: V \rightarrow 2^{AP}$ is the labeling function that assigns to every vertex $v \in V$, the largest subset of alphabet containing atomic propositions that are true at the given vertex.
    
    \item $\varphi \in \mathsf{LTL}$ is an LTL specification that defines the objective of the player. The set $\mathsf{LTL}$ is the set of all LTL formulas that can be written using the alphabet $AP$. Note that $\mathsf{LTL}$ is, in general, countably infinite set. 
    
    % \item $K$ represents a finite set of information states of the player.
    
    \item $\mu$ is called the misperception function of the player. The misperception of a player is how a player perceives other players and their characteristics in the game. For instance, to capture the misperception of P2 about P1's objective, we write $\mu(\varphi) = \psi$ where $\varphi$ and $\psi$ are LTL formulas. Note that, the misperception of a player, say P1, about another player, say P2, depends on the information available with P1 about the P2. 
    
    \item $\eta$ is called as an inference mechanism. An inference mechanism represents how the player updates the misperception function $\mu$, given the game play (see Def.~\ref{} below). 
    
    \item $B$ is a model of mind. For instance, a bounded-rational player's mind can be modeled using k-level theory \cite{}, Cognitive Hierarchy model \cite{}, \etc, whereas a rational player may be modeled by defining a solver used by the player, such as  Nash equilibrium solver or Zielonka solver \etc, to solve for equilibrium.  
\end{itemize}
}


\begin{remark}
The accessibility relation, $\alpha$, represents a subset of edges $E \times A$ accessible to the player, \ie enabled for the player. When for a every pair $(u, a)$, there exists a unique $v \in V$ such that $(u, a, v) \in \alpha$, we say that $\alpha$ is a deterministic. We usually denote a deterministic accessibility relation as $\alpha: V \times A \rightarrow V$. Otherwise, $\alpha$ is said to be non-deterministic. To represent a stochastic accessibility relation, we associate a probability value $p \in [0, 1]$ with every edge, thus writing an edge in $\alpha$ as $(u, a, v, p)$.
\end{remark}


A game consists of two players, $P_1$ and $P_2$, each defined using their characteristics $X_i$ where $i \in \{1, 2\}$ and $X$ can take values from the set $\{A, \alpha, AP, L, \varphi, \mu, \eta, B\}$. Both players, P1 and P2, construct their own model of game using the arena $G$ and a model of their opponent $P_j^i = \mu_i(P_j)$ for $i \neq j$. The player computes his/her strategy by solving the constructed game. 


Let us set up the player characteristics, for this article, to represent a zero-sum game under information asymmetry. 

\begin{itemize}
    \item P1: has Complete Information
    \begin{itemize}
        \item $A_1, \alpha_1$: are the set of actions and accessibility relation for P1. 
        \item $AP, L$: are the alphabet and labeling function common to both, P1 and P2. 
        \item $\varphi_1$ is a \textit{Syntactically-Cosafe LTL} objective of P1. 
        \item $\mu = \cal{I}$, where $\cal{I}$ represents an identity function. This represents that P1 has no misperception about P2. 
        \item \textcolor{red}{$\eta$ is not necessary, because P1 has complete information and complete observation. However, it seems we are trying to infer $B$ of P2 to estimate the level of P2's thinking! This would mean we have \textit{a general game with incomplete information, not just asymmetry, right?}}
        \item $B$ is a level-$k$ Cognitive Hierarchy (CH) solver. 
    \end{itemize}
    
    \item P2: does not know P1's true objective.
    \begin{itemize}
        \item $A_2, \alpha_2$: are the set of actions and accessibility relation for P2. 
        \item $AP, L$: are the alphabet and labeling function common to both, P1 and P2. 
        \item $\varphi_2$ is the objective of P2. Ideally, as we want to define a zero-sum game, $\varphi_2 = \neg \varphi_1$. However, under information asymmetry, P2 does not know P1's true objective. Let $\psi$ be P2's misperception of P1's objective. Then, we write $\varphi_2 = \neg \psi$. We note that $\psi$ might change as the game evolves. 
        \item Given a finite game play $\rho$, the misperception function is given as follows 
            \begin{align*}
                \mu(X, \rho) = \begin{cases}
                           \psi & \text{if } X = \varphi_1 \\
                           {\cal I} &   \text{otherwise}
                         \end{cases}
            \end{align*}
        \item Given a finite game play $\rho$ of length $n$, the inference mechanism $\eta$ is a function that updates P2's misperception of P1' objective, given by $\psi_{n+1} = \eta(\psi_n, \rho)$
        \item $B$ is a CH-solver of level-$k'$ such that $k' < k$.
    \end{itemize}
\end{itemize}


Recall that each player constructs a game in his/her brain. This game is constructed in two steps: (a) by constructing a transition system to capture the dynamics of their interaction, and (b) by constructing an automaton that accepts the language of sc-LTL specification that represents their objective(s). As we want to synthesize strategy for P1, we will define the following terms from P1's perspective. 


\textbf{Step 1:} A transition system may be of two types; turn-based or concurrent. 

\begin{definition}[Turn-based Transition System]
Given P1's model, $P_1$, and P1's perception of P2, $P_2^1$, the transition system, as constructed by P1 in his own mind when the interaction is \textit{turn-based}, is given by 
    \begin{align}
        TS = \langle S, Act, T, AP, L \rangle
    \end{align}
where
    \begin{itemize}
        \item $S = V \times V \times \{1, 2\}$ is the set of states in the transition system. A state $(v_1, v_2, 1)$ represents that P1 is at state $v_1$ in arena, P2 is at state $v_2$ in arena and it is P1's turn to make a move. 
    
        \item $Act = A_1 \cup A_2$ where $A_1$ and $A_2$ are action sets of P1 and P2, respectively. 
        
        \item $T \subseteq S \times Act \times S$ is the accessibility relation in the transition system. $T$ is said to be \textit{deterministic}, if for every pair $(s \in S, a \in Act)$ there exists a unique $s' \in S$ such that $(s, a, s') \in T$. Otherwise, $T$ is said to be non-deterministic. A non-deterministic $T$ is said to be stochastic, when the edge relation satisfies $\sum\limits_{s' \text{ s.t. } (s, a, s') \in T} \mathbb{P}(s' \mid s, a) = 1.0$. 
        
        \item $AP$ is the alphabet of transition system. 
        
        \item $L: S \rightarrow 2^{AP}$ is the labeling function, that assigns to every state $s \in S$, the subset of atomic propositions from $AP$ that are true in the given state. The function is defined as $L(s) = L(v_1) \cup L_2(v_2)$. 
    \end{itemize}
\end{definition}


\begin{definition}[Concurrent Transition System]
Given P1's model, $P_1$, and P1's perception of P2, $P_2^1$, the transition system, as constructed by P1 in his own mind when the interaction is \textit{concurrent}, is given by 
    \begin{align}
        TS = \langle S, Act, T, AP, L \rangle
    \end{align}
where
    \begin{itemize}
        \item $S = V \times V$ is the set of states in the transition system. A state $(v_1, v_2, 1)$ represents that P1 is at state $v_1$ in arena, P2 is at state $v_2$ in arena and it is P1's turn to make a move. 
    
        \item $Act = A_1 \times A_2$ where $A_1$ and $A_2$ are action sets of P1 and P2, respectively. 
        
        \item $T \subseteq S \times Act \times S$ is the accessibility relation in the transition system. $T$ is said to be \textit{deterministic}, if for every pair $(s \in S, a \in Act)$ there exists a unique $s' \in S$ such that $(s, a, s') \in T$. Otherwise, $T$ is said to be non-deterministic. A non-deterministic $T$ is said to be stochastic, when the edge relation satisfies $\sum\limits_{s' \text{ s.t. } (s, a, s') \in T} \mathbb{P}(s' \mid s, a) = 1.0$. 
        
        \item $AP$ is the alphabet of transition system. 
        
        \item $L: S \rightarrow 2^{AP}$ is the labeling function, that assigns to every state $s \in S$, the subset of atomic propositions from $AP$ that are true in the given state. The function is defined as $L(s) = L(v_1) \cup L_2(v_2)$. 
    \end{itemize}
\end{definition}


\textbf{Step 2:} A deterministic finite automaton (DFA) is given by $A = \langle Q, \Sigma, \delta, q_0, F \rangle$. It is known result that, given a sc-LTL specification $\varphi$, there exists a DFA that accepts the same language as that of $\varphi$. 


Given a transition system and an automaton $A_1$ equivalent to his specification $\varphi_1$, P1 constructs a zero-sum game as follows


\begin{definition}[Game]
Let a turn-based (resp. concurrent) transition $TS = \langle S, Act, T, AP, L \rangle$ and an DFA $A = \langle Q, \Sigma, \delta, q_0, F \rangle$ be given. Then, a turn-based (resp. concurrent) game is defined as 
\[
    \game = \langle S \times Q, Act, \Delta, F \rangle
\]
where 
\begin{itemize}
    \item usual definitions
\end{itemize}
\end{definition}


The game as defined above is ignorant of model of the opponent, and assumes the opponent to be a perfect adversary; \ie an opponent with complete information and complete observation. However, under information asymmetry, P1 incorporates the model of opponent $P_2^1$, which accounts for P2's misperception, into his decision-making. This yields a hypergame, in contrast to a game. 


\begin{definition}[Hypergame]
Let $\game_1$ be a game constructed by P1 using his own model; $P_1$, and $\game_2$ be a game constructed by P2 using her model of herself; $P_2$. Then, a first-level hypergame is defined as
\[
    {\cal H}^1 = \langle \game_1, \game_2 \rangle
\]

When P1 uses his model of P2; $P_2^1$, to make his decision-making, we represent the interaction using a second-level hypergame,
\[
    {\cal H}^2 = \langle (\game_1, \game_2^1), \game_2 \rangle
\]
\end{definition}


\begin{remark}
In a second-level hypergame, P1 computes his strategy by solving a first-level hypergame. 
\end{remark}


\begin{remark}
As P1 has complete information, $\game_2^1 = \game_2$.
\end{remark}


It is easy to confuse between the levels of a CH-model and levels of a hypergame. We understand that CH-model (characteristic $B_1$ of P1 and $B_2$ of P2) represents how a player computes his/her strategy given the player structure $P_i$. Whereas, the levels of hypergame represent the awareness of a player about the other player's awareness of existing misperception. For instance, in a second-level hypergame (where P1 solves first-level hypergame), P1 will solve the game $\game_2$ using $B_2^1$ to estimate P2's response strategy given the player structure $P_2^1$. When using CH-model to model bounded-rationality, $B_2^1$ could compute strategy for a $k'$-level agent, for some $k' < k$ and $k$ being the level of CH-model solver $B_1$. 


We now formalize the problem as follows, 
\begin{problem}
Let $P_1$ and $P_2$ represent the player structures for two bounded-rational players P1 and P2 interacting over an arena $G$, with characteristics as described in above section. Then, synthesize an almost-sure winning strategy and an optimal response strategy in positive-winning for P1. 
\end{problem}




% We represent the objectives of players as a Syntactically-Cosafe Linear Temporal Logic (sc-LTL) specifications. At the beginning of the game, let $\varphi$ be the specification of P1, and $\psi$ be P2's misperception of P1's objective. Then, had P2 been a rational agent, P2 would have played a game to satisfy the negation of P1's objective, \textit{i.e.} P2 tries to satisfy $\neg \psi$. However, we assume the players to be bounded-rational and, hence, they cannot solve for equilibrium strategy. Nonetheless, when $\psi = \varphi$, we observe that the strategy synthesis problem reduces to conventional reactive synthesis. Therefore, we focus on the case where $\psi \neq \varphi$ at the beginning of the game. 


% We start by defining the notion of winning for P1 and P2 in the game. A \textit{play} of the game is an ordered sequence, $\rho = (s_0, a_0^1, a_0^2), (s_1, a_1^1, a_1^2), \ldots, $ where at every turn both players; P1 and P2, choose an action, which is independent of their opponent's choice of action at that turn. In other words, the game is a concurrent (\textit{a.k.a.} simultaneous) game. In such a game, we say P1 has won the game when $\rho \models \varphi$\footnote{Let $\mathsf{Occ}(\rho) = \{s \mid s \in \rho\}$ represent the set of states appearing in the play $\rho$. Then, we say $\rho \models \varphi$ when $\mathsf{Occ}(\rho) \cap F \neq \emptyset$.}, and P2 has won the game when $\rho \not\models \varphi$. Note that, we define winning based on ``true" objective of P1. Therefore, P2 does not win the game by satisfying $\neg\psi$, because $\psi$ is not the true objective of P1. 


% Given that P2 starts with a misperception $\psi$ of P1's objective, it is possible that P2 may infer P1's ``true" objective; $\varphi$, by observing P1's behavior in the game. To capture this capability of P2, we equip him with an inference mechanism, which is a function that maps P2's misperception at current turn $t$, say $\psi_{t}$, and a finite history of states; $h \in S^\ast$, to produce a new misperception $\psi_{t+1}$. Formally, we define an inference mechanism as follows,  


% \begin{definition}[Inference Mechanism]
% Let $G$ be a subset of $S$ and $\mathsf{LTL}$ be the set of all LTL formulas that can be defined over a finite set $AP$ of atomic propositions. An inference mechanism is a function $\eta: \mathsf{LTL} \times S^\ast \rightarrow \mathsf{LTL}$, which maps a current misperception $\psi_t$ of P2 and a finite history of states $h \in S^\ast$ to a return an updated misperception $\psi_{t+1}$ of P1's objective. 
% \end{definition}


% In this article, we restrict the scope of inference mechanism to inferring parameterized sc-LTL objectives. For example, given a set of states $G \subseteq S$, we may represent P2's misperceived objective of P1 as $\psi_t = \Diamond g_t$, where $g_t \in G$. In this case, the problem of inferring an LTL specification reduces to the problem of estimating the current sub-goal that P1 is pursuing from the set $G$. One approach for sub-goal inference is using \textit{change detection with adaptive sliding window}, described in Sect.~\ref{}. 


% The inference mechanism describes how P2 updates his knowledge, and thus the game he plays against P1. However, P2 is assumed to be a bounded rational. In this article, we use Cognitive Hierarchy (CH) model to represent bounded rationality of players, which is described in Sect.~\ref{}. Given the model of bounded rationality and an inference mechanism, we formalize the problem statement. 


% \begin{problem}
% Assume that P1 is a $k$-level thinker, according to CH model, and knows the inference mechanism $\eta$ by which P2 updates his misperception. Then, synthesize a deceptive strategy $\pi: S \rightarrow A_1$ for P1 that can deceive P2 by controlling his misperception, if necessary, to ensure that P1 will satisfy $\varphi$ with probability one.  
% \end{problem}



==> Archived/Archived/archieved_change_detection.tex <==

\newpage 

\begin{itemize}
    \item observations $y_{1,t}$
    \item hidden sequence of states: $z_{1,t}$ where $z_t$ is assumed to be the goal pursuit by agent at time $t$.
    \item the run length: $r_t$--that is a non- negative discrete quantity denoting the number of time steps elapsed at time t since the last change point occurred in the sequence. It holds that $r_t = 0$ at a change point.
\end{itemize}

The following prior is given:
\[
P(z_t|z_{t-1})
\]
however, the duration $P(d_t|z_t)$ is not given but to be detected.

objective: to compute 
\[
P(r_t,z_t |y_{1,t})
\]
in a online manner.

\begin{align*}
    \gamma_t  = & P(r_t,z_t ,y_{1,t})\\
     = & \sum_{r_{t-1}}\sum_{z_{t-1}}P(r_t,z_t, r_{t-1},z_{t-1}, y_{1,t})\\
    = &\sum_{r_{t-1}}\sum_{z_{t-1}} P(r_t,z_t| r_{t-1},z_{t-1}, y_{1,t}) P(r_{t-1}, z_{t-1}, y_{1,t}) \\
    = &\sum_{r_{t-1}}\sum_{z_{t-1}} P(r_t,z_t| r_{t-1},z_{t-1}, y_{1,t}) P(r_{t-1}, z_{t-1}, y_{1,t-1}, y_t) \\
    = &\sum_{r_{t-1}}\sum_{z_{t-1}} P(r_t,z_t| r_{t-1},z_{t-1}, y_{1,t}) P(y_t| r_{t-1}, z_{t-1}, y_{1,t-1})\cdot P(r_{t-1}, z_{t-1}, y_{1,t-1}) \\
     =  & \sum_{r_{t-1}}\sum_{z_{t-1}} 
     P(r_t,z_t| r_{t-1}, z_{t-1}, y_{1,{t}})P(y_t | r_{t-1}, z_{t-1}, y^{(r_{t-1})})\cdot P(r_{t-1},z_{t-1}, y_{1,t-1})\\
     =  & \sum_{r_{t-1}}\sum_{z_{t-1}} 
     P(r_t,z_t| r_{t-1}, z_{t-1}, y_{1,{t}})P(y_t | r_{t-1}, z_{t-1}, y^{(r_{t-1})})\cdot \textcolor{blue}{\gamma_{t-1}}.
\end{align*}
The calculation $ P(y_t| r_t,z_t, y^{r_t}) = P(y_t| z_t, y^{r_t}) $ can be obtained from the predictive model given goal $z_t$ and history $y^{r_t}$.

The question is how to calculate
\[
P(r_t,z_t| r_{t-1}, z_{t-1}, y_{1,{t}})
\]

in bayesian online change point detection, hazard function is introduced to define $P(r_t|r_{t-1})$. For example, geometric distribution.

This prior information is not easy to assume in our setting.

We use change detection to predict.
\[
P(r_t,z_t| r_{t-1}, z_{t-1}, y_{1,{t}})
= 1- {1}(\max_{j\in Z}B^j(z_{t-1}) > A)
\]

where $Z$ is the domain of $z_t$,  $B^{j}(z_{t-1})$ is CUmulative SUM statistic (CUSUM)
defined by 
\[
B^{j}(z_{t-1}) =  \max_{1 \le k \le m}\frac{P_j(y_{k,m}^{(r_{t-1})})}{P_0(y_{k, m}^{(r_{t-1})})},
\]
where $m$ is the window size that depends on the false alarm constraints, $P_j$ is calculated from the hypothesis $j$ (an alternative mode), $P_0$ is calculated from the hypothesis $z_{t-1}$ (the current mode, assuming no change). For step $k=1,2,\ldots m $, we compare each step and see if significant change has been detected given two comparison. When at least one alternative $j$ and a step $k$ yields large Bayes factor, then a change is detected and $r_t$ is reset to zero. Otherwise, $r_t= r_{t+1}+ 1$.

In short, the CUSUM statistics compare the  Bayesian factor between that the data is obtained by a hypothesis $j$ from step $k$ onwards. Maximizing over all $k$ given the worst case.  

==> Archived/Archived/general-hypergame-formulation.tex <==
We choose to model a game under information asymmetry as a hypergame \cite{}. A hypergame model can capture both the misperception of P2 about P1's objective, and the awareness of P1 that the P2 is misperceiving his objective. 


In \cite{}, a hypergame model of level-1 is defined as ${\cal H}^1 = \langle \game_1, \game_2 \rangle$, where $\game_1$ is the game on graph as constructed by P1 given his objective $\varphi_1$ and $\game_2$ is the game on graph as constructed by P2 given his objective $\varphi_2$. When P1 is aware that P2 is misperceiving his objective but P2 is not aware of her misperception, the resulting hypergame is said to be of level-2, and is defined as ${\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle$. In a level-2 hypergame, P1 computes his strategy by solving the level-1 hypergame, while P2 computes his strategy by solving the game on graph $\game_2$. 


The above hypergame model from \cite{} does not account for evolving misperception in the game. When P2 is equipped with an inference mechanism, her misperception evolves and so does her strategy. One way to understand P2's evolving misperception and its effect on her strategy is the following. Let $\mathsf{LTL}$ be the range of P2's inference mechanism $\eta$. Then, for every \ac{ltl} formula $\Psi \in \mathsf{LTL}$, P2 will construct a game on graph $\game(\Psi)$ in which P2's objective is to satisfy $\varphi_2 = \neg \Psi$. In general, given a finite set of atomic propositions $AP$, the set $\mathsf{LTL}$ is infinite. However, in this paper, we study the case where $\mathsf{LTL}$ is finite. 


\begin{assumption}
Let $\mathsf{LTL}$ denote a finite subset of \ac{ltl} specifications that can be defined using a finite set of atomic propositions, $AP$.
\end{assumption}


Let the specifications in $\mathsf{LTL}$ be denoted by $\Psi_i$ for $i = 1, 2, \ldots, N$. Then at some state $s \in {\cal S}$, based on her current misperception $\psi_t \in \mathsf{LTL}$, P2 plays the best strategy for her in the game $\game(\psi_t)$. \todo[inline]{ambiguous. best = best according to bounded rational model} To explicitly capture the dependence of hypergames on P2's misperception at time $t$, we define hypergame as follows. 


\begin{definition}[Hypergame]
Given a finite set $\mathsf{LTL}$ of \ac{ltl} specifications, a level-1 hypergame is defined as 
\[
    {\cal H}^1(\psi_t) = \langle \game(\varphi_1), \game(\psi_t)  \rangle
\]
where P1 is playing the game $\game(\varphi_1)$, and P2 is playing the game $\game(\psi_t) \in \{\game(\Psi_1), \game(\Psi_2), \ldots, \game(\Psi_N)\}$. And a level-2 hypergame is given by 
\[
    {\cal H}^2(\psi_t) = \langle {\cal H}^1(\psi_t), \game(\psi_t) \rangle
\]
\end{definition}


% When the domain and the range of inference mechanism $\eta$ (see Def.~\ref{}) of P2 is finite, it is possible to define a game on graph like structure for a level-1 hypergame, which we call a \textit{hypergame on graph}. 


Given the definition of hypergame, we now define a new graph---which we call a ``Hypergame on Graph"---to model the hypergame ${\cal H}^1(\psi_t)$ that P1 uses to compute his winning strategy. 


\begin{definition}[Hypergame on Graph]
Let $TS$ be a transition system and ${\cal A}_1 = \langle Q_1, \Sigma, \delta_1, q_{01}, F_1, Acc_1 \rangle$ be a \ac{dfa} equivalent to the specification $\varphi_1$. Similarly, let ${\cal A}_2^i = \langle Q_2^i, \Sigma, \delta_2^i, q_{02}^i, F_2^i, Acc_2 \rangle$ be a \ac{dfa} equivalent to specification to $\Psi_i$ for $\Psi_i \in \mathsf{LTL}$. Let ${\cal I} = \{1, 2, \ldots, N\}$ be an indicator set over the set $\mathsf{LTL}$. Let ${\cal A} = \langle Q, \Sigma, \delta, q_{0}, F, Acc_2 \rangle$ be the union of ${\cal A}_1$ and all \ac{dfa}s ${\cal A}_2^i$. Then, a hypergame on graph is the tuple \todo[inline]{Define DFA union in preliminaries. }
\[
    {\cal H} = \langle V, Act, \Delta, ({\cal F}_1, Acc_1), ({\cal F}_2, Acc_2) \rangle
\]
where the components of hypergame graph are as follows
\begin{itemize}
    \item $V = S^{\ast} \times Q \times {\cal I}$, where $h \in S^{k}$ is an ordered sequence of $TS$ states of length $k$, $q \in Q$ is the automata state and $i \in \cal I$ is the game that P2 is playing based on her misperception. We shall refer to $h$ as history, and write it as $h = (s_{0}, \ldots, s_k)$. When history is not available for length $k$, the unknown components will be replaced with $\emptyset$. The state $s_k$ represents the current state in $TS$. 
    
    \item $Act$ is the set of actions. 
    
    \item $\Delta: V \times Act \rightarrow \distr(V)$ is a stochastic transition function. A state $(h', q', i') \in V$ is included in $\Delta((h, q, i), a)$ if and only if $s_t' \in \supp(T(s_t, a))$ and $h'[0:k-1] = h[1:k]$ and $q' = \delta(q, L(s_k'))$ and $i' = \eta(\psi_0, h')$, where $\psi_0$ is the initial misperception. In such a case, $\mathbb{P}((h', q', i') \in V \mid (h, q, i) \in V, a \in Act) = \mathbb{P}(s' \in S \mid s \in S, a \in Act)$. 
    
    \item $({\cal F}_1, Acc_1)$ represents the objective for P1. The set ${\cal F}_1$ is defined as $S^k \times F_1 \times {\cal I}$. $Acc_1 \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P1.
    
    \item $({\cal F}_2, Acc_2)$ represents the objective for P2. The set ${\cal F}_2$ is defined as ${\cal F}_2 = \{(h, q, i) \in V \mid h \in S^k \text{ and } q \in F_2^i\}$. $Acc_2 \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P2.
    
    \todo[inline]{Fix notation: $\Delta, \cal F$ are repeated in $\game$ and $\cal H$.}
\end{itemize}
\end{definition}




% \begin{definition}[Hypergame]
% Let $\game_1$ and $\game_2$ be the games on graph as constructed by P1 and P2 in their mind, given P1's objective is to satisfy $\varphi_1$ and P2's objective is to satisfy $\varphi_2$. Then, a \textit{first-level} hypergame is a tuple
% \[
%     {\cal H}^1 = \langle \game_1, \game_2 \rangle.
% \]

% When one player is aware of misperception and other is not, we get a \textit{second-level} hypergame, given by the tuple
% \[
%     {\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle
% \]
% where P1 solves the first-level hypergame to compute his strategy. 
% \end{definition}


% We note that a \textit{second-level} hypergame models the game with information asymmetry described in Problem~\ref{}. We refer the reader to \cite{} for a general treatment of $k$-th level hypergame. 


% A definition of hypergame given in Def.~\ref{} does not account for evolving misperception. 




% % When P1 is aware of P2's misperception, P1 computes his strategy by anticipating the P2's strategy, given her perception $\psi_t$ of P1's objective. In order to anticipate P2's strategy, P1 must first construct a model of his opponent, P2. An opponent model consists of what P1 knows about (a) how P2 perceives P1's objective at $t=0$, (b) how P2 updates her misperception, \ie the inference mechanism of P2, and (c) given the misperception $\psi_t$, how does P2 compute her strategy.



==> Archived/Archived/hypergame-19Nov19.tex <==
We choose to model a game under information asymmetry as a hypergame \cite{}. A hypergame model can capture both the misperception of P2 about P1's objective, and the awareness of P1 that the P2 is misperceiving his objective. 


In \cite{}, a hypergame model of level-1 is defined as ${\cal H}^1 = \langle \game_1, \game_2 \rangle$, where $\game_1$ is the game on graph as constructed by P1 given his objective $\varphi_1$ and $\game_2$ is the game on graph as constructed by P2 given his objective $\varphi_2$. When P1 is aware that P2 is misperceiving his objective but P2 is not aware of her misperception, the resulting hypergame is said to be of level-2, and is defined as ${\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle$. In a level-2 hypergame, P1 computes his strategy by solving the level-1 hypergame, while P2 computes his strategy by solving the game on graph $\game_2$. 


The above hypergame model from \cite{} does not account for evolving misperception in the game. When P2 is equipped with an inference mechanism, her misperception evolves and so does her strategy. One way to understand P2's evolving misperception and its effect on her strategy is the following. Let $\mathsf{LTL}$ be the range of P2's inference mechanism $\eta$. Then, for every \ac{ltl} formula $\Psi \in \mathsf{LTL}$, P2 will construct a game on graph $\game(\Psi)$ in which P2's objective is to satisfy $\varphi_2 = \neg \Psi$. In general, given a finite set of atomic propositions $AP$, the set $\mathsf{LTL}$ is infinite. However, in this paper, we study the case where $\mathsf{LTL}$ is finite. 


\begin{assumption}
Let $\mathsf{LTL}$ denote a finite subset of \ac{ltl} specifications that can be defined using a finite set of atomic propositions, $AP$.
\end{assumption}


Let the specifications in $\mathsf{LTL}$ be denoted by $\Psi_i$ for $i = 1, 2, \ldots, N$. Then at some state $s \in {\cal S}$, based on her current misperception $\psi_t \in \mathsf{LTL}$, P2 plays the best strategy for her in the game $\game(\psi_t)$. \todo[inline]{ambiguous. best = best according to bounded rational model} To explicitly capture the dependence of hypergames on P2's misperception at time $t$, we define hypergame as follows. 


\begin{definition}[Hypergame]
Given a finite set $\mathsf{LTL}$ of \ac{ltl} specifications, a level-1 hypergame is defined as 
\[
    {\cal H}^1(\psi_t) = \langle \game(\varphi_1), \game(\psi_t)  \rangle
\]
where P1 is playing the game $\game(\varphi_1)$, and P2 is playing the game $\game(\psi_t) \in \{\game(\Psi_1), \game(\Psi_2), \ldots, \game(\Psi_N)\}$. And a level-2 hypergame is given by 
\[
    {\cal H}^2(\psi_t) = \langle {\cal H}^1(\psi_t), \game(\psi_t) \rangle
\]
\end{definition}


% When the domain and the range of inference mechanism $\eta$ (see Def.~\ref{}) of P2 is finite, it is possible to define a game on graph like structure for a level-1 hypergame, which we call a \textit{hypergame on graph}. 


Given the definition of hypergame, we now define a new graph---which we call a ``Hypergame on Graph"---to model the hypergame ${\cal H}^1(\psi_t)$ that P1 uses to compute his winning strategy. 


\begin{definition}[Hypergame on Graph]
Let $TS$ be a transition system and ${\cal A}_1 = \langle Q_1, \Sigma, \delta_1, q_{01}, F_1, Acc_1 \rangle$ be a \ac{dfa} equivalent to the specification $\varphi_1$. Similarly, let ${\cal A}_2^i = \langle Q_2^i, \Sigma, \delta_2^i, q_{02}^i, F_2^i, Acc_2 \rangle$ be a \ac{dfa} equivalent to specification to $\Psi_i$ for $\Psi_i \in \mathsf{LTL}$. Let ${\cal I} = \{1, 2, \ldots, N\}$ be an indicator set over the set $\mathsf{LTL}$. Let ${\cal A} = \langle Q, \Sigma, \delta, q_{0}, F, Acc_2 \rangle$ be the union of ${\cal A}_1$ and all \ac{dfa}s ${\cal A}_2^i$. Then, a hypergame on graph is the tuple \todo[inline]{Define DFA union in preliminaries. }
\[
    {\cal H} = \langle V, Act, \Delta, ({\cal F}_1, Acc_1), ({\cal F}_2, Acc_2) \rangle
\]
where the components of hypergame graph are as follows
\begin{itemize}
    \item $V = S^{\ast} \times Q \times {\cal I}$, where $h \in S^{k}$ is an ordered sequence of $TS$ states of length $k$, $q \in Q$ is the automata state and $i \in \cal I$ is the game that P2 is playing based on her misperception. We shall refer to $h$ as history, and write it as $h = (s_{0}, \ldots, s_k)$. When history is not available for length $k$, the unknown components will be replaced with $\emptyset$. The state $s_k$ represents the current state in $TS$. 
    
    \item $Act$ is the set of actions. 
    
    \item $\Delta: V \times Act \rightarrow \distr(V)$ is a stochastic transition function. A state $(h', q', i') \in V$ is included in $\Delta((h, q, i), a)$ if and only if $s_t' \in \supp(T(s_t, a))$ and $h'[0:k-1] = h[1:k]$ and $q' = \delta(q, L(s_k'))$ and $i' = \eta(\psi_0, h')$, where $\psi_0$ is the initial misperception. In such a case, $\mathbb{P}((h', q', i') \in V \mid (h, q, i) \in V, a \in Act) = \mathbb{P}(s' \in S \mid s \in S, a \in Act)$. 
    
    \item $({\cal F}_1, Acc_1)$ represents the objective for P1. The set ${\cal F}_1$ is defined as $S^k \times F_1 \times {\cal I}$. $Acc_1 \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P1.
    
    \item $({\cal F}_2, Acc_2)$ represents the objective for P2. The set ${\cal F}_2$ is defined as ${\cal F}_2 = \{(h, q, i) \in V \mid h \in S^k \text{ and } q \in F_2^i\}$. $Acc_2 \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P2.
    
    \todo[inline]{Fix notation: $\Delta, \cal F$ are repeated in $\game$ and $\cal H$.}
\end{itemize}
\end{definition}

\todo[inline]{limit the number of switching. using switching game formulation.}

Write about what if $F_2, Acc_2 $ not considered. 


% \begin{definition}[Hypergame]
% Let $\game_1$ and $\game_2$ be the games on graph as constructed by P1 and P2 in their mind, given P1's objective is to satisfy $\varphi_1$ and P2's objective is to satisfy $\varphi_2$. Then, a \textit{first-level} hypergame is a tuple
% \[
%     {\cal H}^1 = \langle \game_1, \game_2 \rangle.
% \]

% When one player is aware of misperception and other is not, we get a \textit{second-level} hypergame, given by the tuple
% \[
%     {\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle
% \]
% where P1 solves the first-level hypergame to compute his strategy. 
% \end{definition}


% We note that a \textit{second-level} hypergame models the game with information asymmetry described in Problem~\ref{}. We refer the reader to \cite{} for a general treatment of $k$-th level hypergame. 


% A definition of hypergame given in Def.~\ref{} does not account for evolving misperception. 




% % When P1 is aware of P2's misperception, P1 computes his strategy by anticipating the P2's strategy, given her perception $\psi_t$ of P1's objective. In order to anticipate P2's strategy, P1 must first construct a model of his opponent, P2. An opponent model consists of what P1 knows about (a) how P2 perceives P1's objective at $t=0$, (b) how P2 updates her misperception, \ie the inference mechanism of P2, and (c) given the misperception $\psi_t$, how does P2 compute her strategy.



==> Archived/Problem_formulation.tex <==
We consider the problem of computing optimal strategies for a controllable player, Alice (P1), in a game where P1 plays against an adversarial uncontrollable player, Bob (P2), who has partial information about P1's objective in the game. We assume that (a) P1 and P2 are bounded-rational players, (b) P1 knows what P2 believes to be her objective at the beginning of the game, (c) P1 knows how P2 updates his belief after observing the game play, and (d) P1 and P2 have complete observability of the game. Under assumptions (b) and (c), we note that the above game is a two-player zero-sum game under information asymmetry \cite{}. 


We, now, describe the formalism used to characterize the interaction between P1 and P2. The game between P1 and P2 is said to be played over a game arena (hereby referred to as simply, arena). 


{\definition[Arena] An arena is a digraph, $G = \langle V, E \rangle$. The set $V$ denotes the set of vertices (interchangeably also called as ``states") of arena and $E \subseteq V \times V$ denotes the edges of arena. 
}

An arena represents: (a) a superset all the states that any player can take, and (b) a superset of all the edges that are accessible to any player, during the game. It is noted that, some states and/or edges in the arena may not be accessible to some players.


Every player in the game is defined by its characteristics. These characteristics define what action capabilities does the player have, what sensing modalities does the player have, or how the player reasons about thinks and reasons about his environment and other players. 


{\definition[Player] Let $G = \langle V, E \rangle$ be an arena. Then, a player in an arena, $G$, is defined as a following tuple, 
\[
    P = \langle G, A, \alpha, AP, L, \varphi, \mu, \eta, B \rangle 
\]
where every element (except $G$) is said to be a characteristic of the player and is defined as, 
\begin{itemize}
    \item $A$ is a set of actions that the player can perform.
    
    \item $\alpha \subseteq E \times A$ represents the accessibility relation for the player. Given an edge $(u, v) \in E$ and an action $a \in A$, we abuse the notation and write $(u, a, v) \in \alpha$ to denote that the player reaches the state $v$ by performing an action $a$ at state $u$. 
    
    \item $AP$ is the set of atomic propositions, also called the alphabet of the player. 
    
    \item $L: V \rightarrow 2^{AP}$ is the labeling function that assigns to every vertex $v \in V$, the largest subset of alphabet containing atomic propositions that are true at the given vertex.
    
    \item $\varphi \in \mathsf{LTL}$ is an LTL specification that defines the objective of the player. The set $\mathsf{LTL}$ is the set of all LTL formulas that can be written using the alphabet $AP$. Note that $\mathsf{LTL}$ is, in general, countably infinite set. 
    
    % \item $K$ represents a finite set of information states of the player.
    
    \item $\mu$ is called the misperception function of the player. The misperception of a player is how a player perceives other players and their characteristics in the game. For instance, to capture the misperception of P2 about P1's objective, we write $\mu(\varphi) = \psi$ where $\varphi$ and $\psi$ are LTL formulas. Note that, the misperception of a player, say P1, about another player, say P2, depends on the information available with P1 about the P2. 
    
    \item $\eta$ is called as an inference mechanism. An inference mechanism represents how the player updates the misperception function $\mu$, given the game play (see Def.~\ref{} below). 
    
    \item $B$ is a model of mind. For instance, a bounded-rational player's mind can be modeled using k-level theory \cite{}, Cognitive Hierarchy model \cite{}, \etc, whereas a rational player may be modeled by defining a solver used by the player, such as  Nash equilibrium solver or Zielonka solver \etc, to solve for equilibrium.  
\end{itemize}
}


\begin{remark}
The accessibility relation, $\alpha$, represents a subset of edges $E \times A$ accessible to the player, \ie enabled for the player. When for a every pair $(u, a)$, there exists a unique $v \in V$ such that $(u, a, v) \in \alpha$, we say that $\alpha$ is a deterministic. We usually denote a deterministic accessibility relation as $\alpha: V \times A \rightarrow V$. Otherwise, $\alpha$ is said to be non-deterministic. To represent a stochastic accessibility relation, we associate a probability value $p \in [0, 1]$ with every edge, thus writing an edge in $\alpha$ as $(u, a, v, p)$.
\end{remark}


A game consists of two players, $P_1$ and $P_2$, each defined using their characteristics $X_i$ where $i \in \{1, 2\}$ and $X$ can take values from the set $\{A, \alpha, AP, L, \varphi, \mu, \eta, B\}$. Both players, P1 and P2, construct their own model of game using the arena $G$ and a model of their opponent $P_j^i = \mu_i(P_j)$ for $i \neq j$. The player computes his/her strategy by solving the constructed game. 


Let us set up the player characteristics, for this article, to represent a zero-sum game under information asymmetry. 

\begin{itemize}
    \item P1: has Complete Information
    \begin{itemize}
        \item $A_1, \alpha_1$: are the set of actions and accessibility relation for P1. 
        \item $AP, L$: are the alphabet and labeling function common to both, P1 and P2. 
        \item $\varphi_1$ is a \textit{Syntactically-Cosafe LTL} objective of P1. 
        \item $\mu = \cal{I}$, where $\cal{I}$ represents an identity function. This represents that P1 has no misperception about P2. 
        \item \textcolor{red}{$\eta$ is not necessary, because P1 has complete information and complete observation. However, it seems we are trying to infer $B$ of P2 to estimate the level of P2's thinking! This would mean we have \textit{a general game with incomplete information, not just asymmetry, right?}}
        \item $B$ is a level-$k$ Cognitive Hierarchy (CH) solver. 
    \end{itemize}
    
    \item P2: does not know P1's true objective.
    \begin{itemize}
        \item $A_2, \alpha_2$: are the set of actions and accessibility relation for P2. 
        \item $AP, L$: are the alphabet and labeling function common to both, P1 and P2. 
        \item $\varphi_2$ is the objective of P2. Ideally, as we want to define a zero-sum game, $\varphi_2 = \neg \varphi_1$. However, under information asymmetry, P2 does not know P1's true objective. Let $\psi$ be P2's misperception of P1's objective. Then, we write $\varphi_2 = \neg \psi$. We note that $\psi$ might change as the game evolves. 
        \item Given a finite game play $\rho$, the misperception function is given as follows 
            \begin{align*}
                \mu(X, \rho) = \begin{cases}
                           \psi & \text{if } X = \varphi_1 \\
                           {\cal I} &   \text{otherwise}
                         \end{cases}
            \end{align*}
        \item Given a finite game play $\rho$ of length $n$, the inference mechanism $\eta$ is a function that updates P2's misperception of P1' objective, given by $\psi_{n+1} = \eta(\psi_n, \rho)$
        \item $B$ is a CH-solver of level-$k'$ such that $k' < k$.
    \end{itemize}
\end{itemize}


Recall that each player constructs a game in his/her brain. This game is constructed in two steps: (a) by constructing a transition system to capture the dynamics of their interaction, and (b) by constructing an automaton that accepts the language of sc-LTL specification that represents their objective(s). As we want to synthesize strategy for P1, we will define the following terms from P1's perspective. 


\textbf{Step 1:} A transition system may be of two types; turn-based or concurrent. 

\begin{definition}[Turn-based Transition System]
Given P1's model, $P_1$, and P1's perception of P2, $P_2^1$, the transition system, as constructed by P1 in his own mind when the interaction is \textit{turn-based}, is given by 
    \begin{align}
        TS = \langle S, Act, T, AP, L \rangle
    \end{align}
where
    \begin{itemize}
        \item $S = V \times V \times \{1, 2\}$ is the set of states in the transition system. A state $(v_1, v_2, 1)$ represents that P1 is at state $v_1$ in arena, P2 is at state $v_2$ in arena and it is P1's turn to make a move. 
    
        \item $Act = A_1 \cup A_2$ where $A_1$ and $A_2$ are action sets of P1 and P2, respectively. 
        
        \item $T \subseteq S \times Act \times S$ is the accessibility relation in the transition system. $T$ is said to be \textit{deterministic}, if for every pair $(s \in S, a \in Act)$ there exists a unique $s' \in S$ such that $(s, a, s') \in T$. Otherwise, $T$ is said to be non-deterministic. A non-deterministic $T$ is said to be stochastic, when the edge relation satisfies $\sum\limits_{s' \text{ s.t. } (s, a, s') \in T} \mathbb{P}(s' \mid s, a) = 1.0$. 
        
        \item $AP$ is the alphabet of transition system. 
        
        \item $L: S \rightarrow 2^{AP}$ is the labeling function, that assigns to every state $s \in S$, the subset of atomic propositions from $AP$ that are true in the given state. The function is defined as $L(s) = L(v_1) \cup L_2(v_2)$. 
    \end{itemize}
\end{definition}


\begin{definition}[Concurrent Transition System]
Given P1's model, $P_1$, and P1's perception of P2, $P_2^1$, the transition system, as constructed by P1 in his own mind when the interaction is \textit{concurrent}, is given by 
    \begin{align}
        TS = \langle S, Act, T, AP, L \rangle
    \end{align}
where
    \begin{itemize}
        \item $S = V \times V$ is the set of states in the transition system. A state $(v_1, v_2, 1)$ represents that P1 is at state $v_1$ in arena, P2 is at state $v_2$ in arena and it is P1's turn to make a move. 
    
        \item $Act = A_1 \times A_2$ where $A_1$ and $A_2$ are action sets of P1 and P2, respectively. 
        
        \item $T \subseteq S \times Act \times S$ is the accessibility relation in the transition system. $T$ is said to be \textit{deterministic}, if for every pair $(s \in S, a \in Act)$ there exists a unique $s' \in S$ such that $(s, a, s') \in T$. Otherwise, $T$ is said to be non-deterministic. A non-deterministic $T$ is said to be stochastic, when the edge relation satisfies $\sum\limits_{s' \text{ s.t. } (s, a, s') \in T} \mathbb{P}(s' \mid s, a) = 1.0$. 
        
        \item $AP$ is the alphabet of transition system. 
        
        \item $L: S \rightarrow 2^{AP}$ is the labeling function, that assigns to every state $s \in S$, the subset of atomic propositions from $AP$ that are true in the given state. The function is defined as $L(s) = L(v_1) \cup L_2(v_2)$. 
    \end{itemize}
\end{definition}


\textbf{Step 2:} A deterministic finite automaton (DFA) is given by $A = \langle Q, \Sigma, \delta, q_0, F \rangle$. It is known result that, given a sc-LTL specification $\varphi$, there exists a DFA that accepts the same language as that of $\varphi$. 


Given a transition system and an automaton $A_1$ equivalent to his specification $\varphi_1$, P1 constructs a zero-sum game as follows


\begin{definition}[Game]
Let a turn-based (resp. concurrent) transition $TS = \langle S, Act, T, AP, L \rangle$ and an DFA $A = \langle Q, \Sigma, \delta, q_0, F \rangle$ be given. Then, a turn-based (resp. concurrent) game is defined as 
\[
    \game = \langle S \times Q, Act, \Delta, F \rangle
\]
where 
\begin{itemize}
    \item usual definitions
\end{itemize}
\end{definition}


The game as defined above is ignorant of model of the opponent, and assumes the opponent to be a perfect adversary; \ie an opponent with complete information and complete observation. However, under information asymmetry, P1 incorporates the model of opponent $P_2^1$, which accounts for P2's misperception, into his decision-making. This yields a hypergame, in contrast to a game. 


\begin{definition}[Hypergame]
Let $\game_1$ be a game constructed by P1 using his own model; $P_1$, and $\game_2$ be a game constructed by P2 using her model of herself; $P_2$. Then, a first-level hypergame is defined as
\[
    {\cal H}^1 = \langle \game_1, \game_2 \rangle
\]

When P1 uses his model of P2; $P_2^1$, to make his decision-making, we represent the interaction using a second-level hypergame,
\[
    {\cal H}^2 = \langle (\game_1, \game_2^1), \game_2 \rangle
\]
\end{definition}


\begin{remark}
In a second-level hypergame, P1 computes his strategy by solving a first-level hypergame. 
\end{remark}


\begin{remark}
As P1 has complete information, $\game_2^1 = \game_2$.
\end{remark}


It is easy to confuse between the levels of a CH-model and levels of a hypergame. We understand that CH-model (characteristic $B_1$ of P1 and $B_2$ of P2) represents how a player computes his/her strategy given the player structure $P_i$. Whereas, the levels of hypergame represent the awareness of a player about the other player's awareness of existing misperception. For instance, in a second-level hypergame (where P1 solves first-level hypergame), P1 will solve the game $\game_2$ using $B_2^1$ to estimate P2's response strategy given the player structure $P_2^1$. When using CH-model to model bounded-rationality, $B_2^1$ could compute strategy for a $k'$-level agent, for some $k' < k$ and $k$ being the level of CH-model solver $B_1$. 


We now formalize the problem as follows, 
\begin{problem}
Let $P_1$ and $P_2$ represent the player structures for two bounded-rational players P1 and P2 interacting over an arena $G$, with characteristics as described in above section. Then, synthesize an almost-sure winning strategy and an optimal response strategy in positive-winning for P1. 
\end{problem}




% We represent the objectives of players as a Syntactically-Cosafe Linear Temporal Logic (sc-LTL) specifications. At the beginning of the game, let $\varphi$ be the specification of P1, and $\psi$ be P2's misperception of P1's objective. Then, had P2 been a rational agent, P2 would have played a game to satisfy the negation of P1's objective, \textit{i.e.} P2 tries to satisfy $\neg \psi$. However, we assume the players to be bounded-rational and, hence, they cannot solve for equilibrium strategy. Nonetheless, when $\psi = \varphi$, we observe that the strategy synthesis problem reduces to conventional reactive synthesis. Therefore, we focus on the case where $\psi \neq \varphi$ at the beginning of the game. 


% We start by defining the notion of winning for P1 and P2 in the game. A \textit{play} of the game is an ordered sequence, $\rho = (s_0, a_0^1, a_0^2), (s_1, a_1^1, a_1^2), \ldots, $ where at every turn both players; P1 and P2, choose an action, which is independent of their opponent's choice of action at that turn. In other words, the game is a concurrent (\textit{a.k.a.} simultaneous) game. In such a game, we say P1 has won the game when $\rho \models \varphi$\footnote{Let $\mathsf{Occ}(\rho) = \{s \mid s \in \rho\}$ represent the set of states appearing in the play $\rho$. Then, we say $\rho \models \varphi$ when $\mathsf{Occ}(\rho) \cap F \neq \emptyset$.}, and P2 has won the game when $\rho \not\models \varphi$. Note that, we define winning based on ``true" objective of P1. Therefore, P2 does not win the game by satisfying $\neg\psi$, because $\psi$ is not the true objective of P1. 


% Given that P2 starts with a misperception $\psi$ of P1's objective, it is possible that P2 may infer P1's ``true" objective; $\varphi$, by observing P1's behavior in the game. To capture this capability of P2, we equip him with an inference mechanism, which is a function that maps P2's misperception at current turn $t$, say $\psi_{t}$, and a finite history of states; $h \in S^\ast$, to produce a new misperception $\psi_{t+1}$. Formally, we define an inference mechanism as follows,  


% \begin{definition}[Inference Mechanism]
% Let $G$ be a subset of $S$ and $\mathsf{LTL}$ be the set of all LTL formulas that can be defined over a finite set $AP$ of atomic propositions. An inference mechanism is a function $\eta: \mathsf{LTL} \times S^\ast \rightarrow \mathsf{LTL}$, which maps a current misperception $\psi_t$ of P2 and a finite history of states $h \in S^\ast$ to a return an updated misperception $\psi_{t+1}$ of P1's objective. 
% \end{definition}


% In this article, we restrict the scope of inference mechanism to inferring parameterized sc-LTL objectives. For example, given a set of states $G \subseteq S$, we may represent P2's misperceived objective of P1 as $\psi_t = \Diamond g_t$, where $g_t \in G$. In this case, the problem of inferring an LTL specification reduces to the problem of estimating the current sub-goal that P1 is pursuing from the set $G$. One approach for sub-goal inference is using \textit{change detection with adaptive sliding window}, described in Sect.~\ref{}. 


% The inference mechanism describes how P2 updates his knowledge, and thus the game he plays against P1. However, P2 is assumed to be a bounded rational. In this article, we use Cognitive Hierarchy (CH) model to represent bounded rationality of players, which is described in Sect.~\ref{}. Given the model of bounded rationality and an inference mechanism, we formalize the problem statement. 


% \begin{problem}
% Assume that P1 is a $k$-level thinker, according to CH model, and knows the inference mechanism $\eta$ by which P2 updates his misperception. Then, synthesize a deceptive strategy $\pi: S \rightarrow A_1$ for P1 that can deceive P2 by controlling his misperception, if necessary, to ensure that P1 will satisfy $\varphi$ with probability one.  
% \end{problem}



==> Archived/archieved.tex <==
The subgoal inference with sliding window change detection can be represented as an inference function $\update: G \times H^{\le k}\rightarrow G \times H^{\le k}$ that maps a current hypothesis and a finite history of length $\le k$ to a new hypothesis and a new history. When a change is detected,  the new history only consists of the most recent observation, that is, a transition in the arena. When there is no change, the new history is obtained by appending the old history with the new observation.

Let $k$ be the maximum length of the sliding window size, $H^{\le k}$ be the set of possible histories of length smaller than or equals $k$, and $G$ be a set of possible subgoals. Consider the inference $\update: G \times H^{\le k}\rightarrow G \times H^{\le k}$, we construct a new game-arena with augmented state space as follows.
\[ \hat M =  (   \vS \times H^{\le k}\times G, \vA, \hat T, \calap, \hat L)
\]
\begin{itemize}
\item  $ \hat \vS= \vS\times H^{\le k}\times G$ is a finite set of states. Each state $(\vs, h, g)$ includes a current game state $\vs$, a finite observation hostory of length $\le k$ and a subgoal $g \in G$.
\item $\hat T :  \vS\times  H^{\le k}\times G \times \vec{A}\rightarrow  \dist{\vS\times  H^{\le k}\times G}$ is the probabilistic transition function, defined as follows.
\begin{multline}
\hat T ( (\vs' , h', g')|(\vs, h, g), (a_1,a_2)) \\=\left\{ \begin{array}{ll}  P(\vs'|\vs, (a_1,a_2)) & \text{ if }  (h',g')= \update( (h, (a_1,a_2), \vs'), g).\\
0 & \text{otherwise}.
\end{array}\right.
\end{multline}
That is, the transition to a new state is probabilistic and follows the transition function in the stochastic system. The history of observations is updated by the subgoal inference, as well as the predicted subgoal.
\item $\calAP$ is a finite set of atomic propositions.
\item $ \hat L: \vS\times H^{\le k}\times G \rightarrow 2^\calAP $ is the labeling function, defined as $\hat L((\vs, h, g))= L(\vs)$.  That is, the label of an augmented state is determined by the label of the first component---that is, the state in the stochastic system. 
\end{itemize}

\begin{algorithm}[!htb]
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE{The sequence of the adversary fictitious inputs}
\ENSURE{The mean level $\lambda^{n}$}
    \FOR{$i = 0, \dots, T$}
        \FOR{$k = 0, \dots, \calK$}
        \STATE{for $t \in [0, n]$, measure the value of \eqref{eqn:r_k}}
        \ENDFOR
        \FOR{$k = 0, \dots, \calK$}
            \STATE{Compute the mean level according to~\eqref{eqn:sigma_k}}
        \ENDFOR
        \STATE{Update the estimation according to~\eqref{eq:lambda_update}}
    \ENDFOR
\end{algorithmic}
\caption{Intelligence Level Learning}
\end{algorithm}


==> Archived/archieved_change_detection.tex <==

\newpage 

\begin{itemize}
    \item observations $y_{1,t}$
    \item hidden sequence of states: $z_{1,t}$ where $z_t$ is assumed to be the goal pursuit by agent at time $t$.
    \item the run length: $r_t$--that is a non- negative discrete quantity denoting the number of time steps elapsed at time t since the last change point occurred in the sequence. It holds that $r_t = 0$ at a change point.
\end{itemize}

The following prior is given:
\[
P(z_t|z_{t-1})
\]
however, the duration $P(d_t|z_t)$ is not given but to be detected.

objective: to compute 
\[
P(r_t,z_t |y_{1,t})
\]
in a online manner.

\begin{align*}
    \gamma_t  = & P(r_t,z_t ,y_{1,t})\\
     = & \sum_{r_{t-1}}\sum_{z_{t-1}}P(r_t,z_t, r_{t-1},z_{t-1}, y_{1,t})\\
    = &\sum_{r_{t-1}}\sum_{z_{t-1}} P(r_t,z_t| r_{t-1},z_{t-1}, y_{1,t}) P(r_{t-1}, z_{t-1}, y_{1,t}) \\
    = &\sum_{r_{t-1}}\sum_{z_{t-1}} P(r_t,z_t| r_{t-1},z_{t-1}, y_{1,t}) P(r_{t-1}, z_{t-1}, y_{1,t-1}, y_t) \\
    = &\sum_{r_{t-1}}\sum_{z_{t-1}} P(r_t,z_t| r_{t-1},z_{t-1}, y_{1,t}) P(y_t| r_{t-1}, z_{t-1}, y_{1,t-1})\cdot P(r_{t-1}, z_{t-1}, y_{1,t-1}) \\
     =  & \sum_{r_{t-1}}\sum_{z_{t-1}} 
     P(r_t,z_t| r_{t-1}, z_{t-1}, y_{1,{t}})P(y_t | r_{t-1}, z_{t-1}, y^{(r_{t-1})})\cdot P(r_{t-1},z_{t-1}, y_{1,t-1})\\
     =  & \sum_{r_{t-1}}\sum_{z_{t-1}} 
     P(r_t,z_t| r_{t-1}, z_{t-1}, y_{1,{t}})P(y_t | r_{t-1}, z_{t-1}, y^{(r_{t-1})})\cdot \textcolor{blue}{\gamma_{t-1}}.
\end{align*}
The calculation $ P(y_t| r_t,z_t, y^{r_t}) = P(y_t| z_t, y^{r_t}) $ can be obtained from the predictive model given goal $z_t$ and history $y^{r_t}$.

The question is how to calculate
\[
P(r_t,z_t| r_{t-1}, z_{t-1}, y_{1,{t}})
\]

in bayesian online change point detection, hazard function is introduced to define $P(r_t|r_{t-1})$. For example, geometric distribution.

This prior information is not easy to assume in our setting.

We use change detection to predict.
\[
P(r_t,z_t| r_{t-1}, z_{t-1}, y_{1,{t}})
= 1- {1}(\max_{j\in Z}B^j(z_{t-1}) > A)
\]

where $Z$ is the domain of $z_t$,  $B^{j}(z_{t-1})$ is CUmulative SUM statistic (CUSUM)
defined by 
\[
B^{j}(z_{t-1}) =  \max_{1 \le k \le m}\frac{P_j(y_{k,m}^{(r_{t-1})})}{P_0(y_{k, m}^{(r_{t-1})})},
\]
where $m$ is the window size that depends on the false alarm constraints, $P_j$ is calculated from the hypothesis $j$ (an alternative mode), $P_0$ is calculated from the hypothesis $z_{t-1}$ (the current mode, assuming no change). For step $k=1,2,\ldots m $, we compare each step and see if significant change has been detected given two comparison. When at least one alternative $j$ and a step $k$ yields large Bayes factor, then a change is detected and $r_t$ is reset to zero. Otherwise, $r_t= r_{t+1}+ 1$.

In short, the CUSUM statistics compare the  Bayesian factor between that the data is obtained by a hypothesis $j$ from step $k$ onwards. Maximizing over all $k$ given the worst case.  

==> Archived/case-study.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Parameters of different algorithms %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we illustrate the proposed algorithm in a robot motion planning example in adversarial environment, shown in Fig.~\ref{fig:grid_world}. In this game, P1 (Blue agent) is to achieve a given temporal logic specification $\varphi$ while player 2 (Red) is the opponent. Both players can move deterministically and simultanously in four compass directions in this $11$-by-$11$ grid world, with action sets $\{\mbox{Up} (U), \mbox{Down} (D), \mbox{Left} (L), \mbox{Right} (R)\}$. In this environment, there are a set of obstacles (marked in black cells) and several critical way-points, marked as $g_i=(x_{g_i}, y_{g_i}), i=1,\ldots, 4$. If a player hits the boundary of the grid world or any obstacles, it will stay put in its original cell. 

\begin{figure}[!htb]
\begin{subfigure}[b]{0.786\linewidth}
    \includegraphics[width=\linewidth]{Figure/fancy_grid_world.png}
    \caption{ }
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{Figure/3th_simulation_grid.png}
    \caption{ }
\end{subfigure}
\caption{(a) The grid world (b) The simulation with the complex specification is: $\neg (p_1\land p_2)  \until ( \Eventually (\mathsf{Reach}(g_1)  \land \Eventually \mathsf{Reach}(g_4) )\\ \lor 
\Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) )$}
\label{fig:grid_world}
\end{figure}
%%% task specification
The following atomic propositions are used: Given that P1's position is $(x_1,y_1) $ and P2's position is $(x_2,y_2)$, 
\begin{enumerate}
\item $p_1\coloneqq \abs{x_1-x_2} + \abs{y_1-y_2} \le \xi$: this is evaluated true if the Manhattan distance  of P1 and P2 are less than a given threshold $\xi$.  In this experiment, we set $\xi= 1$.
\item $p_2\coloneqq x_1\ge 4$: this is evaluated true if P1 is in the control area of P2. 
\item $\mathsf{Reach}(g_i) \coloneqq (x_1,y_1) = g_i$, for each $i=1,\ldots, 4$. This proposition is evaluated true when P1 reaches a given waypoint $g_i$. It can be generalized to be $(x_1,y_1)\in g_i$ if $g_i$ is a set of cells instead of a single cell. 
\end{enumerate}

\begin{figure}[!htb]
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,scale=0.7,semithick, transform shape]
		\tikzstyle{every state}=[fill=black!10!white]
		\node[initial,state]    (0)                 {$q_0$};
        \node[state]            (1) [right of=0]    {$q_1$};
        \node[state, accepting] (2) [right of=1]    {$q_2$};
		\path[->]   
		(0) 		edge                node    {$g2$}                      (1)
        (1)         edge                node    {$g3$}                      (2)
		;
	\end{tikzpicture}
    \caption{The task automaton for the simple specification
          $\varphi_{simple}$. We omitted the selfloops and transition
          to the sink, nonaccepting state with labeling $\{p_1,p_2\}$
          for clarity.}
\label{fig:simple_automaton}
\end{figure}


    
\begin{figure}[!htb]
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,scale=0.7,semithick, transform shape]
    	\tikzstyle{every state}=[fill=black!10!white]
    	\node[initial,state]    (0)                     {$q_0$};
        \node[state]            (1) [below left of=0]   {$q_1$};
        \node[state]            (2) [below of=0]        {$q_2$};
        \node[state]            (3) [below right of=0]  {$q_3$};
        \node[state, accepting] (4) [below of=2]        {$q_4$};
    	\path[->]   
    	(0) 		edge    node[left]      {$g1$}                      (1)
    	(0) 		edge    node            {$g2$}                      (3)
        (1)         edge    node[left]      {$g2$}                      (2)
        (1)         edge    node[left]      {$g4$}                      (4)
        (2)         edge    node            {$g3 \vee g4$}              (4)
        (3)         edge    node            {$g1$}                      (2)
        (3)         edge    node[above]     {$g3$}                      (4)
    	;
    \end{tikzpicture}
    \caption{The task automaton corresponds to the complex
      specification $\varphi_{complex}$. We omitted self-loops and
      transition to the sink, nonaccepting state with labeling
      $\{p_1,p_2\}$ for clarity.}
\label{fig:complex_automaton}
\end{figure}

We perform several experiments with different \ac{ltl} specifications for P1: 
\begin{itemize}
    \item A simple task specification (with the corresponding \ac{dfa} in Fig.~\ref{fig:simple_automaton}): 
   \[ \varphi_{simple}= \neg (p_1\land p_2) \until \left( \Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) \right).\]
   which is, P1 is to avoid being captured by P2 until it reaches $g_2$ and then $g_3$.
    \item A more complex task specification  (with the corresponding \ac{dfa} in Fig.~\ref{fig:complex_automaton}): 
        \begin{align*}
            \varphi_{complex} = \neg (p_1\land p_2)  \until ( \Eventually (\mathsf{Reach}(g_1)  \land \Eventually \mathsf{Reach}(g_4) )\\ \lor 
            \Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) ).
        \end{align*}
        In words, P1 is to avoid being captured by P2
until it either reaches $g_2$ and then $g_3$, or reaches $g_1$ and then $g_4$.
\end{itemize} 
It is noted that in Fig.~\ref{fig:complex_automaton}, the state $q_2$ means that P1 has just seen $g_1$ and $g_2$. P1 can satisfy the task by visiting either $g_3$ and $g_4$. We design the two specifications with the idea that the language of the simple specification is a subset of that of the complex specification. This is related to one of hypothesises, discussed next.
 

The following hypothesises are considered before the experiments.
\begin{enumerate}
    \item Hypothesis 1: The probability of success given the complex specification  should be higher than that given the simple specification, assuming the same hypothesis space of P2.
    \item Hypothesis 2: Given the same specification, the probability of success given P2's hypothesis space ${\cal X}=\{g_2,g_3\}$ will be lower than that given P2's hypothesis space ${\cal X}= \{g_1,g_2,g_3,g_4\}$. 
    \item Hypothesis 3: By playing deceptively and leveraging the private information, player 1 can achieve better performance in regions that he has no chance of winning had the information is symmetric between players.   
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Figure of the gridworld %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Description of two cases %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To test the hypothesises, we conduct the following experiments: 
\begin{itemize}
    \item Comparison of winning rates between simple and complex specifications: In   experiment 1, P1's tasked with the simple specification (with \ac{dfa}  in Fig.~\ref{fig:simple_automaton}). The hypothesis space for P2 is ${\cal X}=\{g_1,g_2,g_3,g_4\}$--that is, at any time, P2 believes that P1 is pursuing a subgoal within $\cal X$.  In experiment 2, P1 is tasked with the complex specification in Fig.~\ref{fig:complex_automaton}. 
    \item Comparison of winning rate for the same specification but different hypothesis spaces of P2: In experiment 3, we consider the same simple specification as that in experiment 1, but change P2's hypothesis space to be ${\cal X}' =\{g_2,g_3\}$.
    \item Analysis of the advantages due to deceptive planning: In experiment 4, we consider the complex specificiation as in experiment 2, but change the initial state to be in the sure losing region of P1 in the game $\game(\varphi_{complex})$ where both players have complete information. 
\end{itemize}
In these experiments, P2 uses level-2 of thinking in the \ac{ch} model. The state space size of the game transition system is $1e+5$. The state space size of the hypergame is up to $1e+43$. The action space size is $16$. Due to the large state space, we use online \ac{mcts} algorithm with the following parameters: the depth of \ac{mcts} simulation is $50$, the number of the simulations is $200$, the exploration scalar $c$ is $\frac{1}{\sqrt{2}}$.  For the change detection algorithm, the window size is $7$, and the threshold is $0.3$. Other parameters are the following: discounting factor $\gamma = 0.8$, the user-specified temperature $\tau$ is $1$. We perform each experiments 100 times and collect the statistics.

The winning rates of the three experiments are shown in Table.~\ref{tab:main_results}. From the experiment, hypothesis 2 is validated:   P2's  easier to be distracted if there are subgoals in her hypothesis that are not pursued by P1. These subgoals becomes decoys that can be used by P1 for deception. Hypothesis 1 is not validated: We anticipate that with the complex specification, P1 could have a higher probability of success than the simple specification. The reason is that the language of the simple specification is a subset of that of the complex one--that is, P1 have more  ways to satisfy the task.
But the winning rate of experiments 2 is slightly lower than that of experiment 1. We expect this is due to the sub-optimality in the online MCTS and will validate the hypothesis with a smaller example for which the exact solution can be obtained. Hypothesis 3 is validated: In the sure-losing region of P1 assuming complete information, P1 can achieve a win rate of $82\%$using deceptive planning that leverages his private information,  comparing to $0\%$ (symmetric information case).


\begin{table}[!htb]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Experiment setups                                                          & Winning rate \\ \hline
 % P1 play level 1 policy, P2 play level 2 policy, goal: g4                   & 0\%          \\ \hline
% P1 play level 3 policy, P2 play level 2 policy, goal: g4                   & 94\%         \\ \hline
1. Simple specification with  ${\cal X} = \{g1, g2, g3, g4\}$                   & 72\%         \\ \hline

2. Complex specification   with  ${\cal X} = \{g1, g2, g3, g4\}$                                                         & 64\%         \\ \hline
3. Simple specification with ${\cal X} =  \{g2, g3\}$                           & 59\%         \\ \hline
4. Starting with sure losing regions for P1 with  complex spec                  & 82\%         \\ \hline
\end{tabular}%
}
\caption{Winning rates under different experiment setups.}
\label{tab:main_results}
\end{table}

% \begin{comment}
 
% \paragraph*{Baseline (Complex specification)}
% Given a specification $\varphi_1=\neg (p_1\land p_2)  \until ( \Eventually (\mathsf{Reach}(g_1)  \land \Eventually \mathsf{Reach}(g_4) )\\ \lor 
% \Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) )$, we construct the game arena with augmented state space. The P1 needs to visit $g2$ first, after visiting $g2$ P1 needs to visit $g3$, or P1 needs to visit $g1$ first, after visiting $g1$ P1 needs to visit $g4$, while avoid being captured by P2.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/3th_prediction.png}
    \caption{The corresponding predictions of P2 in the  trajectory shown in Fig.~\ref{fig:grid_world}.}
    \label{fig:3_th_simulation}
\end{figure}
 Finally, given P1's winning strategy and a predicted strategy of P2, a sampled trajectory is shown in Fig.~\ref{fig:grid_world}. The trajectories of P1 and P2 are shown in blue and red, respectively.
 %A trajectory in the form of 
% \begin{align}
% ((s,q), h, g)
% \xrightarrow{(a_1,a_2)}
% ((s',q'), h', g')
% \end{align}
This trajectory is segmented into two parts: In the first part, P1 uses the deceptive optimally planning and later reaches his winning region for game $\game(\varphi_{safe}\until  \mathsf{Reach}(g_1))$. Then, P1 uses the almost-sure winning strategy of the game $\game(\varphi_{safe}\until  \mathsf{Reach}(g_1))$. After reaching $g_1$, P1 uses deceptive planning  and reaches his winning region for game $\game(\varphi_{safe}\until  \mathsf{Reach}(g_4))$.  Then, P1 uses the almost-sure winning strategy of the game $\game(\varphi_{safe}\until \Eventually \mathsf{Reach}(g_4))$. 
The corresponding prediction of P2's inferred subgoals  is shown in Fig.~\ref{fig:3_th_simulation}. We marked the two time steps when the two almost-sure winning regions are reached. It is observed that once P1 reaches the almost-sure winning region for subgoal $g_1$ (resp. $g_4$), and plays out his almost-sure winning strategy, P2 can correctly infer his subgoal but cannot do anything to prevent P1 from achieving it. Before that, P2's prediction oscillates between four subgoals as an outcome of deception. 

% \paragraph*{Simple specification}
% Given a simple specification $\varphi_1=\neg (p_1\land p_2) \until \left( \Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) \right)$, we construct the game arena with augmented state space. The P1 needs to visit $g2$ first, after visiting $g2$ P1 needs to visit $g3$, while avoid being captured by P2.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Prediction of getting caught %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figure/prediction.png}
%     \caption{The prediction of the single chain with only $\{g2, g3\}$}
%     \label{fig:prediction}
% \end{figure}

\begin{comment}
The following may be used in extended version.

\paragraph*{Complex specification with different initial starting position}
In this case, the P1 starts at $(0, 6)$, and P2 starts at $(4, 2)$.

\paragraph*{Analysis}
In order to get the statically results, we run $100$ simulation between P1 and P2 where P2 is using the level $2$ policy which can be learned from the data. The winning rates under the different experiment setups are shown in the Table~\ref{tab:main_results}. To prove the correctness of the precomputed policy for different levels of policy, we use a simple reach-avoid game which can be described by the P1's specification as the following: 
\begin{align}
\varphi_1 = \neg (p1 \wedge p2)\until \Eventually \mathsf{Reach}(g4) \end{align} 
where P1 is trying to reach $g4$, and P1 uses the level $1$ and level $3$ policies to play again P2 using level $2$ policy.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Table of winning rates %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!htb]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Experiment setups                                                          & Winning rate \\ \hline
P1 play level 1 policy, P2 play level 2 policy, goal: g4                   & 0\%          \\ \hline
P1 play level 3 policy, P2 play level 2 policy, goal: g4                   & 94\%         \\ \hline
Simple specification with decoy set $\{g2, g3\}$                           & 59\%         \\ \hline
Simple specification with decoy set $\{g1, g2, g3, g4\}$                   & 72\%         \\ \hline
Complex specification                                                      & 64\%         \\ \hline
Starting with sure losing regions for P1 with the same complex spec        & 82\%         \\ \hline
\end{tabular}%
}
\caption{Winning rates under different experiment setups.}
\label{tab:main_results}
\end{table}

We compare first two rows in the Table~\ref{tab:main_results}, it indicates that when P1 is using level $1$ policy and P2 is using level $2$ policy, P1 is caught by p2 almost every time out of 100 times. On the other side, when the P1 is playing level $3$ policy and P2 is using the same level of policy, P2 has a very high probability of reaching the goal $g4$. The reason why the winning rate is not $100\%$ is may due to stochasity in the policy caused by the temperature in the softmax bellman operator. 

Comparing the winning rates of simple specification and complex specification, the winning rate of simple specification is no better than that of complex specifications. It demonstrate the effectiveness of the inference. Because when the task automaton is a single chain, it is reasonable to have lower winning rate, since the P2 can quickly infer the subgoal of the P1 and catch the P1. When the task automaton is not a single chain, there are more than one options, P2 can become confused, and it is harder for P2 to catch the P1. 

When the P1 and P2 starting at initial positions which are sure losing for P1, the result shows there is a positive winning rate for P1, which proves the effectiveness of the deception. Since if P2 has the full knowledge of P1, the probability of completing the specification for P1 should be close to $0$. However, when P1 takes the deception into the consideration of planning, the positive winning rate indicates deception help increaing the winning rate. 

% \todo[inline]{Here: include a graph that shows the probability of winning (obtained from value iteration) given P1's strategy in both deceptive planning and the baseline. We hypothesize that the probability of winning should be increased over all sampled states.}

% Then, we consider a mismatch in Blue's opponent model of Red and the true mind of Red. Particularly, we assume that Blue uses a change detection with sliding window of size $n$ and Red uses a change detection with sliding window of size $m$. We test three cases $n=m$, $n=m-k$, and $n=m+k$ and evaluate the probability of satisfying the task from different initial states. \todo[inline]{pick a value of $k$. The hypothesis is that when $n=m-k$ and $k$ is large, the deceptive winning strategy is less effective. When $n=m+k$, the deceptive winning strategy is as good as $n=m$, which was selected long enough to capture the change.}


\end{comment}

To justify that the level $k$ of P2 can be learned correctly, we evaluate the correctness of the proposed opponent modeling method.
\paragraph*{Experimental validation on opponent Modeling}~\label{case_study:opponent_modeling}
We pre-compute the policies of different levels of thinking (until level 4) for P1 and P2 with respect to the decoy $g_1$. 
To validate the correctness of the algorithm, we sample $100$ data points $X = [x_1, x_2, \dots, x_{100}]$ from a Poisson distribution with $\tilde{\lambda} = 2$, which is the ground truth. The goal is to estimate the true $\tilde{\lambda}$. For each date point $x_i$, we use $x_i$-level policy for P2 and $x_i - 1$-level policy for P1 to sample a trajectory with length of $n+1$, where $n=10$. % $\bm{K} = [0,1,2,3,4]^\top$. The user-specified temperature $\tau = 1e-2$.
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{Figure/lambda_learning.png}
    \caption{The convergence of the Poisson parameter $\lambda$ under the update rule~\eqref{eq:lambda_update}.}
    \label{fig:opponent_modeling}
\end{figure}
The following parameters are used in the inference algorithm: The upper bound on the level of thinking of P2 is 4 and the user-specified temperature $\tau = 1e-2$.
Figure~\ref{fig:opponent_modeling} indicates that our algorithm quickly infers the   level of thinking of P2 with a small error, and with the iterations go further, it converges to the ground truth. %We believe that if the data of interaction between P1 and P2 is provided, our algorithm can efficiently infer the truth level of P2's policy.

==> Archived/cognitive_hierarchy.tex <==
In this section, we introduce an efficient algorithm to predict P2's strategy in real-time. This algorithm is based on modeling (the evolving) P2's perceptual game and compute P2's best response in that perceptual game. 

From the perspective of player 1, he   models the perceptual game of P2  with the purpose to  understand how his actions   can influence the hypothesis of P2 about the intention, as well as predicting the counter-strategy of P2 given her hypothesis. 
Given the common knowledge that  a temporal logic formula describes a sequence of temporally extended goals, it is reasonble to consider that P2  tries to infer the changing subgoals of P1 and counteract correspondingly. Thus, we present  a method to model the evolving perception and stratetgy of P2 with 1) Opponent modeling with  cognitive hierarchy; and 2) Change detection algorithm for subgoal inference. 
 
 %Theory of mind with cognitive hierarchy learns the true level $k$ of policy used by P2. The change detection algorithm use the observation between P1 and P2 to update P2's prediction of P1' intention. 

\subsection{Theory of mind with cognitive hierarchy}~\label{sec:cognitive_hierarchy}

One approach of opponent modeling is based on \ac{ch} of
games~\cite{camerer2004cognitive}. In the \ac{ch} of games, players
act according to different levels of reasoning: A player's level-0
strategy is either a nominal strategy or a strategy that randomizes
equally over all actions. A player' level-1 strategy best responds to
an opponent with level-0 strategy. Inductively, a player's level-$k$
strategy best responds to its opponent's level-$(k-1)$ strategy.

% Based on the \ac{ch} model, if P1 knows for which level-$k$ a player P2 is, then P1 not only knows how P2 predicts to be P1's unknown objective as P2 will use the level-$k-1$ policy of P1, but also P1 knows how P2 will respond to the predicted policy of P1.

Given a bounded-rational opponent P2, 
we propose to formulate the opponent modeling as the problem of learning the value of $k$ in P2's level of reasoning.  In \ac{ch} model, it is  discover that each player believes its opponent's level follows a probability distribution~\cite{chong2016generalized}. Thus, we propose an offline learning algorithm to infer P2's level of thinking from the histories. We model the distribution over the different levels as a Poisson distribution with the following probability mass function:
\begin{equation*}
    p^{k} = \frac{\lambda^k e^{-\lambda}}{k!},
\end{equation*}
where $\lambda$ is a parameter. The problem of learning the value of $k$ is transformed into how to estimate the $\lambda$ in the Poisson distribution. 

Given a finite-length history of the game $\rho = \vs_0, (a_0^1, a_0^2), \vs_1, (a_1^1, a_2^2) \dots \vs_n$ where $a_k^i$ is player $i$'s action at the $k$-th step. For a fixed sequence of P1's actions, the probability of $\rho$ for each level-$k$ P2's policy $\pi_2^{(k)}$  is computed by 
\begin{align}
    r^k =  \prod_{t=0}^{n-1} P(\vs_{t+1} \mid \vs_t, \va_t) \cdot \pi_2^{(k)}(a^2_{t} \mid \vs_t) , k \in \{0, 1, \dots, \calK\},
    \label{eqn:r_k}
\end{align}
where $\va_{t} = (a^1_{t}, a^2_{t})$, and $\calK$ is the pre-defined upper bound on the level of thinking of P2. It is noted that the intelligence level $\calK$ tends to infinity, the solution convergences to the Nash equilibrium~\cite{kanellopoulos2019non}. It is noted that this probability $r^k$ does not assume that P1 uses a policy of level $k-1$. 

We compute the scores of different level policies according to: for each $k \in \{0, 1, \dots, \calK\}$,
\begin{equation}
    \sigma^k = \frac{e^{\frac{r^k}{\tau}}}{\sum_{j=1}^{\calK}e^{\frac{r^j}{\tau}}}, 
\label{eqn:sigma_k}
\end{equation}
where $\tau \in \reals^{+}$ is the softmax temperature parameter. We denote $\bm{\sigma} = [\sigma^ 0, \sigma^1, \cdots, \sigma^\calK]^\top$. 

After getting the scores for different policies, we use the following update rule~\cite{frome1973regression} to update the estimation of $\lambda$ in an incremental way, for each past interaction history,
\begin{equation}
    \lambda^{i+1} \leftarrow \frac{i}{i+1} \lambda^{i} + \frac{1}{i+1}\bm{K}^\top \bm{\sigma}, i \in \{0, 1, \dots, T\}
\label{eq:lambda_update}
\end{equation}
where $\bm{K} = [0, 1, \cdots, \calK]^\top$ is a vector of different
levels. The estimated value $\lambda$ gives us a distribution over the
level of thinking for P2 based on past interactions. When P2 is
rational, then based on the \ac{ch} model, $\lambda$ approaches
infinity. Thus, using this inference will not restrict us from playing
against a more rational opponent.

Given the deceptive planning is carried out only once, we assume that P2's level of thinking will not change during interactions. It would be interesting to investigate how P2 adapts her level of thinkings during repeated interactions when P1 employs deceptive strategies.

%Please notice there are difference between the update rules of this and in the paper~\cite{kanellopoulos2019non}. 

\subsection{P2's evolving perceptual game with subgoal inference}~\label{subsec:change_detection}
Given the common knowledge that P1's objective $\varphi_1$ is a temporal logic formula, it is reasonable to assume that during online interaction,  P2 tries to infer the next subgoal in the temporal sequence. Next, we describe a change detection-based subgoal inference algorithm.

We denote the set of possible subgoals to be $G\subset S_1$--a subset of P1's states. We assume that $G$ is a common knowledge and define a set of atomic propositions $\{ p_{g}\mid g\in G\}$. For each $g\in G$, proposition $p_g$ evaluates true at state $s\in S$ when P1 has reached the subgoal state $g$. 

\begin{definition}[P2's hypothesis space]
  Given a set of possible subgoals $G$ for P2, the hypothesis space
  for P2 is ${\cal X} = \{ \varphi_{safe}\until p_g \mid g \in G\}
  $. for each hypothesis $x \coloneqq \varphi_{safe}\until p_g $ ,
  P2's perceptual game is defined by
  \[
    \game (x) = \langle TS, x, \neg x\rangle
    \]
    where P1's task formula is given by $x$ and the game is zero-sum.
  \end{definition}

For simple goal-reaching objective, the optimal strategy for both players can be solved via the solution of the following Markov game:
\[
\langle S, A, \bar P, U_x\rangle
\]
where $S, A $ is defined exactly as these in the transition system
$TS$.  The transition function $\bar P$ is the same as the transition
function $P$ of $TS$ except that in $\bar P$, a state
$s \models (\neg \varphi_{safe}\lor  p_g) $ is made absorbing.
The newly introduced component is a payoff function
$U_x: S\rightarrow [0,1]$ is defined by
\[
U_x(s,a)= \Expect_{s'}\mathbf{1}(s' \models p_g).
\]
That is, the payoff of a state-action pair is given by the probability of P1 reaching his subgoal in one step. P2's payoff is the negation of P1's payoff given the zero-sum property.

Based on the assumption that P2's boundedly rational, we employ the \ac{ch} model of games to solve, the level-$k$ strategy  $\pi_2^{(k)}(x)$ for P2 and level $k-1$ strategy   $\pi_1^{(k-1)}(x)$ for P1, for each game $\game(x)$, $x\in \cal X$. Next, we describe how P2 uses the pairs $\{\langle \pi_1^{(k-1)}(x),\pi_2^{(k)}(x)\rangle  x\in \cal X\}$ of strategies to evolve her perceptual game.


\paragraph*{Sliding-window change detection for subgoal inference} We
index the set of games $\{\game(x)\mid x\in \cal X\} $ for clarify.
For each subgoal $x_\ell $, let $M_\ell$ be the \ac{mc} induced from
the stochastic transition system by P2's prediction of P1's strategy
and P2's counter-strategy in the Markov game.

% todo: describe the sliding window inference at high-level.
To detect a change in P1's subgoal as early as possible, we assume
that P2 employs an online change detection algorithm--sliding window
change detection based on the \ac{cusum}
statistic~\cite{basseville1993detection}. Given a data in forms of a
history (joint state-action sequence) and a nominal model (a Markov
chain), the sliding window uses a sequence of history over a time
window and detects if a change has occurred in the model that
generates the data during this time window. Next, we describe the
algorithm in more details.

For each hypothesis $M_\ell$ and a nominal model $M_0$, the algorithm computes the log-likelihood ratio,
\begin{align}
S_k^\ell =\sum_{i=1}^k s_i^\ell,
\end{align}
where $s_i^\ell= \ln \frac{P_\ell(y_i)}{P_0(y_i)}$, $y_i$ is the
$i$-th observation of the transitions \emph{within the sliding window
  size} and $P_\ell(y_i)$ (resp. $P_0(y_i)$) is the probability of
observing the transition in the model $M_\ell$ (resp. $M_0$). For
example, given a history $\rho= \vs_0\va_0\vs_1\ldots \vs_n$, and a
sliding window from $[k, k+m]$ with size $m+1$, the history within
this sliding window is
$\vs_{k}\va_k \ldots \vs_{k+m}\va_{k+m}\vs_{k+m+1}$ and
$y_i=(\vs_{k+i}, \va_{k+i})$ is the $i$-th observation within the
window.
%\todo[inline]{Do we take $s_{k+1+i}$ into consideration. If we take that into consideration, we will take the system dynamics into consideration. If we do not take that into consideration, we only consider the decision of agent at state $s_{k+i}$--- feel free to change this according to your implementation. I am ok with dropping $s_{k+i+1}$.} 

Based on the definition, the log likelihood ratio shows a negative
drift before a change and a positive drift after the change. Thus, the
relative information for change detection lies in the difference
between the log likelihood ratio and its current minimum value. The
CUSUM score is given by
\begin{align}
    Z_k^\ell  = S_k^\ell - \min_{1\le j\le k} S_j^\ell.
\end{align}

Recursively, the CUSUM score is computed for each hypothesis $x_\ell$
as
\begin{align}
Z_k^\ell = \max\{0, Z_{k-1}^\ell + \ln \frac{P_\ell(y_k)}{P_0(y_k)} \},
\end{align}
where $Z_0^\ell= 0$.


A change is detected at time $t$ when the score of at least one model,
say $M_\ell$, exceeds a threshold $h>0$.
\[
t= \min\{ k:  \exists x_\ell \in {\cal X},\; Z_k^\ell \ge h\}.
\]
Once a change is detected, the algorithm sets the nominal model to be
the current predicted model, disregards the history until the
change, and keeps running the online change detection given new
observation from the change point onwards. In the case when multiple
models has similar CUSUM scores, we select one model based on
some domain-specific heuristics or at uniformly random.
\begin{remark}
  Here, we described the change detection assuming boundedly
  rationality of P2 with level-$k$ learned by P1 from historical
  interactions. However, this change detection does not restrict to
  boundedly rational players. If P2 were rational, the equilibrium of
  the Markov game $\game(x)$ for each $x\in \cal X$ would be solved
  and used for subgoal inference.
  \end{remark}
 



==> Archived/defs.tex <==
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% based on defs.tex by S. Boyd
% modified by Jie Fu
\newif\ifuseboldmathops
\newif\ifuseittextabbrevs
\useboldmathopstrue   % comment out to use mathbb
%\useittextabbrevstrue % comment out to use non-italic text abbrevs like e.g.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% text abbrevs
\ifuseittextabbrevs
	\newcommand{\cf}{{\it cf.}}
	\newcommand{\eg}{{\it e.g.}}
	\newcommand{\ie}{{\it i.e.}}
	\newcommand{\etc}{{\it etc.}}
	\newcommand{\etal}{{et~al.}}
\else
	\newcommand{\cf}{cf.}
	\newcommand{\eg}{e.g.}
	\newcommand{\ie}{i.e.~}
	\newcommand{\etc}{etc.}
	\newcommand{\etal}{et~al.}
\fi

% standard math sets
\ifuseboldmathops
	%\newcommand{\reals}{{\mbox{\bf R}}}
	\newcommand{\reals}{\mathbf{R}}
	\newcommand{\integers}{\mathbf{Z}}
	\newcommand{\complex}{\mathbf{C}}
	\newcommand{\symm}{\mathbf{S}}  % symmetric matrices
\else
	\newcommand{\reals}{\mathbb{R}}
	\newcommand{\integers}{\mathbb{Z}}
	\newcommand{\complex}{\mathbb{C}}
	\newcommand{\symm}{\mathbb{S}}  % symmetric matrices
\fi

% control theory sets
\ifuseboldmathops
	\newcommand{\HH}{\mathbf{H}}
	\newcommand{\LL}{\mathbf{L}}
\else
	\newcommand{\HH}{\mathbb{H}}
	\newcommand{\LL}{\mathbb{L}}
\fi

% probability operators
\ifuseboldmathops
	\newcommand{\Expect}{\mathop{\bf E{}}\nolimits}
	\newcommand{\Prob}{\mathop{\bf P{}}\nolimits}
\else
	\newcommand{\Expect}{\mathop{\mathbb{E}{}}\nolimits}
	\newcommand{\Prob}{\mathop{\mathbb{P}{}}\nolimits}
\fi

% convex operators
\ifuseboldmathops
	\renewcommand{\Re}{\mathop{\bf Re}}
	\renewcommand{\Im}{\mathop{\bf Im}}
	
	\newcommand{\prox}{\mathop{\bf prox}} % proximal operator
	\newcommand{\dom}{\mathop{\bf dom}}   % domain
	\newcommand{\aff}{\mathop{\bf aff}}   % affine hull
	\newcommand{\cl}{\mathop{\bf cl}}     % closure
	\newcommand{\intr}{\mathop{\bf int}}  % interior
	\newcommand{\Co}{\mathop{\bf Co}}     % convex hull
	\newcommand{\relint}{\mathop{\bf rel int}} % relative interior
	\newcommand{\bd}{\mathop{\bf bd}}     % boundary
	
	\newcommand{\Tr}{\mathop{\bf Tr}}
	\newcommand{\diag}{\mathop{\bf diag}}
\else
	\renewcommand{\Re}{\mathop{\mathrm{Re}}}
	\renewcommand{\Im}{\mathop{\mathrm{Im}}}
	
	\newcommand{\prox}{\mathop{\mathrm{prox}}} % proximal operator
	\newcommand{\dom}{\mathop{\mathrm{dom}}}   % domain
	\newcommand{\aff}{\mathop{\mathrm{aff}}}   % affine hull
	\newcommand{\cl}{\mathop{\mathrm{cl}}}     % closure
	\newcommand{\intr}{\mathop{\mathrm{int}}}  % interior
	\newcommand{\Co}{\mathop{\mathrm{Co}}}     % convex hull
	\newcommand{\relint}{\mathop{\mathrm{rel int}}} % relative interior
	\newcommand{\bd}{\mathop{\mathrm{bd}}}     % boundary
	
	\newcommand{\Tr}{\mathop{\mathrm{Tr}}}     % trace
	\newcommand{\diag}{\mathop{\mathrm{diag}}} % diagonal matrix
\fi

% useful non-bold operators
\newcommand{\eqbydef}{\mathrel{\stackrel{\Delta}{=}}}
\newcommand{\eqbyset}{\mathrel{\stackrel{\mathrm{set}}{=}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}

% lin alg stuff
\newcommand{\Span}{\mathop{\mathrm{span}}}
\newcommand{\Range}{\mathop{\mathrm{range}}}
\newcommand{\Null}{\mathop{\mathrm{null}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}

\newcommand{\ones}{\mathbf 1}
\newcommand{\lambdamax}{{\lambda_{\rm max}}}
\newcommand{\lambdamin}{{\lambda_{\rm min}}}
\newcommand{\sigmamax}{{\sigma_{\rm max}}}
\newcommand{\sigmamin}{{\sigma_{\rm min}}}

% linear temporal logic 
% from Baier, Katoen
\newcommand{\truev}{\mathsf{true}}

\newcommand{\falsev}{\mathsf{false}}
\newcommand{\Always}{\Box \, }
\newcommand{\Eventually}{\Diamond \, }
\newcommand{\Next}{\bigcirc \, }
\newcommand{\until}{\mbox{$\, {\sf U}\,$}}
\newcommand{\R}{\mbox{$\, {\sf R}\,$}}
\newcommand{\Unless}{\mbox{$\, {\sf W}\,$}}
\newcommand{\Model}{{\cal K}}


% \newcommand{\Eventually}{\mbox{$\tilde{{\sf F}} \, $}}
% \newcommand{\Untils}{\mbox{$\, \tilde{{\sf U}}\,$}}
% \newcommand{\Alwaysp}{\mbox{${\sf G}^{{-}1} \, $}}
% \newcommand{\Everp}{\mbox{${\sf F}^{{-}1} \, $}}
% \newcommand{\Nextp}{\mbox{${\sf X}^{{-}1} \, $}}


\newcommand{\G}{\Always}
\newcommand{\U}{\Until}
\newcommand{\WU}{\mbox{$\, {\sf W}\,$}}
\newcommand{\Release}{\mbox{$\, {\sf R}\,$}}
\newcommand{\X}{\Next}
%\newcommand{\V}{\mbox{$\, \overline{{\sf U}} \,$}}
\newcommand{\Lagrange}{\mathcal{L}}

%\newcommand{\Always}{\Box \, }
 %\newcommand{\Eventually}{\Diamond \, }
% \newcommand{\Next}{\bigcirc \, }
\newcommand{\sink}{\mathsf{sink} }

%\newcommand{\Next}{\kern0.5ex\vcenter{\hbox{$\scriptstyle\bigcirc$}}\kern0.5ex}
\newcommand{\BoolTrue}{\mbox{\sf true}}
\newcommand{\BoolFalse}{\mbox{\sf false}}
\newcommand{\agg}{\mathcal{A}}
\newcommand{\normal}[1]{\mathcal{N}\left(#1\right)}


\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\grid}[1]{\left[#1\right]}

\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\card}[1]{\mathsf{card}(#1)}

\newcommand{\stateof}[1]{\llbracket#1\rrbracket}

\newcommand{\prob}{\mbox{Prob}}
\newcommand{\update}{\eta}

\newcommand{\supp}{\mbox{Supp}}


\newcommand{\labelcost}{\mbox{goal}}
\newcommand{\bigO}{\mathbb{O}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calAP}{\mathcal{AP}}

\newcommand{\fac}{\mathsf{fac}}

\newcommand{\calD}{\mathcal{D}}



\newcommand{\init}{\mathsf{Init}}
\newcommand{\final}{\mathsf{Final}}
\newcommand{\suff}{\mathsf{Suff}}
\newcommand{\last}{\mathsf{Last}}
\newcommand{\semi}{\mathsf{semi}}
\newcommand{\occ}{\mathsf{Occ}}



\newcommand{\guard}{\mathsf{Guard}}
\newcommand{\task}{\mathcal{T}}

\newcommand{\val}{\mathcal{V}}
\newcommand{\prog}{\mathsf{Prog}}



\newcommand{\avoid}{\mathfrak{O}}
\newcommand{\cost}{\mathcal{C}}
\newcommand{\softmax}{\mbox{softmax}}
\newcommand{\softmin}{\mbox{softmin}}

\newcommand{\softidx}{\mbox{softidx}}
\newcommand{\indicator}{\mathbf{1}}

\renewcommand{\vec}[1]{\mathbf{#1}}

\newcommand{\inside}[1]{\llbracket
{#1} \rrbracket
}

\newcommand{\idx}{\mathbf{\eta}}

\newcommand{\nat}{\mathbb{Z}}

\newcommand{\weight}{\mathbf{w}}
\newcommand{\prodInit}{\hat{\mu}} 
\newcommand{\prodP}{\hat{P}} 
\newcommand{\option}{\mathsf{O}} 

\newcommand{\path}{\mathsf{Path}} 
\newcommand{\win}{\mathsf{Win}} 

% acronym

\acrodef{mdp}[MDP]{Markov Decision Process}
\acrodef{pomdp}[POMDP]{Partially Observable Markov Decision Process}
\acrodef{ltl}[LTL]{Linear Temporal Logic}
\acrodef{dfa}[DFA]{Deterministic Finite Automaton}


%%% define the theorem environment

\theoremstyle{definition}
 \newtheorem{definition}{Definition}
 \newtheorem{example}{Example}
\newtheorem{problem}{Problem}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{theorem}{Theorem}



\newcommand{\goal}{\mathfrak{g}}

\newcommand{\goals}{\mathsf{G}}
\newcommand{\reach}{\mbox{Reach}}
\newcommand{\caught}{\mbox{Caught}}
\newcommand{\unsafe}{\mbox{Unsafe}}
\newcommand{\hgame}{\mathcal{HG}}


\newcommand{\alg}{\mathsf{ALG}}
%% new operators for game solution
\newcommand{\pre}{\mathsf{Pre}}
\newcommand{\apre}{\mathsf{Apre}}

\newcommand{\vS}{S}

\newcommand{\vA}{\mathsf{A}}
\newcommand{\vP}{\mathsf{P}}

% symbol for automaton
\newcommand{\calA}{\mathcal{A}}
% symbol for the game
\newcommand{\game}{\mathcal{G}}

\newcommand{\games}{\mathsf{GSEQ}}



\newcommand{\vs}{s}
\newcommand{\va}{a}
\newcommand{\vtheta}{\vartheta}

\newcommand{\know}{\vS^{(k)}}

\newcommand{\knows}{\mathcal{K}}

%%% define acronym
\acrodef{smdp}[Semi-MDP]{Semi-Markov decision process}
\acrodef{mcts}[MCTS]{Monte Carlo tree search}
\acrodef{uct}[UCT]{Upper Confidence Bound 1 applied to trees}
\acrodef{scltl}[scLTL]{syntactically co-safe LTL}
\acrodef{ssp}[SSP]{Stochastic Shortest Path}
\acrodef{p2sg}[SG(2)]{Two-player Stochastic Game}
\acrodef{mc}[MC]{Markov chain}
\acrodef{ch}[CH]{Cognitive Hierarchy}

\acrodef{cusum}[CUSUM]{Cumulative SUM}

% introduce belief reach-unsafe states in belief mdp
\newcommand{\reachBeliefMDP}{\bar{\mathcal{F}}} % in math environment.
\newcommand{\unsafeBeliefMDP}{\bar{\mathcal{O}}}
\newcommand{\dist}{\mathcal{D}}
\newcommand{\level}{\mathsf{level}}


==> Archived/detection.tex <==
\color{blue}
The correctness of P1's \ac{bsr} strategy hinges on the correctness in the modeling of P2's inference and  predicted P2's \ac{bsr} strategy.
In this section, we develop a detection method to identify the inconsistency between the actual behavior of P2 observed during online interaction and P1's model of P2's behavior used in the \ac{mdp} $\tilde {\cal H}$. If the method identifies the inconsistency, then it alerts P1 that the deceptive policy $\tilde{\pi}^\ast_{1}(\tilde{\cal H})$ may not be effective.


Given P1's  strategy $\tilde{\pi}^\ast_{1}$, we induces, from the \ac{mdp} $\tilde {\cal H}$,  a Markov chain $\{\tilde{V}^1_t, t\ge 0\}$, where $\tilde{V}^1_t$ is a random variable representing the state visited in $\tilde{\cal H}$ at time $t$. The transition probability matrix $P^1: \tilde V\rightarrow \dist(\tilde V)$ is given by 
\[
P^1(\tilde{v}' \mid \tilde{v}) = \sum_{a_1 \in A_1} \tilde{\pi}^\ast_1(\tilde{\cal H})(\tilde{v}, a_1)\tilde{\Delta}(\tilde{v}' \mid \tilde{v}, a_1).
\]


The online interaction is conducted as follows: Both players start with the initial state $s_0$, then players simultaneously select a pair of action $(a_1,a_2) \in A$, where $a_1$ is determined by $\tilde{\pi}_1^\ast$ and $a_2$ is determined by P2. After the selection, they move to a next state, and the interaction goes on. The interaction ends when a sink state in $\tilde H$ is visited, or an inconsistency in P2's behavior is identified by the detection method. In this interaction, we assume P1 and P2 have the full observation on player's states and actions. This online interaction can generate a length $n+1$ state-action sequence, denoted by $h = s_0 a_0 s_1 a_1 \ldots s_n \in \prefplays$ for some $n\ge 0$. By employing the \ac{dfa} $\calA$ corresponding to P1's \ac{ltl} specification $\varphi_1$ and the inference function $\eta$ in the \ac{mdp} $\tilde{\cal H}$, we can transform the history $h$ to an augmented state-action sequence denoted by $\rho = \tilde{v}_0 a_0\tilde{v}_1a_1\ldots\tilde{v}_n$, where $\tilde{v}_i = (s_i, [\![h_i]\!]_i, q_i, x_i)$ and $\tilde{v}_{i+1} = (s_{i+1}, [\![h_{i+1}]\!]_{x_{i+1}}, q_{i+1}, x_{i+1})$, $q_{i+1} = \delta(q_i, L(s_{i+1}))$, $h_{i+1} = h_i a_i s_{i+1}$, $x_{i+1} = \eta(x_i, h_{i+1})$. It is worth noting that for an unique history $h$, there exists an unique augmented state-action sequence $\rho$ as the transitions in the \ac{dfa} and inference functions are deterministic, and the entire history up to step $i+1$ is used to compute the  $(\eta, x_{i+1})-$equivalent histories at step $i+1$. 


The sequence of augmented state-action $\rho$ is a realization of a stochastic process $\{\tilde{V}^2_t, t\ge 0\}$, where $\tilde{V}^2_t$ is a random variable representing the state visited in $\tilde{\cal H}$ at time $t$. Underlying this stochastic process, there is another probability matrix $P^2$, where $P^2$ is induced from $\tilde{\Delta}$ by P1's strategy and P2's actual behavior. 
To detect the mismatch in P2's model, the problem is equivalent to test the hypothesis: $H_0: P^1= P^2$. 

\todo[inline]{Read this: https://www.stat.washington.edu/jaw/RESEARCH/TALKS/pjb3.pdf to complete later}.

\normalcolor




==> Archived/detection_identity.tex <==
\color{red}
Question: detection using estimated policy is the same as detection using the state transitions?

Given a hypergame ${\cal H} = \langle V, \vA, \Delta, (s_0, h_0, q_0, x_0),  {\cal F}  \rangle$, every state $(s, h, q, x) \in V$, any P1's policy $\pi_1$, and any P2' policy $\pi_2$, where we assume P2 acts based on $x$ and $s$ only, we can induce the a stochastic process $\{V_t, t\ge 0\}$


Essentially, given a augmented state-action sequence $\rho = \Tilde{v}_0 \vec{a}_0 \Tilde{v}_1 \vec{a}_1 \ldots \Tilde{v}_n$ is sampled from the stochastic process $\{V_t, t\ge 0\}$, the probability of this augmented state-action sequence is follows:
\begin{align*}
    P(\rho) = \prod_{t=0}^{n-1} \Delta(v_{t+1} \mid v_t, \vec{a}_t) \pi_1(a_{1, t} \mid v_t) \pi_2(a_{2,t} \mid s_t, x_t)
\end{align*}
where
\begin{align*}
    \Delta(v_{t+1} \mid v_{t}, \vec{a}_t) = P(s_{t+1} \mid s_t,\vec{a}_t)\indicator(\delta(q_t, L(s_{t+1})) = q_{t+1}) \indicator(\eta(x_t, h_t \vec{a}_t s_{t+1}) = x_{t+1})
\end{align*}
where $\indicator(E)$ is the indicator function that returns $1$ if the statement $E$ is true, and $0$ otherwise, $h_{t+1} = h_t \vec{a}_t s_{t+1}$. 

Since we can also write the probability of the augmented state-action sequence as follows:
\begin{align*}
    P(\rho)  = \prod_{t=0}^{n-1} P(v_{t}, \vec{a}_t, v_{t+1})
\end{align*}
implies
\begin{align}
    \prod_{t=0}^{n-1} P(v_{t}, \vec{a}_t, v_{t+1})
    &= \prod_{t=0}^{n-1} \Delta(v_{t+1} \mid v_t, \vec{a}_t) \pi_1(a_{1, t} \mid v_t) \pi_2(a_{2,t} \mid s_t, x_t)
    \label{eq:3}
\end{align}

\section{blue method}
If we only estimate on the action sequences.
We let
\begin{align*}
    P(v_{t+1} \mid v_t, \vec{a}_{2,t}) = \Delta(v_{t+1} \mid v_t, \vec{a}_t) \pi_1(a_{1, t} \mid v_t)
\end{align*}

If the $\pi_1$ is deterministic, meaning $\pi_1$ becomes a Dirac delta function, then we can rewrite $\pi_{1}$ as a mapping $U: V \rightarrow A$, and the probability of this augmented state-action sequence is as follows:
\begin{align}
    P(v_{t+1} \mid v_t, \vec{a}_{2,t}) = \Delta(v_{t+1} \mid v_t, \vec{a}_t) \indicator(U(v_t) =a_{1, t})
\label{eq:4}
\end{align}
Further, if the two-player transition system is deterministic, meaning $P(s' \mid s, (a_1, a_2))$ is a Dirac delta function, then we can rewrite $P(s' \mid s, (a_1, a_2))$ as a mapping T: $S \times A \rightarrow S$, and the probability of this augmented state-action sequence can be written as follows:
\begin{align}
    \Delta(v_{t+1} \mid v_t, \vec{a}_t) = \indicator(T(s_t,\vec{a}_t) = s_{t+1})\indicator(\delta(q_t, L(s_{t+1})) = q_{t+1}) \indicator(\eta(x_t, h_t \vec{a}_t s_{t+1}) = x_{t+1})
\label{eq:5}
\end{align}

Then if we plug Equation~\ref{eq:4} and Equation~\ref{eq:5} back to Equation~\ref{eq:3}, then we get 
\begin{align}
    &\prod_{t=0}^{n-1} P(v_{t}, \vec{a}_t, v_{t+1}) \\
    &= \prod_{t=0}^{n-1} \indicator(T(s_t,\vec{a}_t) = s_{t+1})\indicator(\delta(q_t, L(s_{t+1})) = q_{t+1}) \indicator(\eta(x_t, h_t \vec{a}_t s_{t+1}) = x_{t+1}) \indicator(U(v_t) =a_{1, t}) \pi_2(a_{2,t} \mid s_t, x_t)
\label{eq:6}
\end{align}

From Eq.~\ref{eq:6}, we can see that only estimating on the actions sequences does not reflect the likelihood of augmented state sequence $\rho$, but it is correct under the following conditions:
\begin{enumerate}
    \item Two-player transition system is deterministic.
    \item The inference function is a deterministic, which already is in our case.
    \item The P1's policy is deterministic.
    \item There is an exception, if you take the likelihood ratio test, the $P(v_{t+1} \mid v_{t}, \vec{a}_{t})$ will be canceled when there is a difference between policies for P2.
\end{enumerate}
Conclusion: Blue method is correct for dectecting the mismatch.

\section{red method}
If we estimate the transition probability between states, we have the following:
\begin{align}
    \prod_{t=0}^{n-1} P(v_{t}, v_{t+1}) = \prod_{t=0}^{n-1} \sum_{\vec{a_{t}}} P(v_{t}, \vec{a}_t, v_{t+1})
    &= \prod_{t=0}^{n-1} \sum_{a_t} \Delta(v_{t+1} \mid v_t, \vec{a}_t) \pi_1(a_{1, t} \mid v_t) \pi_2(a_{2,t} \mid s_t, x_t)
\end{align}
If we plug in $\Delta(v_{t+1} \mid v_{t}, \vec{a}_t) = P(s_{t+1} \mid s_t,\vec{a}_t)\indicator(\delta(q_t, L(s_{t+1})) = q_{t+1}) \indicator(\eta(x_t, h_t \vec{a}_t s_{t+1}) = x_{t+1})$, then we have
\begin{align}
    &\prod_{t=0}^{n-1} P(v_{t}, v_{t+1})  \\
    &= \prod_{t=0}^{n-1} \sum_{a_t} P(s_{t+1} \mid s_t,\vec{a}_t)\indicator(\delta(q_t, L(s_{t+1})) = q_{t+1}) \indicator(\eta(x_t, h_t \vec{a}_t s_{t+1}) = x_{t+1}) \pi_1(a_{1, t} \mid v_t) \pi_2(a_{2,t} \mid s_t, x_t)
    \label{eq:10}
\end{align}
From Eq.~\ref{eq:10}, we can see that estimating on the transitions between states does not reflect the likelihood of the given sequence of the augmented state-action pairs, it is only correct under the following conditions:
\begin{enumerate}
    \item The inference function is deterministic, which already is in our case.
    \item P1 and P2's policies are deterministic.
\end{enumerate}

Compare Eq~\ref{eq:3} and Eq.~\ref{eq:10}, we see that these two methods are only the same under the following conditions:
\begin{enumerate}
    \item Only if P1 and P2's policies are deterministic, then the summation can be removed. 
\end{enumerate}

\normalcolor


==> Archived/general-hypergame-formulation.tex <==
We choose to model a game under information asymmetry as a hypergame \cite{}. A hypergame model can capture both the misperception of P2 about P1's objective, and the awareness of P1 that the P2 is misperceiving his objective. 


In \cite{}, a hypergame model of level-1 is defined as ${\cal H}^1 = \langle \game_1, \game_2 \rangle$, where $\game_1$ is the game on graph as constructed by P1 given his objective $\varphi_1$ and $\game_2$ is the game on graph as constructed by P2 given his objective $\varphi_2$. When P1 is aware that P2 is misperceiving his objective but P2 is not aware of her misperception, the resulting hypergame is said to be of level-2, and is defined as ${\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle$. In a level-2 hypergame, P1 computes his strategy by solving the level-1 hypergame, while P2 computes his strategy by solving the game on graph $\game_2$. 


The above hypergame model from \cite{} does not account for evolving misperception in the game. When P2 is equipped with an inference mechanism, her misperception evolves and so does her strategy. One way to understand P2's evolving misperception and its effect on her strategy is the following. Let $\mathsf{LTL}$ be the range of P2's inference mechanism $\eta$. Then, for every \ac{ltl} formula $\Psi \in \mathsf{LTL}$, P2 will construct a game on graph $\game(\Psi)$ in which P2's objective is to satisfy $\varphi_2 = \neg \Psi$. In general, given a finite set of atomic propositions $AP$, the set $\mathsf{LTL}$ is infinite. However, in this paper, we study the case where $\mathsf{LTL}$ is finite. 


\begin{assumption}
Let $\mathsf{LTL}$ denote a finite subset of \ac{ltl} specifications that can be defined using a finite set of atomic propositions, $AP$.
\end{assumption}


Let the specifications in $\mathsf{LTL}$ be denoted by $\Psi_i$ for $i = 1, 2, \ldots, N$. Then at some state $s \in {\cal S}$, based on her current misperception $\psi_t \in \mathsf{LTL}$, P2 plays the best strategy for her in the game $\game(\psi_t)$. \todo[inline]{ambiguous. best = best according to bounded rational model} To explicitly capture the dependence of hypergames on P2's misperception at time $t$, we define hypergame as follows. 


\begin{definition}[Hypergame]
Given a finite set $\mathsf{LTL}$ of \ac{ltl} specifications, a level-1 hypergame is defined as 
\[
    {\cal H}^1(\psi_t) = \langle \game(\varphi_1), \game(\psi_t)  \rangle
\]
where P1 is playing the game $\game(\varphi_1)$, and P2 is playing the game $\game(\psi_t) \in \{\game(\Psi_1), \game(\Psi_2), \ldots, \game(\Psi_N)\}$. And a level-2 hypergame is given by 
\[
    {\cal H}^2(\psi_t) = \langle {\cal H}^1(\psi_t), \game(\psi_t) \rangle
\]
\end{definition}


% When the domain and the range of inference mechanism $\eta$ (see Def.~\ref{}) of P2 is finite, it is possible to define a game on graph like structure for a level-1 hypergame, which we call a \textit{hypergame on graph}. 


Given the definition of hypergame, we now define a new graph---which we call a ``Hypergame on Graph"---to model the hypergame ${\cal H}^1(\psi_t)$ that P1 uses to compute his winning strategy. 


\begin{definition}[Hypergame on Graph]
Let $TS$ be a transition system and ${\cal A}_1 = \langle Q_1, \Sigma, \delta_1, q_{01}, F_1, Acc_1 \rangle$ be a \ac{dfa} equivalent to the specification $\varphi_1$. Similarly, let ${\cal A}_2^i = \langle Q_2^i, \Sigma, \delta_2^i, q_{02}^i, F_2^i, Acc_2 \rangle$ be a \ac{dfa} equivalent to specification to $\Psi_i$ for $\Psi_i \in \mathsf{LTL}$. Let ${\cal I} = \{1, 2, \ldots, N\}$ be an indicator set over the set $\mathsf{LTL}$. Let ${\cal A} = \langle Q, \Sigma, \delta, q_{0}, F, Acc_2 \rangle$ be the union of ${\cal A}_1$ and all \ac{dfa}s ${\cal A}_2^i$. Then, a hypergame on graph is the tuple \todo[inline]{Define DFA union in preliminaries. }
\[
    {\cal H} = \langle V, Act, \Delta, ({\cal F}_1, Acc_1), ({\cal F}_2, Acc_2) \rangle
\]
where the components of hypergame graph are as follows
\begin{itemize}
    \item $V = S^{\ast} \times Q \times {\cal I}$, where $h \in S^{k}$ is an ordered sequence of $TS$ states of length $k$, $q \in Q$ is the automata state and $i \in \cal I$ is the game that P2 is playing based on her misperception. We shall refer to $h$ as history, and write it as $h = (s_{0}, \ldots, s_k)$. When history is not available for length $k$, the unknown components will be replaced with $\emptyset$. The state $s_k$ represents the current state in $TS$. 
    
    \item $Act$ is the set of actions. 
    
    \item $\Delta: V \times Act \rightarrow \distr(V)$ is a stochastic transition function. A state $(h', q', i') \in V$ is included in $\Delta((h, q, i), a)$ if and only if $s_t' \in \supp(T(s_t, a))$ and $h'[0:k-1] = h[1:k]$ and $q' = \delta(q, L(s_k'))$ and $i' = \eta(\psi_0, h')$, where $\psi_0$ is the initial misperception. In such a case, $\mathbb{P}((h', q', i') \in V \mid (h, q, i) \in V, a \in Act) = \mathbb{P}(s' \in S \mid s \in S, a \in Act)$. 
    
    \item $({\cal F}_1, Acc_1)$ represents the objective for P1. The set ${\cal F}_1$ is defined as $S^k \times F_1 \times {\cal I}$. $Acc_1 \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P1.
    
    \item $({\cal F}_2, Acc_2)$ represents the objective for P2. The set ${\cal F}_2$ is defined as ${\cal F}_2 = \{(h, q, i) \in V \mid h \in S^k \text{ and } q \in F_2^i\}$. $Acc_2 \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P2.
    
    \todo[inline]{Fix notation: $\Delta, \cal F$ are repeated in $\game$ and $\cal H$.}
\end{itemize}
\end{definition}




% \begin{definition}[Hypergame]
% Let $\game_1$ and $\game_2$ be the games on graph as constructed by P1 and P2 in their mind, given P1's objective is to satisfy $\varphi_1$ and P2's objective is to satisfy $\varphi_2$. Then, a \textit{first-level} hypergame is a tuple
% \[
%     {\cal H}^1 = \langle \game_1, \game_2 \rangle.
% \]

% When one player is aware of misperception and other is not, we get a \textit{second-level} hypergame, given by the tuple
% \[
%     {\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle
% \]
% where P1 solves the first-level hypergame to compute his strategy. 
% \end{definition}


% We note that a \textit{second-level} hypergame models the game with information asymmetry described in Problem~\ref{}. We refer the reader to \cite{} for a general treatment of $k$-th level hypergame. 


% A definition of hypergame given in Def.~\ref{} does not account for evolving misperception. 




% % When P1 is aware of P2's misperception, P1 computes his strategy by anticipating the P2's strategy, given her perception $\psi_t$ of P1's objective. In order to anticipate P2's strategy, P1 must first construct a model of his opponent, P2. An opponent model consists of what P1 knows about (a) how P2 perceives P1's objective at $t=0$, (b) how P2 updates her misperception, \ie the inference mechanism of P2, and (c) given the misperception $\psi_t$, how does P2 compute her strategy.



==> Archived/hypergame-19Nov19.tex <==
We choose to model a game under information asymmetry as a hypergame \cite{}. A hypergame model can capture both the misperception of P2 about P1's objective, and the awareness of P1 that the P2 is misperceiving his objective. 


In \cite{}, a hypergame model of level-1 is defined as ${\cal H}^1 = \langle \game_1, \game_2 \rangle$, where $\game_1$ is the game on graph as constructed by P1 given his objective $\varphi_1$ and $\game_2$ is the game on graph as constructed by P2 given his objective $\varphi_2$. When P1 is aware that P2 is misperceiving his objective but P2 is not aware of her misperception, the resulting hypergame is said to be of level-2, and is defined as ${\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle$. In a level-2 hypergame, P1 computes his strategy by solving the level-1 hypergame, while P2 computes his strategy by solving the game on graph $\game_2$. 


The above hypergame model from \cite{} does not account for evolving misperception in the game. When P2 is equipped with an inference mechanism, her misperception evolves and so does her strategy. One way to understand P2's evolving misperception and its effect on her strategy is the following. Let $\mathsf{LTL}$ be the range of P2's inference mechanism $\eta$. Then, for every \ac{ltl} formula $\Psi \in \mathsf{LTL}$, P2 will construct a game on graph $\game(\Psi)$ in which P2's objective is to satisfy $\varphi_2 = \neg \Psi$. In general, given a finite set of atomic propositions $AP$, the set $\mathsf{LTL}$ is infinite. However, in this paper, we study the case where $\mathsf{LTL}$ is finite. 


\begin{assumption}
Let $\mathsf{LTL}$ denote a finite subset of \ac{ltl} specifications that can be defined using a finite set of atomic propositions, $AP$.
\end{assumption}


Let the specifications in $\mathsf{LTL}$ be denoted by $\Psi_i$ for $i = 1, 2, \ldots, N$. Then at some state $s \in {\cal S}$, based on her current misperception $\psi_t \in \mathsf{LTL}$, P2 plays the best strategy for her in the game $\game(\psi_t)$. \todo[inline]{ambiguous. best = best according to bounded rational model} To explicitly capture the dependence of hypergames on P2's misperception at time $t$, we define hypergame as follows. 


\begin{definition}[Hypergame]
Given a finite set $\mathsf{LTL}$ of \ac{ltl} specifications, a level-1 hypergame is defined as 
\[
    {\cal H}^1(\psi_t) = \langle \game(\varphi_1), \game(\psi_t)  \rangle
\]
where P1 is playing the game $\game(\varphi_1)$, and P2 is playing the game $\game(\psi_t) \in \{\game(\Psi_1), \game(\Psi_2), \ldots, \game(\Psi_N)\}$. And a level-2 hypergame is given by 
\[
    {\cal H}^2(\psi_t) = \langle {\cal H}^1(\psi_t), \game(\psi_t) \rangle
\]
\end{definition}


% When the domain and the range of inference mechanism $\eta$ (see Def.~\ref{}) of P2 is finite, it is possible to define a game on graph like structure for a level-1 hypergame, which we call a \textit{hypergame on graph}. 


Given the definition of hypergame, we now define a new graph---which we call a ``Hypergame on Graph"---to model the hypergame ${\cal H}^1(\psi_t)$ that P1 uses to compute his winning strategy. 


\begin{definition}[Hypergame on Graph]
Let $TS$ be a transition system and ${\cal A}_1 = \langle Q_1, \Sigma, \delta_1, q_{01}, F_1, Acc_1 \rangle$ be a \ac{dfa} equivalent to the specification $\varphi_1$. Similarly, let ${\cal A}_2^i = \langle Q_2^i, \Sigma, \delta_2^i, q_{02}^i, F_2^i, Acc_2 \rangle$ be a \ac{dfa} equivalent to specification to $\Psi_i$ for $\Psi_i \in \mathsf{LTL}$. Let ${\cal I} = \{1, 2, \ldots, N\}$ be an indicator set over the set $\mathsf{LTL}$. Let ${\cal A} = \langle Q, \Sigma, \delta, q_{0}, F, Acc_2 \rangle$ be the union of ${\cal A}_1$ and all \ac{dfa}s ${\cal A}_2^i$. Then, a hypergame on graph is the tuple \todo[inline]{Define DFA union in preliminaries. }
\[
    {\cal H} = \langle V, Act, \Delta, ({\cal F}_1, Acc_1), ({\cal F}_2, Acc_2) \rangle
\]
where the components of hypergame graph are as follows
\begin{itemize}
    \item $V = S^{\ast} \times Q \times {\cal I}$, where $h \in S^{k}$ is an ordered sequence of $TS$ states of length $k$, $q \in Q$ is the automata state and $i \in \cal I$ is the game that P2 is playing based on her misperception. We shall refer to $h$ as history, and write it as $h = (s_{0}, \ldots, s_k)$. When history is not available for length $k$, the unknown components will be replaced with $\emptyset$. The state $s_k$ represents the current state in $TS$. 
    
    \item $Act$ is the set of actions. 
    
    \item $\Delta: V \times Act \rightarrow \distr(V)$ is a stochastic transition function. A state $(h', q', i') \in V$ is included in $\Delta((h, q, i), a)$ if and only if $s_t' \in \supp(T(s_t, a))$ and $h'[0:k-1] = h[1:k]$ and $q' = \delta(q, L(s_k'))$ and $i' = \eta(\psi_0, h')$, where $\psi_0$ is the initial misperception. In such a case, $\mathbb{P}((h', q', i') \in V \mid (h, q, i) \in V, a \in Act) = \mathbb{P}(s' \in S \mid s \in S, a \in Act)$. 
    
    \item $({\cal F}_1, Acc_1)$ represents the objective for P1. The set ${\cal F}_1$ is defined as $S^k \times F_1 \times {\cal I}$. $Acc_1 \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P1.
    
    \item $({\cal F}_2, Acc_2)$ represents the objective for P2. The set ${\cal F}_2$ is defined as ${\cal F}_2 = \{(h, q, i) \in V \mid h \in S^k \text{ and } q \in F_2^i\}$. $Acc_2 \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P2.
    
    \todo[inline]{Fix notation: $\Delta, \cal F$ are repeated in $\game$ and $\cal H$.}
\end{itemize}
\end{definition}

\todo[inline]{limit the number of switching. using switching game formulation.}

Write about what if $F_2, Acc_2 $ not considered. 


% \begin{definition}[Hypergame]
% Let $\game_1$ and $\game_2$ be the games on graph as constructed by P1 and P2 in their mind, given P1's objective is to satisfy $\varphi_1$ and P2's objective is to satisfy $\varphi_2$. Then, a \textit{first-level} hypergame is a tuple
% \[
%     {\cal H}^1 = \langle \game_1, \game_2 \rangle.
% \]

% When one player is aware of misperception and other is not, we get a \textit{second-level} hypergame, given by the tuple
% \[
%     {\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle
% \]
% where P1 solves the first-level hypergame to compute his strategy. 
% \end{definition}


% We note that a \textit{second-level} hypergame models the game with information asymmetry described in Problem~\ref{}. We refer the reader to \cite{} for a general treatment of $k$-th level hypergame. 


% A definition of hypergame given in Def.~\ref{} does not account for evolving misperception. 




% % When P1 is aware of P2's misperception, P1 computes his strategy by anticipating the P2's strategy, given her perception $\psi_t$ of P1's objective. In order to anticipate P2's strategy, P1 must first construct a model of his opponent, P2. An opponent model consists of what P1 knows about (a) how P2 perceives P1's objective at $t=0$, (b) how P2 updates her misperception, \ie the inference mechanism of P2, and (c) given the misperception $\psi_t$, how does P2 compute her strategy.



==> Archived/new_detection.tex <==

The correctness of P1's \ac{bsr} strategy hinges on the correctness in the modeling of P2's inference and predicted P2's \ac{bsr} strategy. In this section, we develop a detection method to identify the inconsistency between the actual behavior of P2 observed during online interaction and P1's model of P2's behavior used in the \ac{mdp} $\tilde {\cal H}$. If the method identifies the inconsistency, then it alerts P1 that the deceptive policy $\tilde{\pi}^\ast_{1}$ may not be effective.

Consider a finite  history $h = s_0 \vec{a}_0 s_1\vec{a}_1 \ldots s_n$ where $\vec{a}_i = (a_{1,i},a_{2,i}), i=0,\ldots, n-1$ are pairs of actions for P1 and P2, respectively. Under the assumption of complete observations, both players can observe the history $h$. By  employing the \ac{dfa} $\calA$ corresponding to P1's \ac{ltl} specification $\varphi_1$ and the inference function $\eta$ in the \ac{mdp} $\tilde{\cal H}$, we can transform the history $h$ to an augmented state-action sequence denoted by $\rho = \tilde{v}_0 \vec{a}_0\tilde{v}_1\vec{a}_1\ldots\tilde{v}_n$, where $\tilde{v}_i = (s_i, [\![h_i]\!]_i, q_i, x_i)$ and $\tilde{v}_{i+1} = (s_{i+1}, [\![h_{i+1}]\!]_{x_{i+1}}, q_{i+1}, x_{i+1})$, $q_{i+1} = \delta(q_i, L(s_{i+1}))$, $h_{i+1} = h_i \vec{a}_i s_{i+1}$, $x_{i+1} = \eta(x_i, h_{i+1})$. It is worth noting that for a unique history $h$, there exists a unique augmented state-action sequence $\rho$ as the transitions in the \ac{dfa} and inference functions are deterministic, and the entire history up to step $i+1$ is used to compute the $(\eta, x_{i+1})-$equivalent histories at step $i+1$. The detection problem reduces to: Given the hyper game transition system $\cal H$, a predicted inference function for P2 $\eta$ and P2's \ac{bsr} strategies for a set $X$ of hypotheses, how likely is the observation $\rho$ generated by our predicted model of opponent? Where given the observation $\rho$, $\cal H$, any P1's policy $\phi_1$, and any P2's policy $\pi_2$, we have the likelihood of the $\rho$ as the following:
\begin{align*}
    L(\rho  = s_0 \vec{a}_0 s_1 \vec{a}_1 \ldots s_n ) = \prod_{i=0}^{n-1} \Delta(v_{i+1} \mid v_{i}, \vec{a}_{i}) \pi_{1}(a_{1, i} \mid v_i) \pi_{2}(a_{2, i} \mid v_{i})
\end{align*}
where $\Delta$ is the probabilitisc transtion function in the $\cal H$.

The answer to this problem is likelihood ratio test. Given two hypothesis $H_0: $ the data is generated by our predicted model of P2; and $H_1:$ the data is not generated by our prediction, the goal is to test which hypothesis is a good fit for the data. We consider a simpler case and assume our predicted model of inference $\eta$ is correct for P2, and want to test if P2  deviates from the predicted \ac{bsr} strategies. Given the observation $\rho$, $\cal H$, and P1's policy $\pi_1^\ast$, the likelihood of $\rho$ is computed by
\[
L_0 = L(\rho = s_0 \vec{a}_0 s_1 \vec{a}_1 \ldots s_n \mid \pi_2^{B,2}) = \prod_{i=0}^{n-1}P(s_{i+1} \mid s_{i}, \vec{a}_i) \pi_1^\ast(a_{1,i} \mid \tilde{v})\pi_2^{B,2}(a_{2, i} \mid s_i, x_i)
\]
where $s_i=\tilde v_i[1]$ and $x_i  = \tilde v_i[4]$ are the first and last components of $\tilde v_i$. 

At the same time, we obtain an estimate of P2's strategy from history as
\[
  \hat \pi_2 (a_2\mid \tilde v) =\left\{ \begin{array}{ll}
                                      \frac{ \#\indicator( \tilde v, a_2)}{\# 
                                       \indicator(\tilde v)} & \text{ if } {\# 
                                                          \indicator(\tilde v)}\ne 0,\\
                                    \uparrow & \text{ undefined otherwise.}
                                \end{array}\right.
                            \]
                            where $\#\indicator(\tilde v,a_2)$ is the number of
                            times P2 selected action $a_2$ given the
                            current state $\tilde v$, and $\#\indicator(\tilde v)$ is the number of times the state $\tilde v$ is visited. For unseen state-action pairs, we need not to estimate the policy given the pair as it won't be used in the likelihood ratio test.

                            Based on the maximum likelihood estimate of P2's strategy from history, we have
                            \[
                            L_1 =   L( \rho = s_0 \vec{a}_0 s_1 \vec{a}_1 \ldots s_n \mid \hat \pi_2) = \prod_{i=0}^{n-1} P(s_{i+1} \mid s_i, \vec{a}_i) \pi_1^\ast(a_{1, i} \mid \tilde{v})
                            \hat \pi_2(a_{i+1,2}\mid s_i, x_i)
\]
The likelihood ratio is computed as
\[
  \lambda = L_0/L_1.
  \]
  We conduct a likelihood ratio test and
  calculate $\chi^2= -2 \ln \lambda$, which is an approximate Chi-square distribution of $n$ degree of freedom and $k$ is the number of parameters $\{ \tilde \pi_2(a_2\mid \tilde v)\mid\#\indicator(\tilde v,a_2)\ne 0\}$ estimated with maximum likelihood estimate. By selecting a confidence level $\alpha$, we reject the null hypothesis if $\chi^2$ is larger than the Chi-square percentile  with $n$ degree of freedom given the level $\alpha$.

  Given that the sequence of P2's hypothesis $x_i$, $i=0,\ldots, n$ is not observable by P1, we cannot evaluate whether our predicted inference function $\eta$ of P2 is the exact inference function used by P2. To detect the mismatch in both P2's strategies and inference mechanism, we would need to estimate P2's policy from the observed history and compare that with the null hypothesis. As P2 can select finite-memory strategy modeled by a finite-state automaton with unknown structure, the policy cannot be learned from positive data (that is, what P2 does). To learn a finite-state automaton without the structure, both positive data and negative data are required \cite{}.
  
However, learning the true policy of P2 is not our goal. For deception purpose, as long as P2's actual behavior fits our predicted behavior of P2 (null hypothesis $H_0$), we consider the deception is effective.

\begin{remark}
  The detection algorithm monitors P2's behavior during online interaction. However, this likelihood ratio test can easily generalize to multiple histories during repeated interactions. P1 may also use this test to self-validate its model of P2 before carrying out important missions. 
\end{remark}

==> Archived/old_detection.tex <==



\subsection{Detecting the Mismatch for Modeling Opponent}~\label{subsec:detecting_inconsistency}

The correctness of P1's \ac{bsr} strategy hinges on the correctness in the modeling of P2's inference and predicted P2's \ac{bsr} strategy. In this section, we develop a detection method to identify the inconsistency between the actual behavior of P2 observed during online interaction and P1's model of P2's behavior used in the \ac{mdp} $\tilde {\cal H}$. If the method identifies the inconsistency, then it alerts P1 that the deceptive policy $\tilde{\pi}^\ast_{1}(\tilde{\cal H})$ may not be effective.

Given P1's  strategy $\tilde{\pi}^\ast_{1}$, we induces, from the \ac{mdp} $\tilde {\cal H}$,  a Markov chain $\{\tilde{V}^1_t, t\ge 0\}$, where $\tilde{V}^1_t$ is a random variable representing the state visited in $\tilde{\cal H}$ at time $t$. The transition probability matrix $P^1: \tilde V\rightarrow \dist(\tilde V)$ is given by 
\[
P^1(\tilde{v}' \mid \tilde{v}) = \sum_{a_1 \in A_1} \pi^\ast_1(\tilde{\cal H})(\tilde{v}, a_1)\tilde{\Delta}(\tilde{v}' \mid \tilde{v}, a_1).
\]


% We consider a deterministic inference function from Def~\ref{def:inference} used in the \ac{mdp} $\tilde{\cal H}$, \ie, $\eta: X \times \prefplays \rightarrow X$ maps a hypothesis $x\in X$ and a history $h\in \prefplays$ to a new hypothesis $x' = \eta(x, h)$. Moreover, for ease of understanding, we assume for any hypothesis $x \in X$, the set of equivalent history $[\![h]\!]$ is a singleton, \ie, $[\![h]\!] = h, \forall h \in \prefplays$. Given the inference function $\eta$, any hypothesis $x\in X$, and two history $h_1, h_2 \in \prefplays$, where $h_1 \not = h_2$, we have $\eta(x, h_1) \not= \eta(x, h_2)$, \ie, $h_1, h_2$ are not $\eta$-\emph{equivalent}. Our propose detection method can be extended to $\eta$ - \emph{equivalent} case and $(\eta, x)$-\emph{equivalent} case for a given hypothesis $x$.

% During online interaction, P1 observes length $n+1$ states sequence, denoted by $\rho^1 \downharpoonright_S = s_0^1s_1^1\ldots s_n^1$, which is a projection of $\rho^1$ on the states $S$, and $\rho^1$ is a length $n+1$ realization from the stochastic process $\{\tilde V^1_t, t\ge 0\}$. If we do not consider $\eta$ - \emph{equivalent} and $(\eta, x)$-\emph{equivalent}, then we have for any $\rho^1 \downharpoonright_S$ projected from the $\rho^1$, we have one to one map to the realization $\rho^1$.


% During online iteration, P2's actual behavior induces another stochastic process $\{\tilde{V}^2_t, t\ge 0\}$ where $\tilde{V}^2_t$ is a random variable representing the state visited at time $t$ by P2. This stochastic process's length $n+1$ realization is denoted by $\rho^2$, and we denote the projection of $\rho^2$ on the states $s$ as $\rho^2\downharpoonright_S$. When P2 is encountering with P1, we can observe another state sequence $\rho^2\downharpoonright_S = s_0^2s_1^2\ldots s_n^2$. Underlying this stochastic process $\{\tilde{V}^2_t, t\ge 0\}$, there is a transition probability matrix $P^2$ where $P2$ relates to P2's actual behavior, and we can estimate it from a sequence of data.
The online interaction is conducted as follows: Both players start with the initial state $s_0$, then players simultaneously select a pair of action $(a_1,a_2) \in A$, where $a_1$ is determined by $\tilde{\pi}_1^\ast$ and $a_2$ is determined by P2. After the selection, they move to a next state, and the interaction goes on. The interaction ends when a sink state in $\tilde H$ is visited, or an inconsistency in P2's behavior is identified by the detection method. In this interaction, we assume P1 and P2 have the full observation on player's states and actions. This online interaction can generate a length $n+1$ state-action sequence, denoted by $h = s_0 a_0 s_1 a_1 \ldots s_n \in \prefplays$ for some $n\ge 0$. By employing the \ac{dfa} $\calA$ corresponding to P1's \ac{ltl} specification $\varphi_1$ and the inference function $\eta$ in the \ac{mdp} $\tilde{\cal H}$, we can transform the history $h$ to an augmented state-action sequence denoted by $\rho = \tilde{v}_0 a_0\tilde{v}_1a_1\ldots\tilde{v}_n$, where $\tilde{v}_i = (s_i, [\![h_i]\!]_i, q_i, x_i)$ and $\tilde{v}_{i+1} = (s_{i+1}, [\![h_{i+1}]\!]_{x_{i+1}}, q_{i+1}, x_{i+1})$, $q_{i+1} = \delta(q_i, L(s_{i+1}))$, $h_{i+1} = h_i a_i s_{i+1}$, $x_{i+1} = \eta(x_i, h_{i+1})$. It is worth noting that for a unique history $h$, there exists a unique augmented state-action sequence $\rho$ as the transitions in the \ac{dfa} and inference functions are deterministic, and the entire history up to step $i+1$ is used to compute the $(\eta, x_{i+1})-$equivalent histories at step $i+1$. 

The sequence of augmented state-action $\rho$ is a realization of a stochastic process $\{\tilde{V}^2_t, t\ge 0\}$, where $\tilde{V}^2_t$ is a random variable representing the state visited in $\tilde{\cal H}$ at time $t$. Underlying this stochastic process, there is another probability matrix $P^2$, where $P^2$ is induced from $\Delta$ by P1's strategy and P2's actual behavior. \lening{
\[P^2(\tilde{v}' \mid \tilde{v}) = \sum_{a_2 \in A_2}\sum_{a_1 \in A_1} \tilde{\pi}^\ast_1(\tilde{\cal H})(\tilde{v}, a_1) \Delta(\tilde{v}' \mid \tilde{v}, (a_1, a_2)) \pi_2(\tilde{v}, a_2),\]
where $\pi_2$ is P2's actual policy.}
If the stochastic processes $\{\tilde{V}^2_t, t\ge 0\}$ is the same as $\{\tilde{V}^1_t, t\ge 0\}$, then P1's prediction of P2's behavior is correct. 

Given a length $n+1$ augmented sequence of state-action $\rho=\tilde{v}_0 a_0\tilde{v}_1a_1\ldots \tilde{v}_n$ from the online interaction, we can transform the problem of detecting the mismatch  into the following: Is the sequence of augmented states $\rho$ generated by the transition probability matrix $P^1$? We develop Algorithm~\ref{alg:detecting} to detect the mismatch based on \cite{polansky2007detecting}. The key idea of this algorithm is to use the sampled state-action sequence $\rho$ to obtain a Maximum likelihood estimator (MLE) $\bar{P}^2$ of the transition matrix $P^2$ and conduct the likelihood-ratio test. In this section, we assume $\{\tilde{V}_t^1, t\ge 0\}$ and $\{\tilde{V}_t^2, t\ge 0\}$ are independent and identically distributed (i.i.d). Then, by central limit theorem~\cite{}, we can assume that test statistics follows $\chi^2$ distribution. We define a distance measure between $P^1$ and $\bar{P}^2$ using the estimate of $P^2$, essentially we define $\Lambda$ as the log likelihood-ratio between $P^1$ and $\bar{P}^2$ as follows
\begin{align}
    \Lambda = 2 (\sum_{(\tilde{v}, \tilde{v}')}\log ( \bar{P}^2(\tilde{v}' \mid \tilde{v}))-\sum_{(\tilde{v}, \tilde{v}')} \log( P^1(\tilde{v}' \mid \tilde{v}))),
\label{eq:distance}
\end{align}
where $(\tilde{v},\tilde{v}')$ is the visiting state pair in the augmented state-action sequence $\rho = \tilde{v}_0 a_0 \tilde{v}_1 a_1 \ldots \tilde{v}_n$.
Given a significance level $\alpha$ (normally defined by users), we can compute the $1-\alpha$ quantitile $\chi^2_{1-\alpha;c}$, where $c = \abs{\{(\tilde{v}, \tilde{v}')\}}$ and $\chi^2_{1-\alpha;c}$ can be directly computed. Then, the likelihood-ratio test provides the decision rules as follows~\cite{}: if $\Lambda \ge \chi^2_{1-\alpha;c}$, we reject $H_0$; if $ \Lambda \le \chi^2_{1-\alpha;c}$, we do not reject $H_0$. 
\lening{please let me know if more details are needed. }




\begin{algorithm}[!htb]
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE A length $n+1$ state-action sequence $\rho$, P1's optimal policy $\tilde{\pi}^\ast_1$, and the \ac{mdp} $\tilde{\cal H}$.
\ENSURE Boolean value for $P^1 = P^2$.
% \STATE{
% \[P^1(\tilde{v}' \mid \tilde{v}) = \sum_{a_1 \in A_1} \tilde{\pi}^\ast_1(\tilde{\cal H})(\tilde{v}, a_1)\tilde{\Delta}(\tilde{v}' \mid \tilde{v}, a_1).
% \]} \COMMENT{Transition probability matrix $P^1$ of the stochastic process $\{\tilde{V}^1_t, t \ge 0\}$}
% \label{ln:p1}
\STATE{For $\tilde{v} \in \tilde{V}$
\[\Omega(\tilde{v}) = \sum_{t=0}^{n} \indicator(\rho_t = \tilde{v}).\]}
\COMMENT{The number of visitation to $\tilde{v}$ given $\rho$.}
\label{ln:frequency_state}
\STATE{For $(\tilde{v}, \tilde{v}')\in \tilde{V} \times \tilde{V}$
\[\Omega(\tilde{v}, \tilde{v}') = \sum_{t=0}^{n-1}\indicator(\rho_t = s, \rho_{t+1} = \tilde{v}').\]}
\COMMENT{The number of visiting state pair $(\tilde{v}, \tilde{v}')$  given $\rho$.}
\label{ln:frequency_state_pair}
\STATE{
\[
\bar{P}^2(\tilde{v}' \mid \tilde{v}) = \begin{cases}
\Omega(\tilde{v}, \tilde{v}') / \Omega(\tilde{v}), &\text{if } \Omega(\tilde{v}) > 0, \\
\indicator(\tilde{v} = \tilde{v}'), &\text{if } \Omega(\tilde{v}) = 0.
\end{cases}\]} 
%\COMMENT{Maximum likelihood estimator $\bar{P}^2$ for $P^2$, where $P^2$ is from the stochastic process $\{\tilde{V}_t^2, t\ge 0\}$}
\label{ln:estimation}
\STATE{
Calculate $\Lambda$ using \eqref{eq:distance}.
% \begin{align*}
%     \Gamma = 2( \sum_{(\tilde{v}, \tilde{v}') \in \Xi} \Omega(\tilde{v}, \tilde{v}') \log(P^1(\tilde{v} \mid \tilde{v}')) +  \sum_{(\tilde{v}, \tilde{v}') \in \Xi} \Omega(\tilde{v}, \tilde{v}') \log(\bar{P}^2(\tilde{v} \mid \tilde{v}'))).
% \end{align*}
%\COMMENT{An objective function $\Gamma$, a metric on the transition probability matrices.}
%\label{ln:objective}
}
\IF{$\Lambda > \chi^2_{1-\alpha;c}$}\label{ln:if}
\RETURN{Reject $H_0$} \COMMENT{Inconsistency is detected: $\rho$ is not generated by $P^1$.}
\ELSE
\RETURN{Do not reject $H_0$} \COMMENT{Inconsistency is not detected.}
\ENDIF
\end{algorithmic}
\caption{Detect the mismatch in opponent modeling.}
\label{alg:detecting}
\end{algorithm}

% Given the sampled sequences of states $\rho^i\downharpoonright_S$,  we first introduce $\Omega(\tilde{v})$ and $\Omega(\tilde{v}, \tilde{v}')$ to denote the frequencies of state $\tilde{v}$ and state pair $(\tilde{v}, \tilde{v}')$ in the given sampled sequence of states $h$. We can directly compute $\Omega(\tilde{v})$ and $\Omega(\tilde{v}, \tilde{v}')$ for each state $\tilde{v}$ and state pair $(\tilde{v}, \tilde{v}')$ from $h \downharpoonright_S$ in the Algorithm~\ref{alg:detecting} line~\ref{ln:frequency_state} and line~\ref{ln:frequency_state_pair}, for both visited and unvisited states, where $\indicator(E)$ is the indicator function that returns $1$ if the statement $E$ is true, and $0$ otherwise. We can approximate the transition matrix $P$ associated to stochastic process $\{\tilde{V}^i_t, t\ge 0\}$ by a maximum likelihood estimator denoted by $\bar{P}^{i}$ from sampled $h^i$ in line~\ref{ln:estimation}.
% Recall that there is a one to one map from the $\rho^1$ to observed states $\rho^1\downharpoonright_S$, for player 1, given the optimal deceptive policy $\pi_1^\ast(\tilde{\cal H})$ and the \ac{mdp} $\tilde{\cal H}$, we can induce the $P^1$ from the $\tilde{\Delta}$ directly in line~\ref{ln:}. For simplicity of the notation, we use $P\bar{P}^1$ instead of $P$ We introduce $\Omega(s, s')$ to denote the frequencies of the state pair $(s, s')$ and estimate it from the observed states $\rho^1 \downharpoonright_S$ in line~\ref{}. For player 2, due to unknown model employed by P2, given $\rho^2 \downharpoonright_S $ we can estimate the frequencies of state $s$ denoted by $\Omega(s)$ and state pair $(s, s')$ $\Omega(s, s')$ in in the algorithm~\ref{alg:detecting} line~\ref{}, where $\indicator(E)$ is the indicator function that returns $1$ if the statement $E$ is true, and $0$ otherwise. After obtaining $\Omega(s)$ and $\Omega(s, s')$, we can approximate the $P^2$ by $\bar{P^2}$ for P2 using a maximum likelihood estimator for P2's actual behavior's projection on state $S$ $\rho^2\downharpoonright_S$.

% Given the optimal deceptive policy $\tilde{\pi}_1^\ast$ and the \ac{mdp} $\tilde{\cal H}$, we can induce the $P^1$ from the $\tilde{\Delta}$ directly in line~\ref{ln:p1}. We introduce $\Omega(\tilde{v})$ and $\Omega(\tilde{v}, \tilde{v}')$ to denote the frequencies of state $\tilde{v}$ and the frequencies of the state pair $(\tilde{v}, \tilde{v}')$ in the augmented states $\rho$, respectively. Given a sequence of augmented states $\rho = \tilde{v}_0 a_0\tilde{v}_1a_1 \ldots \tilde{v}_n$, we estimate $\Omega(\tilde{v})$ and $\Omega(\tilde{v}, \tilde{v}')$ in line~\ref{ln:frequency_state} and line~\ref{ln:frequency_state_pair}, where $\indicator(E)$ is the indicator function that returns $1$ if the statement $E$ is true, and $0$ otherwise. After obtaining $\Omega(\tilde{v})$ and $\Omega(\tilde{v}, \tilde{v}')$, we can approximate the $P^2$ by $\bar{P^2}$ for P2 using a maximum likelihood estimator in line~\ref{ln:estimation}.

% After the maximum likelihood estimation, we employ the log of the likelihood ratio to introduce a distance measure $L$ each player $i$ as follows
% \begin{align*}
%     L^i = \sum_{(\tilde{v}, \tilde{v}') \in \Xi} \Omega^i(\tilde{v}, \tilde{v}') \log(\bar{P}^i(\tilde{v} \mid \tilde{v}')), i \in \{1, 2\},
% \end{align*}
% where $\Xi$ is the set contains all the state pairs $(\tilde{v}, \tilde{v}')$ in $\rho$.

% Given the distance measure $L^i$ for $\rho$ for $i \in \{1,2\}$, we propose an objective function $\Gamma$, a metric on the transition probability matrices, as follows
% \begin{align*}
%     \Gamma = - 2 \sum_{i}L^i.
% \end{align*}
% After the maximum likelihood estimation, we propose an objective function $\Gamma$, a metric on the transition probability matrices, in the eqation~\ref{eq:gamma}. Essentially, each term in $\Gamma$, \ie, the log of likelihood is the amount of information brought by the frequencies of state pairs and each transition matrix $P \in \{P^1, \bar{P}^2\}$. With the metric $\Gamma$ on $\rho$, we can identify the mismatch between the behavior of P2 and P1's model of P2's behavior. If the objective function $\Gamma$ exceeds some pre-defined threshold $\lambda$ in line~\ref{ln:if}, then the algorithm returns $P^1 \not = \bar{P}^2$, so P1's model on the P2's behavior mismatches P2's actual behavior. In that case, the optimal deceptive policy $\tilde{\pi}^\ast_1(\tilde{\cal H})$ does not serve its purpose in the actual interaction wiht P2, and P1 needs to stop. Otherwise, $P^1 = \bar{P}^2$, which means the approach does not detect the mismatch, and P1 can continue using the optimal deceptive solution $\tilde{\pi}_{1}^\ast(\tilde{\cal H})$ to outmaneuver P2.
If the algorithm rejects $H_0$, then it means that the algorithm identifies $P^1 \not = \bar{P}^2$. So we have a mismatch between the behavior of P2 and P1's model of P2's behavior, then P1 needs to stop the interaction with P2, and the optimal deceptive policy $\tilde{\pi}^\ast_1(\tilde{\cal H})$ does not serve its purpose in the actual interaction with P2. Otherwise, approach does not detect the mismatch, and P1 can continue using the optimal deceptive solution $\tilde{\pi}_{1}^\ast(\tilde{\cal H})$ to outmaneuver P2.




% Suppose $h^\ast$ is a realization of length $n+1$ from the induced stochastic process from the \ac{mdp} $\tilde{\cal H}$ and P1's strategy $\pi^\ast_1(\cal H)$, where $n$ is user-defined length of realizations, we have the transition probability matrix as
% \begin{align*}
%     \Omega^\ast(\tilde{v}' \mid \tilde{v}) =& \sum_{a \in A_1} \pi^\ast_1(\tilde{\cal H})(\tilde{v}, a) \tilde{\Delta}(\tilde{v}' \mid \tilde{v}, a),
% \end{align*}
% where $\tilde{\Delta}(\tilde{v}' \mid \tilde{v}, a)$ is the transition probability function from $\tilde{\cal H}$,
% and we let
% \begin{align*}
%     \Omega^\ast(\tilde{v}, \tilde{v}') = \sum_{k=0}^{n-1}\indicator(\tilde{V}^k = \tilde{v}, \tilde{V}^{k+1} = \tilde{v}')
% \end{align*}
% where $\indicator$ is the indicator function.

% Suppose $h^\rhd$ is another realization of length $n+1$, which is obtained online when P1 is using the same deceptive optimal strategy $\pi^\ast(\tilde{\cal H})$ to play against P2, where P2 potentially differs from P1's opponent modeling. \footnote{This realization is collected online by letting P1 using $\pi^\ast(\tilde{\cal H})$ to play against P2}. 
% The transition probability matrix here is estimated differently, and we let
% \begin{align*}
%     \Omega^\rhd(v, v') = \sum_{k=0}^{n-1}\indicator(V^k = v, V^{k+1} = v')
% \end{align*}
% and
% \begin{align*}
%   \Omega^\rhd(v) = \sum_{k=0}^{n-1} \indicator(V^k = v).
% \end{align*}
% Bartlett~\cite{bartlett1951frequency} has shown the maximum likelihood estimator of $\Omega^\rhd(v' \mid v)$ is given by 
% \begin{align*}
%     \Omega^\rhd(v' \mid v)  = \begin{cases}
%     \Omega^\rhd(v, v') / \Omega^\rhd(v), &\text{if } \Omega^\rhd(v) > 0, \\
%     \indicator(v = v'), &\text{if } \Omega^\rhd(v) = 0
%     \end{cases}
% \end{align*}

% We develop a test, inspired by~\cite{bartlett1951frequency}, of $H_0: \Omega^\ast = \Omega^\rhd$ versus the alternative hypothesis $H_1: \Omega^\ast \not = \Omega^\rhd$. First we introduce the test statistic based on the log of the likelihood ratio test statistic, given by
% \begin{align*}
%     \Gamma = -2 (L(h^\ast) + L(h^\rhd))
% \end{align*}
% where 
% \begin{align*}
%     L(h) = \sum_{(v, v') \in \Xi(h)} \Omega(v, v') \log(\Omega(v \mid v')),
% \end{align*}
% where $\Xi(h)$ contains all $(v, v')$ such that $\Omega(v, v') > 0$. 

% After introducing the metric $\Gamma$ on the space of transition probability matrices, we can develop a size-$\alpha$ test of $H_0: \Omega^\ast = \Omega^\rhd$, and we reject the null hypothesis $H_0$ when 
% $\Gamma > \lambda_{\alpha}$, where $\lambda_{\alpha}$ is the solution to the equation
% \begin{align*}
% \sup_{\Omega} P(\Gamma > \lambda \mid \Omega^\ast  = \Omega^\rhd = \Omega) = \alpha,
% \end{align*}
% with respect to $\lambda$, where $\alpha$ \footnote{Picking $\alpha$ is beyond this paper's scope. In practice, people select $\alpha = 0.01$ or $\alpha = 0.05$.} is the confidence level.

% If the test rejects the null hypothesis $H_0$, then we should realize that the opponent modeling incorporated by the P1 is inconsistent with P2. Moreover, P1 should stop the online interaction with P2 and modify the opponent modeling for performance improvement.

% where 
% \begin{align*}
%     L(h^x) = \sum_{(v, v')} \hat{P}^x(v, v') \log(\bar{P}^x(v \mid v')), x \in \{\ast, \rhd\}
% \end{align*}
% and $\lambda_{\alpha}$ is the solution to the equation
% \begin{align*}
% \sup_{\Omega} \Pr(-2 (L(h^\ast) + L(h^\rhd)) > \lambda \mid \bar{P}^\ast  = \bar{P}^\rhd = \bar{P}) = \alpha,
% \end{align*}
% with respect to $\lambda$, where $\alpha$ \footnote{Picking $\alpha$ is beyond this paper's scope. In practice, people select $\alpha = 0.01$ or $\alpha = 0.05$.} is the confidence level.


% \begin{algorithm}[!htb]
% \begin{algorithmic}[1]
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \REQUIRE length $n+1$ state sequences $h^x$.
% \ENSURE Estimated $\bar{P}^x(s' \mid s)$, $\hat{P}^x(s, s')$, and $\tilde{P}^x(s)$, for states $s$ and $s'$ in the $h^x$.

% \STATE{$\hat{P}^x(s, s') = \sum_{k=0}^{n-1}\indicator(S_k = s, S_{k+1} = s')$}

% \STATE{$\tilde{P}^x(s) = \sum_{k=0}^{n-1} \indicator(S_k = s)$}

% \STATE{\begin{align*}
%     \bar{P}^x(s' \mid s)  = \begin{cases}
%     \hat{P}^x(s, s') / \tilde{P}^x(s), &\text{if } \bar{P}^x(s) > 0, \\
%     \indicator(s = s'), &\text{if } \tilde{P}^x(s) = 0.
%     \end{cases}
% \end{align*}}
% \RETURN{$\bar{P}^x$, $\hat{P}^x$, and $\tilde{P}^x$}

% \end{algorithmic}
% \caption{Maximum Likelihood Estimation}
% \label{alg:estimation}
% \end{algorithm}



% \begin{remark}
% Another consideration for deceptive planning is to limit the number of hypothesis updates of P2. With a frequent changing hypothesis, P2 may select more adverse co
% \end{remark}

% \todo[inline]{limit the number of switching. using switching game formulation.}

% \begin{definition}[Hypergame]
% Let $\game_1$ and $\game_2$ be the games on graph as constructed by P1 and P2 in their mind, given P1's objective is to satisfy $\varphi_1$ and P2's objective is to satisfy $\varphi_2$. Then, a \textit{first-level} hypergame is a tuple
% \[
%     {\cal H}^1 = \langle \game_1, \game_2 \rangle.
% \]

% When one player is aware of misperception and other is not, we get a \textit{second-level} hypergame, given by the tuple
% \[
%     {\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle
% \]
% where P1 solves the first-level hypergame to compute his strategy. 
% \end{definition}


% We note that a \textit{second-level} hypergame models the game with information asymmetry described in Problem~\ref{}. We refer the reader to \cite{} for a general treatment of $k$-th level hypergame. 


% A definition of hypergame given in Def.~\ref{} does not account for evolving misperception. 




% % When P1 is aware of P2's misperception, P1 computes his strategy by anticipating the P2's strategy, given her perception $\psi_t$ of P1's objective. In order to anticipate P2's strategy, P1 must first construct a model of his opponent, P2. An opponent model consists of what P1 knows about (a) how P2 perceives P1's objective at $t=0$, (b) how P2 updates her misperception, \ie the inference mechanism of P2, and (c) given the misperception $\psi_t$, how does P2 compute her strategy.


==> Archived/planning.tex <==
% \todo[inline]{
% \begin{itemize}
%     \item almost-sure winning region of the game with complete information. comparing with the almost sure winning region for P1 in the hypergame on graph. Hypothesis: almost-sure winning in the hypergame, taking into account of P2's perceived rational strategy, will be a superset (after projecting onto $S\times Q$) of the almost-sure winning region. showing one example. Use toy example.
%     @abhishek with very general statement : combining the subgraph of switched games. Appendix: algorithms.
% \end{itemize}
% 2. }

In this section, we provide a solution to Problem~\ref{problem_statement} for a class of hypergames on graphs in which P2 uses change detection algorithm to identify the time-varying subgoal of P1 and reasons iteratively using the \ac{ch} model of games to compute her counter-strategy. 
The solution includes two steps: In the first step, we construct this class of hypergame on graph with finite, discrete state space from Def.~\ref{def:hypergame_graph} given P2's inference mechanism. In the second step, we compute the deceptive strategy for P1. 

Let $\path^{\le m}$ be a set of histories with length $\le m$ that can be generated from the game transition system. Note that the length of a  history  is defined by the number of state-action pairs in that history. For example, the history $\vs_0\va_0\vs_1\va_1\ldots \vs_{ m-1}\va_{m-1}\vs_{m}$ is of length $m$. The length corresponds to the size of the sliding window in change detection algorithm.
\begin{definition}
 Assuming that P2 uses a change detection inference $\eta: \path^{\le m  } \times {\cal X}\rightarrow \cal X$ and P1's objective is given by a co-safe \ac{ltl} formula,  the  hypergame on  graph is computed as 
\[
{\cal H} = \langle V, A, \Delta , u_0, {\cal F},  Acc_1 \rangle 
\]
with the following components:
\begin{itemize}
    \item $V= \path^{\le m} \times Q\times \cal X$. Each state includes a finite history $\rho = s_0 a_0 s_1 a_1\ldots s_\ell \va_\ell \vs_{\ell+1}$ where $\ell+1\le m$, an automaton state $q$ and the hypothesis $x$ of P2 in that state. 
    \item $A$ is the set of joint actions.
    \item $\Delta$ is the transition function, defined as follows. Given $v = (h s, q, x)$  with $h \in \path^{\le m-1} $. Given action $a \in A$ and state $s' $ for which $P( s' \mid s, a)>0$, 
      we distinguish two cases, depending on whether P2's hypothesis changes:
      \begin{itemize}
      \item If there is no change in hypothesis, that is,
        $\eta(x, h s a s')= x$, then let
        $v' = (h s a s' , \delta(q, L(s')), x)$ and
        $\Delta(v' \mid v, a) =P(s'\mid s,a)$.
      \item Otherwise, $\eta(x, h s a s')= x'$ and $x'\ne x$. Then
        let $v'' = (s' , \delta(q, L(s')) , x')$ and
        $ \Delta(v' \mid v, a) = P(s' \mid s, a) $ \end{itemize} That
      is, when P2 detects a change, then the history is discarded due
      to the change detection algorithm.
         \item $u_0 \sim \dist(V)$ is the initial state distribution. Given the initial state $\vs_0$, if the initial hypothesis  $x_0$ is deterministic, the initial state distribution is $u_0(\vs_0, q, x_0)=1$ with $q= \delta(q_0, L(\vs_0))$. If the initial hypothesis is given by a probabilistic distribution $b_0\in \dist(\cal X)$, then the initial distribution is $u_0((\vs_0, q, x))=b_0(x)$ with $q = \delta(q_0, L(\vs_0))$.
    \item ${\cal F}$ is the set of final states for P1. The set ${\cal F}$ is defined as the set $\path^{\le m} \times F \times {\cal X}$, where $F$ is the set of accepting states of the automaton $\cal A$. 
    \item $Acc =  \text{ Co-safety} $ is the acceptance condition for P1.
\end{itemize}
\end{definition}



Intuitively, for player 1 to plan the best strategy, he needs to keep track of the history which is used by player 2 to update her hypothesis, P2's  hypothesis at the current state, the current game state, as well as the transition in the game arena given both player's actions.
Based on the \ac{ch} theory, by knowing the subgoal inferred by P2, P1 is able to compute P2's counter-strategy using iterative reasoning--that is, if P1 predicts that P2's current hypothesis is $x$, then P1 assumes that P2 will adapt the counter-strategy $\pi_2^{(k)}(x)$--the level-$k$ strategy in $\game(x)$. For simplicity in notation, as the level-$k$ is clear from the context,  we denote P2's strategy to be $\pi_2: S\times {\cal X}\rightarrow \dist(A)$  so that $\pi_2(s,x) = \pi_2^{(k)}(x)$, for all $(s,x) \in S\times {\cal X}$.

Finally, marginalizing out P2's strategy from the hypergame on graph, we obtain a Markov decision problem with co-safe objective. The optimal policy in this \ac{mdp} is \emph{proactive} and \emph{deceptive} because  P1 predicts how his future action can influence the perception of P2 and plans his action to steer P2's perception in a way advantageous to his own temporal logic objective.  The Markov decision problem with co-safe objective is defined by:
\[
{\cal H}^{\pi_2} = \langle   V, A_1, \Delta^{\pi_2}, {\cal F}, \text{co-safety} \rangle 
\]
with the transition function defined by marginalizing out P2's action given her strategy ${\pi_2}$:
\[
\Delta^{\pi_2}(v' \mid v,a_1) = \sum_{a_2 \in A_2} \Delta(v' \mid v,(a_1,a_2)){\pi_2}(v, a_2).
\]
and for any $v\in \cal F$ or $v=(hs,q,x)$ and
$s\models \neg \varphi_{safe}$, $\Delta^{\pi_2} (v\mid v,a_1)=1$. Note
that upon reaching $v\in \cal F$, the history satisfies P1's co-safe
LTL specification. Upon reaching $v\in \neg \varphi_{safe}$, the
history violates P1's invariant safety objective and thus the
specification.

From the result of probabilistic model checking \cite{Baier2008},
to maximize the probability of satisfying the co-safe LTL specification, P1 equivalently maximizes the probability of reaching the set of states in $\cal F$.
\[
\max_{\pi} \Expect\left(\sum_{t=0}^\infty \mathbf{1}(v_t \in \calF)\right)
\]
To solve the optimal policy, we compute the set of states, $V_{=1}$, from which there exists a policy $\pi_{=1}$ that ensures the set $\cal F$ can be reached with probability one. This set $V_{=1}$ can be computed using accepting end components for qualitative reasoning in \ac{mdp}s \cite{Baier2008} and has linear time complexity in the size (state and transitions) of the \ac{mdp}. Next, we solve the stochastic shortest path problem given the following reward function  $r: V\times A_1\rightarrow [0,1]$ defined by,
\begin{equation}
    \label{eq:reward}
r(v,a) =  \sum_{v'\in V} \Delta^{\pi_2}(v' \mid v,a) \mathbf{1}(v' \in V_{=1}).
\end{equation}
and the states in $V_{=1}$ are all made to be absorbing.
 
The optimal policy $\pi$ is obtained from solving the \ac{mdp} ${\cal H}^{\pi_2}$ with the total reward criteria:
\[
\max_{\pi}  \Expect\left(\sum_{t=0}^\infty r(v_t,a_t) \mid v_0 \sim u_0\right).
\]
The optimal planning problem with the total reward criteria can be found in \cite{Puterman1994}. Let $\pi^\ast$ be the solution of the total reward planning problem. The optimal deceptive policy $\pi$   can be obtained by sequentially composing the policy $\pi^\ast$ and $\pi_{=1}$ as follows.
\[
\pi(v)=\left\{
\begin{array}{c cc}
    \pi^\ast( v) & \text{ if } v \notin V_{=1} , \\
     \pi_{=1}(v)& \text{ otherwise}. 
\end{array}\right.
 \]
 where policy $\pi_{=1}$  ensures the set $\cal F$ can be reached with probability one.

In practice, due to the large state space of the problem, we employed an online \ac{mcts}~\cite{silver2010monte,browne2012survey} to solve the probabilistic planning problem in ${\cal H}^{\pi_2}$. In the online version of MCTS, since the specification can be complex, it is a rare event to sample a trajectory that satisfies the specification. In other words, the reward function defined by Eq.~\eqref{eq:reward}
 is too sparse for any online planners. To mitigate this problem, we define the subgoal reward signals for  P1 during online planning.  We define the  subgoal reward signals as follows.
 
 \begin{itemize}
     \item First, for each state $q\in Q$ of the \ac{dfa}, we define a function $\level: Q\rightarrow \nat$ so that 
  $\level(q)$ is   the minimal number of transitions it takes to reach a state in the accepting states $F$ of the \ac{dfa}.
  \item Second, for each state $q\in Q$,  we employ reactive synthesis for concurrent reachability game \cite{de2000concurrent} to solve the \emph{almost-sure winning region} for the following game: 
  $\game(\varphi(q)) =\varphi_{safe}\until \lor_{\sigma \in X} \Eventually \sigma$ and the set $X =\{\sigma\mid  q\xrightarrow{\sigma} q' \land \level(q')< \level(q).
 \}$ 
 \item Given each state $v=(h s ,q,x)$, let the current reward function to be 
\[ r(h s,q') = \alpha \text{ if } s \in \win^1(\game(\varphi(q))).\]
 \end{itemize}
 where $\alpha$ is a positive constant.

  %Further, we assign penalty $-100$ for states at which the safety property $\varphi_{safe}$ is violated. 
  
 This subgoal reward signal may produce sub-optimal policies as it
 does not use backward induction in dynamic programming to define the
 reward. We are currently investigate how to improve the online
 planner.
% we use the sure-winning regions for P1 to give an intermediate reward, which speeds up the convergence of the algorithm. Instead of giving a reward when the simulated trajectory satisfies the specification, we give an intermediate reward when the system makes progress, meaning it reaches a state within a subgoal of the specification. By doing that, the reward signal can be quickly backpropagated. This can guide the system to pick the best action for the current state efficiently. For more details of sure-winning regions computation, readers are referred to~\cite{de2000concurrent}.For more details, readers are referred to Algorithm~\ref{alg:mcts} in Appendix~\ref{sec:pseudo_code}. 

==> Archived/sections/archieved.tex <==
The subgoal inference with sliding window change detection can be represented as an inference function $\update: G \times H^{\le k}\rightarrow G \times H^{\le k}$ that maps a current hypothesis and a finite history of length $\le k$ to a new hypothesis and a new history. When a change is detected,  the new history only consists of the most recent observation, that is, a transition in the arena. When there is no change, the new history is obtained by appending the old history with the new observation.

Let $k$ be the maximum length of the sliding window size, $H^{\le k}$ be the set of possible histories of length smaller than or equals $k$, and $G$ be a set of possible subgoals. Consider the inference $\update: G \times H^{\le k}\rightarrow G \times H^{\le k}$, we construct a new game-arena with augmented state space as follows.
\[ \hat M =  (   \vS \times H^{\le k}\times G, \vA, \hat T, \calap, \hat L)
\]
\begin{itemize}
\item  $ \hat \vS= \vS\times H^{\le k}\times G$ is a finite set of states. Each state $(\vs, h, g)$ includes a current game state $\vs$, a finite observation hostory of length $\le k$ and a subgoal $g \in G$.
\item $\hat T :  \vS\times  H^{\le k}\times G \times \vec{A}\rightarrow  \dist{\vS\times  H^{\le k}\times G}$ is the probabilistic transition function, defined as follows.
\begin{multline}
\hat T ( (\vs' , h', g')|(\vs, h, g), (a_1,a_2)) \\=\left\{ \begin{array}{ll}  P(\vs'|\vs, (a_1,a_2)) & \text{ if }  (h',g')= \update( (h, (a_1,a_2), \vs'), g).\\
0 & \text{otherwise}.
\end{array}\right.
\end{multline}
That is, the transition to a new state is probabilistic and follows the transition function in the stochastic system. The history of observations is updated by the subgoal inference, as well as the predicted subgoal.
\item $\calAP$ is a finite set of atomic propositions.
\item $ \hat L: \vS\times H^{\le k}\times G \rightarrow 2^\calAP $ is the labeling function, defined as $\hat L((\vs, h, g))= L(\vs)$.  That is, the label of an augmented state is determined by the label of the first component---that is, the state in the stochastic system. 
\end{itemize}

\begin{algorithm}[!htb]
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE{The sequence of the adversary fictitious inputs}
\ENSURE{The mean level $\lambda^{n}$}
    \FOR{$i = 0, \dots, T$}
        \FOR{$k = 0, \dots, \calK$}
        \STATE{for $t \in [0, n]$, measure the value of \eqref{eqn:r_k}}
        \ENDFOR
        \FOR{$k = 0, \dots, \calK$}
            \STATE{Compute the mean level according to~\eqref{eqn:sigma_k}}
        \ENDFOR
        \STATE{Update the estimation according to~\eqref{eq:lambda_update}}
    \ENDFOR
\end{algorithmic}
\caption{Intelligence Level Learning}
\end{algorithm}


==> Archived/sections/case-study.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Parameters of different algorithms %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In this section, we illustrate the proposed algorithm in a robot motion planning example in adversarial environment, shown in Fig.~\ref{fig:grid_world}. In this game, P1 (Blue agent) is to achieve a given temporal logic specification $\varphi$ while player 2 (Red) is the opponent. Both players can move deterministically and simultanously in four compass directions in this $11$-by-$11$ grid world, with action sets $\{\mbox{Up} (U), \mbox{Down} (D), \mbox{Left} (L), \mbox{Right} (R)\}$. In this environment, there are a set of obstacles (marked in black cells) and several critical way-points, marked as $g_i=(x_{g_i}, y_{g_i}), i=1,\ldots, 4$. If a player hits the boundary of the grid world or any obstacles, it will stay put in its original cell. 

\begin{figure}[!htb]
\begin{subfigure}[b]{0.786\linewidth}
    \includegraphics[width=\linewidth]{Figure/fancy_grid_world.png}
    \caption{ }
\end{subfigure}
\begin{subfigure}[b]{\linewidth}
    \includegraphics[width=\linewidth]{Figure/3th_simulation_grid.png}
    \caption{ }
\end{subfigure}
\caption{(a) The grid world (b) The simulation with the complex specification is: $\neg (p_1\land p_2)  \until ( \Eventually (\mathsf{Reach}(g_1)  \land \Eventually \mathsf{Reach}(g_4) )\\ \lor 
\Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) )$}
\label{fig:grid_world}
\end{figure}
%%% task specification
The following atomic propositions are used: Given that P1's position is $(x_1,y_1) $ and P2's position is $(x_2,y_2)$, 
\begin{enumerate}
\item $p_1\coloneqq \abs{x_1-x_2} + \abs{y_1-y_2} \le \xi$: this is evaluated true if the Manhattan distance  of P1 and P2 are less than a given threshold $\xi$.  In this experiment, we set $\xi= 1$.
\item $p_2\coloneqq x_1\ge 4$: this is evaluated true if P1 is in the control area of P2. 
\item $\mathsf{Reach}(g_i) \coloneqq (x_1,y_1) = g_i$, for each $i=1,\ldots, 4$. This proposition is evaluated true when P1 reaches a given waypoint $g_i$. It can be generalized to be $(x_1,y_1)\in g_i$ if $g_i$ is a set of cells instead of a single cell. 
\end{enumerate}

\begin{figure}[!htb]
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,scale=0.7,semithick, transform shape]
		\tikzstyle{every state}=[fill=black!10!white]
		\node[initial,state]    (0)                 {$q_0$};
        \node[state]            (1) [right of=0]    {$q_1$};
        \node[state, accepting] (2) [right of=1]    {$q_2$};
		\path[->]   
		(0) 		edge                node    {$g2$}                      (1)
        (1)         edge                node    {$g3$}                      (2)
		;
	\end{tikzpicture}
    \caption{The task automaton for the simple specification
          $\varphi_{simple}$. We omitted the selfloops and transition
          to the sink, nonaccepting state with labeling $\{p_1,p_2\}$
          for clarity.}
\label{fig:simple_automaton}
\end{figure}


    
\begin{figure}[!htb]
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,scale=0.7,semithick, transform shape]
    	\tikzstyle{every state}=[fill=black!10!white]
    	\node[initial,state]    (0)                     {$q_0$};
        \node[state]            (1) [below left of=0]   {$q_1$};
        \node[state]            (2) [below of=0]        {$q_2$};
        \node[state]            (3) [below right of=0]  {$q_3$};
        \node[state, accepting] (4) [below of=2]        {$q_4$};
    	\path[->]   
    	(0) 		edge    node[left]      {$g1$}                      (1)
    	(0) 		edge    node            {$g2$}                      (3)
        (1)         edge    node[left]      {$g2$}                      (2)
        (1)         edge    node[left]      {$g4$}                      (4)
        (2)         edge    node            {$g3 \vee g4$}              (4)
        (3)         edge    node            {$g1$}                      (2)
        (3)         edge    node[above]     {$g3$}                      (4)
    	;
    \end{tikzpicture}
    \caption{The task automaton corresponds to the complex
      specification $\varphi_{complex}$. We omitted self-loops and
      transition to the sink, nonaccepting state with labeling
      $\{p_1,p_2\}$ for clarity.}
\label{fig:complex_automaton}
\end{figure}

We perform several experiments with different \ac{ltl} specifications for P1: 
\begin{itemize}
    \item A simple task specification (with the corresponding \ac{dfa} in Fig.~\ref{fig:simple_automaton}): 
   \[ \varphi_{simple}= \neg (p_1\land p_2) \until \left( \Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) \right).\]
   which is, P1 is to avoid being captured by P2 until it reaches $g_2$ and then $g_3$.
    \item A more complex task specification  (with the corresponding \ac{dfa} in Fig.~\ref{fig:complex_automaton}): 
        \begin{align*}
            \varphi_{complex} = \neg (p_1\land p_2)  \until ( \Eventually (\mathsf{Reach}(g_1)  \land \Eventually \mathsf{Reach}(g_4) )\\ \lor 
            \Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) ).
        \end{align*}
        In words, P1 is to avoid being captured by P2
until it either reaches $g_2$ and then $g_3$, or reaches $g_1$ and then $g_4$.
\end{itemize} 
It is noted that in Fig.~\ref{fig:complex_automaton}, the state $q_2$ means that P1 has just seen $g_1$ and $g_2$. P1 can satisfy the task by visiting either $g_3$ and $g_4$. We design the two specifications with the idea that the language of the simple specification is a subset of that of the complex specification. This is related to one of hypothesises, discussed next.
 

The following hypothesises are considered before the experiments.
\begin{enumerate}
    \item Hypothesis 1: The probability of success given the complex specification  should be higher than that given the simple specification, assuming the same hypothesis space of P2.
    \item Hypothesis 2: Given the same specification, the probability of success given P2's hypothesis space ${\cal X}=\{g_2,g_3\}$ will be lower than that given P2's hypothesis space ${\cal X}= \{g_1,g_2,g_3,g_4\}$. 
    \item Hypothesis 3: By playing deceptively and leveraging the private information, player 1 can achieve better performance in regions that he has no chance of winning had the information is symmetric between players.   
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Figure of the gridworld %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Description of two cases %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To test the hypothesises, we conduct the following experiments: 
\begin{itemize}
    \item Comparison of winning rates between simple and complex specifications: In   experiment 1, P1's tasked with the simple specification (with \ac{dfa}  in Fig.~\ref{fig:simple_automaton}). The hypothesis space for P2 is ${\cal X}=\{g_1,g_2,g_3,g_4\}$--that is, at any time, P2 believes that P1 is pursuing a subgoal within $\cal X$.  In experiment 2, P1 is tasked with the complex specification in Fig.~\ref{fig:complex_automaton}. 
    \item Comparison of winning rate for the same specification but different hypothesis spaces of P2: In experiment 3, we consider the same simple specification as that in experiment 1, but change P2's hypothesis space to be ${\cal X}' =\{g_2,g_3\}$.
    \item Analysis of the advantages due to deceptive planning: In experiment 4, we consider the complex specificiation as in experiment 2, but change the initial state to be in the sure losing region of P1 in the game $\game(\varphi_{complex})$ where both players have complete information. 
\end{itemize}
In these experiments, P2 uses level-2 of thinking in the \ac{ch} model. The state space size of the game transition system is $1e+5$. The state space size of the hypergame is up to $1e+43$. The action space size is $16$. Due to the large state space, we use online \ac{mcts} algorithm with the following parameters: the depth of \ac{mcts} simulation is $50$, the number of the simulations is $200$, the exploration scalar $c$ is $\frac{1}{\sqrt{2}}$.  For the change detection algorithm, the window size is $7$, and the threshold is $0.3$. Other parameters are the following: discounting factor $\gamma = 0.8$, the user-specified temperature $\tau$ is $1$. We perform each experiments 100 times and collect the statistics.

The winning rates of the three experiments are shown in Table.~\ref{tab:main_results}. From the experiment, hypothesis 2 is validated:   P2's  easier to be distracted if there are subgoals in her hypothesis that are not pursued by P1. These subgoals becomes decoys that can be used by P1 for deception. Hypothesis 1 is not validated: We anticipate that with the complex specification, P1 could have a higher probability of success than the simple specification. The reason is that the language of the simple specification is a subset of that of the complex one--that is, P1 have more  ways to satisfy the task.
But the winning rate of experiments 2 is slightly lower than that of experiment 1. We expect this is due to the sub-optimality in the online MCTS and will validate the hypothesis with a smaller example for which the exact solution can be obtained. Hypothesis 3 is validated: In the sure-losing region of P1 assuming complete information, P1 can achieve a win rate of $82\%$using deceptive planning that leverages his private information,  comparing to $0\%$ (symmetric information case).


\begin{table}[!htb]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Experiment setups                                                          & Winning rate \\ \hline
 % P1 play level 1 policy, P2 play level 2 policy, goal: g4                   & 0\%          \\ \hline
% P1 play level 3 policy, P2 play level 2 policy, goal: g4                   & 94\%         \\ \hline
1. Simple specification with  ${\cal X} = \{g1, g2, g3, g4\}$                   & 72\%         \\ \hline

2. Complex specification   with  ${\cal X} = \{g1, g2, g3, g4\}$                                                         & 64\%         \\ \hline
3. Simple specification with ${\cal X} =  \{g2, g3\}$                           & 59\%         \\ \hline
4. Starting with sure losing regions for P1 with  complex spec & 82\%         \\ \hline
\end{tabular}%
}
\caption{Winning rates under different experiment setups.}
\label{tab:main_results}
\end{table}

% \begin{comment}
 
% \paragraph*{Baseline (Complex specification)}
% Given a specification $\varphi_1=\neg (p_1\land p_2)  \until ( \Eventually (\mathsf{Reach}(g_1)  \land \Eventually \mathsf{Reach}(g_4) )\\ \lor 
% \Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) )$, we construct the game arena with augmented state space. The P1 needs to visit $g2$ first, after visiting $g2$ P1 needs to visit $g3$, or P1 needs to visit $g1$ first, after visiting $g1$ P1 needs to visit $g4$, while avoid being captured by P2.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figure/3th_prediction.png}
    \caption{The corresponding predictions of P2 in the  trajectory shown in Fig.~\ref{fig:grid_world}.}
    \label{fig:3_th_simulation}
\end{figure}
 Finally, given P1's winning strategy and a predicted strategy of P2, a sampled trajectory is shown in Fig.~\ref{fig:grid_world}. The trajectories of P1 and P2 are shown in blue and red, respectively.
 %A trajectory in the form of 
% \begin{align}
% ((s,q), h, g)
% \xrightarrow{(a_1,a_2)}
% ((s',q'), h', g')
% \end{align}
This trajectory is segmented into two parts: In the first part, P1 uses the deceptive optimally planning and later reaches his winning region for game $\game(\varphi_{safe}\until  \mathsf{Reach}(g_1))$. Then, P1 uses the almost-sure winning strategy of the game $\game(\varphi_{safe}\until  \mathsf{Reach}(g_1))$. After reaching $g_1$, P1 uses deceptive planning  and reaches his winning region for game $\game(\varphi_{safe}\until  \mathsf{Reach}(g_4))$.  Then, P1 uses the almost-sure winning strategy of the game $\game(\varphi_{safe}\until \Eventually \mathsf{Reach}(g_4))$. 
The corresponding prediction of P2's inferred subgoals  is shown in Fig.~\ref{fig:3_th_simulation}. We marked the two time steps when the two almost-sure winning regions are reached. It is observed that once P1 reaches the almost-sure winning region for subgoal $g_1$ (resp. $g_4$), and plays out his almost-sure winning strategy, P2 can correctly infer his subgoal but cannot do anything to prevent P1 from achieving it. Before that, P2's prediction oscillates between four subgoals as an outcome of deception. 

% \paragraph*{Simple specification}
% Given a simple specification $\varphi_1=\neg (p_1\land p_2) \until \left( \Eventually (\mathsf{Reach}(g_2) \land \Eventually \mathsf{Reach}(g_3)) \right)$, we construct the game arena with augmented state space. The P1 needs to visit $g2$ first, after visiting $g2$ P1 needs to visit $g3$, while avoid being captured by P2.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Prediction of getting caught %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Figure/prediction.png}
%     \caption{The prediction of the single chain with only $\{g2, g3\}$}
%     \label{fig:prediction}
% \end{figure}

\begin{comment}
The following may be used in extended version.

\paragraph*{Complex specification with different initial starting position}
In this case, the P1 starts at $(0, 6)$, and P2 starts at $(4, 2)$.

\paragraph*{Analysis}
In order to get the statically results, we run $100$ simulation between P1 and P2 where P2 is using the level $2$ policy which can be learned from the data. The winning rates under the different experiment setups are shown in the Table~\ref{tab:main_results}. To prove the correctness of the precomputed policy for different levels of policy, we use a simple reach-avoid game which can be described by the P1's specification as the following: 
\begin{align}
\varphi_1 = \neg (p1 \wedge p2)\until \Eventually \mathsf{Reach}(g4) \end{align} 
where P1 is trying to reach $g4$, and P1 uses the level $1$ and level $3$ policies to play again P2 using level $2$ policy.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Table of winning rates %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!htb]
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|l|}
\hline
Experiment setups                                                          & Winning rate \\ \hline
P1 play level 1 policy, P2 play level 2 policy, goal: g4                   & 0\%          \\ \hline
P1 play level 3 policy, P2 play level 2 policy, goal: g4                   & 94\%         \\ \hline
Simple specification with decoy set $\{g2, g3\}$                           & 59\%         \\ \hline
Simple specification with decoy set $\{g1, g2, g3, g4\}$                   & 72\%         \\ \hline
Complex specification                                                      & 64\%         \\ \hline
Starting with sure losing regions for P1 with the same complex spec & 82\%         \\ \hline
\end{tabular}%
}
\caption{Winning rates under different experiment setups.}
\label{tab:main_results}
\end{table}

We compare first two rows in the Table~\ref{tab:main_results}, it indicates that when P1 is using level $1$ policy and P2 is using level $2$ policy, P1 is caught by p2 almost every time out of 100 times. On the other side, when the P1 is playing level $3$ policy and P2 is using the same level of policy, P2 has a very high probability of reaching the goal $g4$. The reason why the winning rate is not $100\%$ is may due to stochasity in the policy caused by the temperature in the softmax bellman operator. 

Comparing the winning rates of simple specification and complex specification, the winning rate of simple specification is no better than that of complex specifications. It demonstrate the effectiveness of the inference. Because when the task automaton is a single chain, it is reasonable to have lower winning rate, since the P2 can quickly infer the subgoal of the P1 and catch the P1. When the task automaton is not a single chain, there are more than one options, P2 can become confused, and it is harder for P2 to catch the P1. 

When the P1 and P2 starting at initial positions which are sure losing for P1, the result shows there is a positive winning rate for P1, which proves the effectiveness of the deception. Since if P2 has the full knowledge of P1, the probability of completing the specification for P1 should be close to $0$. However, when P1 takes the deception into the consideration of planning, the positive winning rate indicates deception help increaing the winning rate. 

% \todo[inline]{Here: include a graph that shows the probability of winning (obtained from value iteration) given P1's strategy in both deceptive planning and the baseline. We hypothesize that the probability of winning should be increased over all sampled states.}

% Then, we consider a mismatch in Blue's opponent model of Red and the true mind of Red. Particularly, we assume that Blue uses a change detection with sliding window of size $n$ and Red uses a change detection with sliding window of size $m$. We test three cases $n=m$, $n=m-k$, and $n=m+k$ and evaluate the probability of satisfying the task from different initial states. \todo[inline]{pick a value of $k$. The hypothesis is that when $n=m-k$ and $k$ is large, the deceptive winning strategy is less effective. When $n=m+k$, the deceptive winning strategy is as good as $n=m$, which was selected long enough to capture the change.}


\end{comment}

To justify that the level $k$ of P2 can be learned correctly, we evaluate the correctness of the proposed opponent modeling method.
\paragraph*{Experimental validation on opponent Modeling}~\label{case_study:opponent_modeling}
We pre-compute the policies of different levels of thinking (until level 4) for P1 and P2 with respect to the decoy $g_1$. 
To validate the correctness of the algorithm, we sample $100$ data points $X = [x_1, x_2, \dots, x_{100}]$ from a Poisson distribution with $\tilde{\lambda} = 2$, which is the ground truth. The goal is to estimate the true $\tilde{\lambda}$. For each date point $x_i$, we use $x_i$-level policy for P2 and $x_i - 1$-level policy for P1 to sample a trajectory with length of $n+1$, where $n=10$. % $\bm{K} = [0,1,2,3,4]^\top$. The user-specified temperature $\tau = 1e-2$.
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{Figure/lambda_learning.png}
    \caption{The convergence of the Poisson parameter $\lambda$ under the update rule~\eqref{eq:lambda_update}.}
    \label{fig:opponent_modeling}
\end{figure}
The following parameters are used in the inference algorithm: The upper bound on the level of thinking of P2 is 4 and the user-specified temperature $\tau = 1e-2$.
Figure~\ref{fig:opponent_modeling} indicates that our algorithm quickly infers the   level of thinking of P2 with a small error, and with the iterations go further, it converges to the ground truth. %We believe that if the data of interaction between P1 and P2 is provided, our algorithm can efficiently infer the truth level of P2's policy.

==> Archived/sections/cognitive_hierarchy.tex <==
 From the perspective of player 1, he   models the perceptual game of P2  with the purpose to  understand how his actions   can influence the hypothesis of P2 about the intention, as well as predicting the counter-strategy of P2 given her hypothesis. 
Given the common knowledge that  a temporal logic formula describes a sequence of temporally extended goals, it is reasonble to consider that P2  tries to infer the changing subgoals of P1 and counteract correspondingly. Thus, we present  a method to model the evolving perception and stratetgy of P2 with 1) Opponent modeling with  cognitive hierarchy; and 2) Change detection algorithm for subgoal inference. 
 
 %Theory of mind with cognitive hierarchy learns the true level $k$ of policy used by P2. The change detection algorithm use the observation between P1 and P2 to update P2's prediction of P1' intention. 

\subsection{Theory of mind with cognitive hierarchy}~\label{sec:cognitive_hierarchy}

One approach of opponent modeling is based on \ac{ch} of
games~\cite{camerer2004cognitive}. In the \ac{ch} of games, players
act according to different levels of reasoning: A player's level-0
strategy is either a nominal strategy or a strategy that randomizes
equally over all actions. A player' level-1 strategy best responds to
an opponent with level-0 strategy. Inductively, a player's level-$k$
strategy best responds to its opponent's level-$(k-1)$ strategy.

% Based on the \ac{ch} model, if P1 knows for which level-$k$ a player P2 is, then P1 not only knows how P2 predicts to be P1's unknown objective as P2 will use the level-$k-1$ policy of P1, but also P1 knows how P2 will respond to the predicted policy of P1.

Given a bounded-rational opponent P2, 
we propose to formulate the opponent modeling as the problem of learning the value of $k$ in P2's level of reasoning.  In \ac{ch} model, it is  discover that each player believes its opponent's level follows a probability distribution~\cite{chong2016generalized}. Thus, we propose an offline learning algorithm to infer P2's level of thinking from the histories. We model the distribution over the different levels as a Poisson distribution with the following probability mass function:
\begin{equation*}
    p^{k} = \frac{\lambda^k e^{-\lambda}}{k!},
\end{equation*}
where $\lambda$ is a parameter. The problem of learning the value of $k$ is transformed into how to estimate the $\lambda$ in the Poisson distribution. 

Given a finite-length history of the game $\rho = \vs_0, (a_0^1, a_0^2), \vs_1, (a_1^1, a_2^2) \dots \vs_n$ where $a_k^i$ is player $i$'s action at the $k$-th step. For a fixed sequence of P1's actions, the probability of $\rho$ for each level-$k$ P2's policy $\pi_2^{(k)}$  is computed by 
\begin{align}
    r^k =  \prod_{t=0}^{n-1} P(\vs_{t+1} \mid \vs_t, \va_t) \cdot \pi_2^{(k)}(a^2_{t} \mid \vs_t) , k \in \{0, 1, \dots, \calK\},
    \label{eqn:r_k}
\end{align}
where $\va_{t} = (a^1_{t}, a^2_{t})$, and $\calK$ is the pre-defined upper bound on the level of thinking of P2. It is noted that the intelligence level $\calK$ tends to infinity, the solution convergences to the Nash equilibrium~\cite{kanellopoulos2019non}. It is noted that this probability $r^k$ does not assume that P1 uses a policy of level $k-1$. 

We compute the scores of different level policies according to: for each $k \in \{0, 1, \dots, \calK\}$,
\begin{equation}
    \sigma^k = \frac{e^{\frac{r^k}{\tau}}}{\sum_{j=1}^{\calK}e^{\frac{r^j}{\tau}}}, 
\label{eqn:sigma_k}
\end{equation}
where $\tau \in \reals^{+}$ is the softmax temperature parameter. We denote $\bm{\sigma} = [\sigma^ 0, \sigma^1, \cdots, \sigma^\calK]^\top$. 

After getting the scores for different policies, we use the following update rule~\cite{frome1973regression} to update the estimation of $\lambda$ in an incremental way, for each past interaction history,
\begin{equation}
    \lambda^{i+1} \leftarrow \frac{i}{i+1} \lambda^{i} + \frac{1}{i+1}\bm{K}^\top \bm{\sigma}, i \in \{0, 1, \dots, T\}
\label{eq:lambda_update}
\end{equation}
where $\bm{K} = [0, 1, \cdots, \calK]^\top$ is a vector of different
levels. The estimated value $\lambda$ gives us a distribution over the
level of thinking for P2 based on past interactions. When P2 is
rational, then based on the \ac{ch} model, $\lambda$ approaches
infinity. Thus, using this inference will not restrict us from playing
against a more rational opponent.

Given the deceptive planning is carried out only once, we assume that P2's level of thinking will not change during interactions. It would be interesting to investigate how P2 adapts her level of thinkings during repeated interactions when P1 employs deceptive strategies.

%Please notice there are difference between the update rules of this and in the paper~\cite{kanellopoulos2019non}. 

\subsection{P2's evolving perceptual game with subgoal inference}~\label{subsec:change_detection}
Given the common knowledge that P1's objective $\varphi_1$ is a temporal logic formula, it is reasonable to assume that during online interaction,  P2 tries to infer the next subgoal in the temporal sequence. Next, we describe a change detection-based subgoal inference algorithm.

We denote the set of possible subgoals to be $G\subset S_1$--a subset of P1's states. We assume that $G$ is a common knowledge and define a set of atomic propositions $\{ p_{g}\mid g\in G\}$. For each $g\in G$, proposition $p_g$ evaluates true at state $s\in S$ when P1 has reached the subgoal state $g$. 

\begin{definition}[P2's hypothesis space]
  Given a set of possible subgoals $G$ for P2, the hypothesis space
  for P2 is ${\cal X} = \{ \varphi_{safe}\until p_g \mid g \in G\}
  $. for each hypothesis $x \coloneqq \varphi_{safe}\until p_g $ ,
  P2's perceptual game is defined by
  \[
    \game (x) = \langle TS, x, \neg x\rangle
    \]
    where P1's task formula is given by $x$ and the game is zero-sum.
  \end{definition}

For simple goal-reaching objective, the optimal strategy for both players can be solved via the solution of the following Markov game:
\[
\langle \vS, \vA, \bar P, U_x\rangle
\]
where $\vS,\vA $ is defined exactly as these in the transition system
$TS$.  The transition function $\bar P$ is the same as the transition
function $P$ of $TS$ except that in $\bar P$, a state
$s \models (\neg \varphi_{safe}\lor  p_g) $ is made absorbing.
The newly introduced component is a payoff function
$U_x: S\rightarrow [0,1]$ is defined by
\[
U_x(\vs,\va)= \Expect_{\vs'}\mathbf{1}(\vs' \models p_g).
\]
That is, the payoff of a state-action pair is given by the probability of P1 reaching his subgoal in one step. P2's payoff is the negation of P1's payoff given the zero-sum property.

Based on the assumption that P2's boundedly rational, we employ the \ac{ch} model of games to solve, the level-$k$ strategy  $\pi_2^{(k)}(x)$ for P2 and level $k-1$ strategy   $\pi_1^{(k-1)}(x)$ for P1, for each game $\game(x)$, $x\in \cal X$. Next, we describe how P2 uses the pairs $\{\langle \pi_1^{(k-1)}(x),\pi_2^{(k)}(x)\rangle  x\in \cal X\}$ of strategies to evolve her perceptual game.


\paragraph*{Sliding-window change detection for subgoal inference} We
index the set of games $\{\game(x)\mid x\in \cal X\} $ for clarify.
For each subgoal $x_\ell $, let $M_\ell$ be the \ac{mc} induced from
the stochastic transition system by P2's prediction of P1's strategy
and P2's counter-strategy in the Markov game.

% todo: describe the sliding window inference at high-level.
To detect a change in P1's subgoal as early as possible, we assume
that P2 employs an online change detection algorithm--sliding window
change detection based on the \ac{cusum}
statistic~\cite{basseville1993detection}. Given a data in forms of a
history (joint state-action sequence) and a nominal model (a Markov
chain), the sliding window uses a sequence of history over a time
window and detects if a change has occurred in the model that
generates the data during this time window. Next, we describe the
algorithm in more details.

For each hypothesis $M_\ell$ and a nominal model $M_0$, the algorithm computes the log-likelihood ratio,
\begin{align}
S_k^\ell =\sum_{i=1}^k s_i^\ell,
\end{align}
where $s_i^\ell= \ln \frac{P_\ell(y_i)}{P_0(y_i)}$, $y_i$ is the
$i$-th observation of the transitions \emph{within the sliding window
  size} and $P_\ell(y_i)$ (resp. $P_0(y_i)$) is the probability of
observing the transition in the model $M_\ell$ (resp. $M_0$). For
example, given a history $\rho= \vs_0\va_0\vs_1\ldots \vs_n$, and a
sliding window from $[k, k+m]$ with size $m+1$, the history within
this sliding window is
$\vs_{k}\va_k \ldots \vs_{k+m}\va_{k+m}\vs_{k+m+1}$ and
$y_i=(\vs_{k+i}, \va_{k+i})$ is the $i$-th observation within the
window.
%\todo[inline]{Do we take $s_{k+1+i}$ into consideration. If we take that into consideration, we will take the system dynamics into consideration. If we do not take that into consideration, we only consider the decision of agent at state $s_{k+i}$--- feel free to change this according to your implementation. I am ok with dropping $s_{k+i+1}$.} 

Based on the definition, the log likelihood ratio shows a negative
drift before a change and a positive drift after the change. Thus, the
relative information for change detection lies in the difference
between the log likelihood ratio and its current minimum value. The
CUSUM score is given by
\begin{align}
    Z_k^\ell  = S_k^\ell - \min_{1\le j\le k} S_j^\ell.
\end{align}

Recursively, the CUSUM score is computed for each hypothesis $x_\ell$
as
\begin{align}
Z_k^\ell = \max\{0, Z_{k-1}^\ell + \ln \frac{P_\ell(y_k)}{P_0(y_k)} \},
\end{align}
where $Z_0^\ell= 0$.


A change is detected at time $t$ when the score of at least one model,
say $M_\ell$, exceeds a threshold $h>0$.
\[
t= \min\{ k:  \exists x_\ell \in {\cal X},\; Z_k^\ell \ge h\}.
\]
Once a change is detected, the algorithm sets the nominal model to be
the current predicted model, disregards the history until the
change, and keeps running the online change detection given new
observation from the change point onwards. In the case when multiple
models has similar CUSUM scores, we select one model based on
some domain-specific heuristics or at uniformly random.
\begin{remark}
  Here, we described the change detection assuming boundedly
  rationality of P2 with level-$k$ learned by P1 from historical
  interactions. However, this change detection does not restrict to
  boundedly rational players. If P2 were rational, the equilibrium of
  the Markov game $\game(x)$ for each $x\in \cal X$ would be solved
  and used for subgoal inference.
  \end{remark}
 



==> Archived/sections/conclusion.tex <==

In this work, we propose a hypergame model to capture the interaction between players with asymmetrical information given Boolean temporal logic task specifications,  and   develop  a deceptive optimal planning method. This hypergame model  allows us to reason about the outcomes of games given bounded rational players by integrating the cognitive hierarchy model in games. We introduce a novel opponent modeling method to infer the level of bounded rationality of the opponent and to predict the counter policy of the opponent given her evolving perception of the game.  We are currently investigating the online \ac{mcts} algorithm for temporal logic planning. As future work, we would like to understand the robustness of deception given a potential mismatch in the assumption of the opponent model. It is also important to understand how the opponent may adapt to deception during repeated interactions.

==> Archived/sections/hypergame.tex <==
We choose to model a game under information asymmetry as a hypergame \cite{bennett1980hypergames}. A hypergame model can capture both the misperception of P2, and P1's awareness that P2 is misperceiving his objective.  


\begin{definition} \cite{bennett1980hypergames,Vane}
A hypergame model of level-1 is defined as \[{\cal H}^1 = \langle \game(\varphi_1), \game(x) \rangle,\] where $\game(\varphi_1)$ is the game as constructed by P1 given his objective $\varphi_1$ and $\game(x)$ is the game as constructed by P2 given her hypothesis $x \in \cal X$. When P1 is aware of P2's misperception but P2 is unaware of it, the resulting hypergame is said to be of level-2, and is defined as \[{\cal H}^2 = \langle {\cal H}^1, \game(x) \rangle.\] In a level-2 hypergame, P1 computes his strategy by solving the level-1 hypergame, while P2 computes his strategy by solving the game $\game_2$. 
\end{definition}

Higher levels of hypergames can be defined through a recursive reasoning about higher-order information--what I know that you know that I know ...
In this scope, we restrict to level-2 hypergames.

The above hypergame model does not account for evolving misperception in the encounter.   One way to understand P2's evolving misperception and its effect on her strategy is the following. Say, at some moment during the encounter, P2's hypothesis is $x \in \cal X$ and she remembers a finite history $h \in(\vS \times \vA)^k \times\vS$ of length-$k$. Then, she can evaluate whether the actions of P1 conform with her hypothesis or not. If not, she may update her hypothesis to match her observations. That is, given a hypothesis $x \in \cal X$, P2 selects an action according to the strategy $\pi_2(x)$ in the game $\game(x)$. After observing the actions chosen by P1, she updates the finite history $h \in(\vS \times \vA)^k \times\vS$ in her memory, and uses her inference mechanism $\eta$ to update her hypothesis to $x' = \eta(x, h')$. In the next step, P2 can be assumed to choose an action according to strategy $\pi_2(x')$ in the game $\game(x')$, instead of using $\pi_2(x)$. 
\begin{comment}
\todo[inline]{Add the diagram}

The above discussion naturally leads to a switched game diagram as shown in Fig.~\ref{}. Every state in Fig.~\ref{} represents a game $\game(x_i)$ where $x_i$ is a plausible hypothesis from $\cal X$. The edges in Fig.~\ref{} represent an update in P2's hypothesis, which in turn lead to P2 switching her strategy from some game $\game(x)$ to that in some other game $\game(x')$. We formalize this intuition in the following definition of hypergame and, then, define a hypergame on graph. 
\end{comment}



\begin{definition}[Hypergame on Graph]
\label{def:hypergame_graph}
Let $TS$ be a transition system, $\cal A$ be a specification automaton corresponding to P1's \ac{ltl} specification and $\cal I$ be an indicator set defined over the hypotheses  space $\cal X$. Then a hypergame on graph is a tuple

\[
    {\cal H} = \langle V, \vA, \Delta, {\cal F}, Acc_1,  \rangle
\]
where the components of hypergame on graph are as follows
\begin{itemize}
    \item $V = (\vS \times \vA)^{\ast}  \vS \times Q \times {\cal X}$. Every state $(h, q, x) \in V$ has three components: 
    \begin{itemize}
         \item $h \in (\vS \times \vA)^{\ast} \vS $ is an ordered sequence of state-action pairs terminating in the current state $\vs \in\vS$.
        \item $q \in Q$ is the automata state for keeping track of P1's progress towards satisfying $\varphi_1$. 
        
        \item $x \in \cal X$ represents the hypothesis of P2 in that state. 
    \end{itemize}
    
    \item $\vA$ is the set of joint  actions. 
    
    \item $\Delta: V \times \vA \rightarrow \dist(V)$ is a probabilistic transition function, defined as follows. Consider $v= (h\vs, q, x)$ and $v' = (h\vs \va\vs',q',x')$
     \begin{multline*}
         \Delta(v' |v, a)   =\\ P(s'|s,a)\mathbf{1}(\delta(q, L(s'))\equiv q') \mathbf{1}(\eta(x, h\vs \vs')\equiv x')
     \end{multline*}
    % \begin{itemize}
    %     \item $s' \in \supp(T(s, a))$, where $s \in S$ is the last state in the history $h$ and $s' \in S$ is the last state $h'$. 
    %     \todo[inline]{Note: Haoxiang's algorithm is a special case of this, where history is either carried forward or wiped out completely. }
        
    %     \item $q' \in \delta\big(q, L(s')\big)$, where $s' \in S$ is the last state in $h'$. 
        
    %     \item $x_{i'} = \eta(x_i, h')$ is the updated hypothesis. Here, $x_i \in \cal X$ denotes the hypothesis corresponding to indicator value $i \in \cal I$.
        
    %     \item $a_2 \in \pi_2(s, i)$, where $a_2 \in A_2$ is P2's  action and $\pi_2(s, i)$ denotes the strategy of P2 at a state $s \in S$ when P2's hypothesis is $x_i$.
    % \end{itemize}
    
    \item ${\cal F}$ is the set of final states for P1. The set ${\cal F}$ is defined as the set $(\vS \times \vA)^\ast \times\vS \times F \times {\cal X}$, where $F$ is the set of accepting states of the automaton $\cal A$. 
    
    \item $Acc \in \{ \text{Safety, Co-safety} \}$ is the acceptance condition for P1.
    
\end{itemize}
\end{definition}
%todo: remove the safety acceptance condition.

The transition function is understood as follows: Given a history $h_1=h\vs$ where $\vs$ is the current state and $h$ is the past history till $\vs$, a joint action $\va\in \vA$, the probability of reaching next state $\vs' $ is determined by $P(\vs'|\vs, \va)$ in the transition system. Upon reaching $s'$, P2 updates her hypothesis to $x' = \eta(x, h\vs \va \vs')$ (here we assume the entire history is used for this update). Also, the transition in the specification automaton is triggered to reach state $q' = \delta(q, L(\vs'))$ given the labeling of state $\vs'$. 

\begin{remark}
The definition of hypergame on a graph has infinite states, as a history can be of a finite but unbounded length. The entire history is maintained as part of the state due to the general definition of the inference mechanism. 
When P2 uses incremental inference, which  updates her hypothesis with a bounded length history and a previous hypothesis, the size of the state space becomes finite. Next, we discuss a class of subgoal inference algorithms and then revisit this hypergame on a graph. It is noted that only P1 can construct this hypergame on graph with his privileged knowledge in this level-2 hypergame. 
\end{remark}

% \begin{remark}
% Another consideration for deceptive planning is to limit the number of hypothesis updates of P2. With a frequent changing hypothesis, P2 may select more adverse co
% \end{remark}

% \todo[inline]{limit the number of switching. using switching game formulation.}

% \begin{definition}[Hypergame]
% Let $\game_1$ and $\game_2$ be the games on graph as constructed by P1 and P2 in their mind, given P1's objective is to satisfy $\varphi_1$ and P2's objective is to satisfy $\varphi_2$. Then, a \textit{first-level} hypergame is a tuple
% \[
%     {\cal H}^1 = \langle \game_1, \game_2 \rangle.
% \]

% When one player is aware of misperception and other is not, we get a \textit{second-level} hypergame, given by the tuple
% \[
%     {\cal H}^2 = \langle {\cal H}^1, \game_2 \rangle
% \]
% where P1 solves the first-level hypergame to compute his strategy. 
% \end{definition}


% We note that a \textit{second-level} hypergame models the game with information asymmetry described in Problem~\ref{}. We refer the reader to \cite{} for a general treatment of $k$-th level hypergame. 


% A definition of hypergame given in Def.~\ref{} does not account for evolving misperception. 




% % When P1 is aware of P2's misperception, P1 computes his strategy by anticipating the P2's strategy, given her perception $\psi_t$ of P1's objective. In order to anticipate P2's strategy, P1 must first construct a model of his opponent, P2. An opponent model consists of what P1 knows about (a) how P2 perceives P1's objective at $t=0$, (b) how P2 updates her misperception, \ie the inference mechanism of P2, and (c) given the misperception $\psi_t$, how does P2 compute her strategy.


==> Archived/sections/introduction.tex <==
%\textbf{State the problem: what are we trying to do in this paper?}

Planning in adversarial scenarios is commonly encountered in security and military applications. When the objective of a planning agent is partially unknown to its opponent, deception becomes inseparable from the optimal planning: With a proper deceptive mechanism, the opponent may take actions beneficial to the deceiver. This paper studies game-theoretic  deceptive planning with high-level mission specifications in a class of temporal logic formulas \cite{manna2012temporal}. 
In this class of  games, one player (Player 1/P1) is to achieve a task specified as a syntactically co-safe  temporal logic formula \cite{kupferman2001model}, while its opponent (Player 2/P2) is unaware of either the structure or parameters of the formula. Difference from payoffs in form of reward/cost, Boolean payoffs in
temporal logic allow one to  unambiguously  express high-level desired behaviors including safety (always staying in the safe region), reachability (eventually reaching the goal region), obligation (if event C occurs, return to the base), stability (eventually always staying in region A), and liveness (eventually visiting either region A or region C) \cite{manna2012temporal}. 

 In games with asymmetric information, deception is often used by a player to leverage its private information for tactical advantages against its opponent. 
 Scenarios of interests include economics \cite{gneezy2005deception},  military operations \cite{handel2005masters}, security in cybernetwork \cite{stech2016integrating,horak2017manipulating,Huang2018,Ahmadi2018ThePO}, and  robotics ,and other cyber-physical systems \cite{wagner2011acting,egorov2016target,Masters2017,gharesifard2012evolution,ornik2018deception}. Game-theoretic planning with deception has employed solution concepts of games with asymmetric information including dynamic Bayesian games \cite{Huang2018,zhang2019game} and hypergames \cite{house2010hypergame,ferguson2019game}. In dynamic Bayesian games, a player captures the incomplete information as a probability distribution over a set of the opponent's types.  The authors \cite{Huang2018} studied stealthy and deceptive behaviors and defensive planning in  cyber deception where the type of the opponent, \ie  a legitimate user or an attacker, is the private information. 
 A hypergame  \cite{wang1989solution,bennett1980hypergames} is characterized by players' misperception of the other players' payoffs or other components of the game (state/action space). In repeated normal-form hypergames, the authors  \cite{gharesifard2012evolution} studied how a player's belief of other players' preferences evolves by observing other players' decisions and analyzing inconsistency in the equilibrium.  They  developed stealthy deception \cite{gharesifard2014stealthy}
 to restrict the deceiver's actions so that the action set does not contradict
the belief of the mark. 

Other deceptive planning investigated games with imperfect information. In \cite{ahmadi2018partially}, the authors formulated cyber deception by assuming that the defender has full observability  and the attacker has partial observability. A deceptive strategy minimizes the expected cost of deception against all strategies of the attacker. 
%  Other deceptive planning that exploits bounded rationality of the opponent can be found in \cite{RewardBasedDeceptionCognitive}, where the authors formulated deceptive planning as  a resource allocation game, in which the defender assigns resources of a limited quantity to optimally defend against human adversaries with cognitive bias. 
Besides game-theoretic approaches,  
deceptive path-planning is developed in \cite{Masters2017} for deterministic systems. Deception aims to minimize the probability of an observer identifying its final destination before it has been reached. The idea is similar to that in \cite{ornik2018deception}, where the authors used multi-objective optimal planning for deception where one agent seeks to achieve an objective while confusing the opponent about the true intention by increasing the entropy in the planned policy.


 
In this work, we develop a novel theory of dynamic hypergame--a game of perceptual games with Boolean temporal logic objectives. Based on this hypergame formulation, we obtain a  deceptive strategy that maximizies the probability for the deceiver to satisfy its co-safe \ac{ltl} specification against a boundedly rational opponent. The deceptive planning algorithms include two modules: \emph{Opponent modeling} and \emph{Proactive deception}. In opponent modeling, the goal is to understand how the actions of the deceiver can influence the hypothesis of the mark about the intention of the deceiver, as well as predicting the counter-strategy of the mark given its hypothesis. 
Given the common knowledge that  a temporal logic formula describes a sequence of temporally extended goals, the mark tries to infer the changing subgoals of the deceiver and counteract correspondingly. 
We employ the cognitive hierarchy of game \cite{camerer2004cognitive} and the Theory of Mind \cite{premack1978does} to predict the evolution of the mark's perception  and to predict the  counter-strategy of the mark given actions of the deceiver. Then, we show that by incorporating the predicted behavior policy of the mark, the deceptive planning problem reduces to probabilistic planning in a \ac{mdp} with potentially an infinite state space. However, by restricting to a class of  subgoal inference and change detection algorithms \cite{banerjee2017quickest}, the planning problem can be solved in a finite-state \ac{mdp}.  An interesting observation is that when a temporal logic specification is considered, the subgoals, which are not pursued by the deceiver, become the decoys to distract the mark. 
Finally, we evaluate the performance of the proposed algorithm with experiments of robot motion planning  in adversarial environments.

==> Archived/sections/planning.tex <==
% \todo[inline]{
% \begin{itemize}
%     \item almost-sure winning region of the game with complete information. comparing with the almost sure winning region for P1 in the hypergame on graph. Hypothesis: almost-sure winning in the hypergame, taking into account of P2's perceived rational strategy, will be a superset (after projecting onto $S\times Q$) of the almost-sure winning region. showing one example. Use toy example.
%     @abhishek with very general statement : combining the subgraph of switched games. Appendix: algorithms.
% \end{itemize}
% 2. }

In this section, we provide a solution to Problem~\ref{problem_statement} for a class of hypergames on graphs in which P2 uses change detection algorithm to identify the time-varying subgoal of P1 and reasons iteratively using the \ac{ch} model of games to compute her counter-strategy. 
The solution includes two steps: In the first step, we construct this class of hypergame on graph with finite, discrete state space from Def.~\ref{def:hypergame_graph} given P2's inference mechanism. In the second step, we compute the deceptive strategy for P1. 

Let $\path^{\le m}$ be a set of histories with length $\le m$ that can be generated from the game transition system. Note that the length of a  history  is defined by the number of state-action pairs in that history. For example, the history $\vs_0\va_0\vs_1\va_1\ldots \vs_{ m-1}\va_{m-1}\vs_{m}$ is of length $m$. The length corresponds to the size of the sliding window in change detection algorithm.
\begin{definition}
 Assuming that P2 uses a change detection inference $\eta: \path^{\le m  } \times {\cal X}\rightarrow \cal X$ and P1's objective is given by a co-safe \ac{ltl} formula,  the  hypergame on  graph is computed as 
\[
{\cal H} = \langle V, \vA, \Delta , u_0, {\cal F},  Acc_1 \rangle 
\]
with the following components:
\begin{itemize}
    \item $V= \path^{\le m} \times Q\times \cal X$. Each state includes a finite history $\rho = \vs_0\va_0\vs_1\va_1\ldots \vs_\ell \va_\ell \vs_{\ell+1}$ where $\ell+1\le m$, an automaton state $q$ and the hypothesis $x$ of P2 in that state. 
    \item $\vA$ is the set of joint actions.
    \item $\Delta$ is the transition function, defined as follows. Given $v = (h\vs, q, x)$  with $h \in \path^{\le m-1} $. Given action $\va \in \vA$ and state $\vs' $ for which $P(\vs'|\vs, \va)>0$, 
      we distinguish two cases, depending on whether P2's hypothesis changes:
      \begin{itemize}
      \item If there is no change in hypothesis, that is,
        $\eta(x, h\vs\va \vs')= x$, then let
        $v' = (h \vs\va \vs' , \delta(q, L(\vs')), x)$ and
        $\Delta(v' |v, \va) =P(\vs'|\vs,\va)$.
      \item Otherwise, $\eta(x, h\vs\va \vs')= x'$ and $x'\ne x$. Then
        let $v'' = (\vs' , \delta(q, L(\vs')) , x')$ and
        $ \Delta(v' |v, \va) = P(\vs'|\vs,\va) $ \end{itemize} That
      is, when P2 detects a change, then the history is discarded due
      to the change detection algorithm.
         \item $u_0 \sim \dist(V)$ is the initial state distribution. Given the initial state $\vs_0$, if the initial hypothesis  $x_0$ is deterministic, the initial state distribution is $u_0(\vs_0, q, x_0)=1$ with $q= \delta(q_0, L(\vs_0))$. If the initial hypothesis is given by a probabilistic distribution $b_0\in \dist(\cal X)$, then the initial distribution is $u_0((\vs_0, q, x))=b_0(x)$ with $q = \delta(q_0, L(\vs_0))$.
    \item ${\cal F}$ is the set of final states for P1. The set ${\cal F}$ is defined as the set $\path^{\le m} \times F \times {\cal X}$, where $F$ is the set of accepting states of the automaton $\cal A$. 
    \item $Acc =  \text{ Co-safety} $ is the acceptance condition for P1.
\end{itemize}
\end{definition}



Intuitively, for player 1 to plan the best strategy, he needs to keep track of the history which is used by player 2 to update her hypothesis, P2's  hypothesis at the current state, the current game state, as well as the transition in the game arena given both player's actions.
Based on the \ac{ch} theory, by knowing the subgoal inferred by P2, P1 is able to compute P2's counter-strategy using iterative reasoning--that is, if P1 predicts that P2's current hypothesis is $x$, then P1 assumes that P2 will adapt the counter-strategy $\pi_2^{(k)}(x)$--the level-$k$ strategy in $\game(x)$. For simplicity in notation, as the level-$k$ is clear from the context,  we denote P2's strategy to be $\pi_2: S\times {\cal X}\rightarrow \dist(A)$  so that $\pi_2(s,x) = \pi_2^{(k)}(x)$, for all $(s,x) \in S\times {\cal X}$.

Finally, marginalizing out P2's strategy from the hypergame on graph, we obtain a Markov decision problem with co-safe objective. The optimal policy in this \ac{mdp} is \emph{proactive} and \emph{deceptive} because  P1 predicts how his future action can influence the perception of P2 and plans his action to steer P2's perception in a way advantageous to his own temporal logic objective.  The Markov decision problem with co-safe objective is defined by:
\[
{\cal H}^{\pi_2} = \langle   V, A_1, \Delta^{\pi_2}, {\cal F}, \text{co-safety} \rangle 
\]
with the transition function defined by marginalizing out P2's action given her strategy ${\pi_2}$:
\[
\Delta^{\pi_2}(v' |v,a_1) = \sum_{a_2 \in A_2} \Delta(v'|v,(a_1,a_2)){\pi_2}(v, a_2).
\]
and for any $v\in \cal F$ or $v=(hs,q,x)$ and
$s\models \neg \varphi_{safe}$, $\Delta^{\pi_2} (v\mid v,a_1)=1$. Note
that upon reaching $v\in \cal F$, the history satisfies P1's co-safe
LTL specification. Upon reaching $v\in \neg \varphi_{safe}$, the
history violates P1's invariant safety objective and thus the
specification.

From the result of probabilistic model checking \cite{Baier2008},
to maximize the probability of satisfying the co-safe LTL specification, P1 equivalently maximizes the probability of reaching the set of states in $\cal F$.
\[
\max_{\pi} \Expect\left(\sum_{t=0}^\infty \mathbf{1}(v_t \in \calF)\right)
\]
To solve the optimal policy, we compute the set of states, $V_{=1}$, from which there exists a policy $\pi_{=1}$ that ensures the set $\cal F$ can be reached with probability one. This set $V_{=1}$ can be computed using accepting end components for qualitative reasoning in \ac{mdp}s \cite{Baier2008} and has linear time complexity in the size (state and transitions) of the \ac{mdp}. Next, we solve the stochastic shortest path problem given the following reward function  $r: V\times A_1\rightarrow [0,1]$ defined by,
\begin{equation}
    \label{eq:reward}
r(v,a) =  \sum_{v'\in V} \Delta^{\pi_2}(v'|v,a) \mathbf{1}(v' \in V_{=1}).
\end{equation}
and the states in $V_{=1}$ are all made to be absorbing.
 
The optimal policy $\pi$ is obtained from solving the \ac{mdp} ${\cal H}^{\pi_2}$ with the total reward criteria:
\[
\max_{\pi}  \Expect\left(\sum_{t=0}^\infty r(v_t,a_t) \mid v_0 \sim u_0\right).
\]
The optimal planning problem with the total reward criteria can be found in \cite{Puterman1994}. Let $\pi^\ast$ be the solution of the total reward planning problem. The optimal deceptive policy $\pi$   can be obtained by sequentially composing the policy $\pi^\ast$ and $\pi_{=1}$ as follows.
\[
\pi(v)=\left\{
\begin{array}{c cc}
    \pi^\ast( v) & \text{ if } v \notin V_{=1} , \\
     \pi_{=1}(v)& \text{ otherwise}. 
\end{array}\right.
 \]
 where policy $\pi_{=1}$  ensures the set $\cal F$ can be reached with probability one.

In practice, due to the large state space of the problem, we employed an online \ac{mcts}~\cite{silver2010monte,browne2012survey} to solve the probabilistic planning problem in ${\cal H}^{\pi_2}$. In the online version of MCTS, since the specification can be complex, it is a rare event to sample a trajectory that satisfies the specification. In other words, the reward function defined by Eq.~\eqref{eq:reward}
 is too sparse for any online planners. To mitigate this problem, we define the subgoal reward signals for  P1 during online planning.  We define the  subgoal reward signals as follows.
 
 \begin{itemize}
     \item First, for each state $q\in Q$ of the \ac{dfa}, we define a function $\level: Q\rightarrow \nat$ so that 
  $\level(q)$ is   the minimal number of transitions it takes to reach a state in the accepting states $F$ of the \ac{dfa}.
  \item Second, for each state $q\in Q$,  we employ reactive synthesis for concurrent reachability game \cite{de2000concurrent} to solve the \emph{almost-sure winning region} for the following game: 
  $\game(\varphi(q)) =\varphi_{safe}\until \lor_{\sigma \in X} \Eventually \sigma$ and the set $X =\{\sigma\mid  q\xrightarrow{\sigma} q' \land \level(q')< \level(q).
 \}$ 
 \item Given each state $v=(h\vs ,q,x)$, let the current reward function to be 
\[ r(h\vs,q') = \alpha \text{ if } \vs \in \win^1(\game(\varphi(q))).\]
 \end{itemize}
 where $\alpha$ is a positive constant.

  %Further, we assign penalty $-100$ for states at which the safety property $\varphi_{safe}$ is violated. 
  
 This subgoal reward signal may produce sub-optimal policies as it
 does not use backward induction in dynamic programming to define the
 reward. We are currently investigate how to improve the online
 planner.
% we use the sure-winning regions for P1 to give an intermediate reward, which speeds up the convergence of the algorithm. Instead of giving a reward when the simulated trajectory satisfies the specification, we give an intermediate reward when the system makes progress, meaning it reaches a state within a subgoal of the specification. By doing that, the reward signal can be quickly backpropagated. This can guide the system to pick the best action for the current state efficiently. For more details of sure-winning regions computation, readers are referred to~\cite{de2000concurrent}.For more details, readers are referred to Algorithm~\ref{alg:mcts} in Appendix~\ref{sec:pseudo_code}. 

==> Archived/sections/preliminaries.tex <==
\textbf{Notation:} Let $\Sigma$ be a finite alphabet. A sequence of symbols $w=w_0 w_1 \ldots w_n  $ with $w_i\in \Sigma, i=0,1,\ldots, n$ is called a \emph{finite word} and $\Sigma^\ast$ is the set of all finite words that can be generated with alphabet $\Sigma$. We denote the set of all $\omega$-regular words by $\Sigma^\omega$ obtained by concatenating the elements in $\Sigma$ infinitely many times. 


Given a set $X$, let $\dist(X)$ be the set of all probability distributions over $X$. Given a distribution $\delta \in \dist (X)$, the set $\supp(\delta) = \{ x \in X \mid \delta(x) > 0\}$ is called the support of the distribution. When $\supp(\delta)$ is singleton, the distribution $\delta$ is called as Dirac delta function.

\subsection{Games on Graphs}

We consider an adversarial encounter between two players; a controllable player P1 (pronoun ``he") and an uncontrollable player P2 (pronoun ``she"), where both players choose their moves simultaneously. The dynamics of such an encounter can be captured as a concurrent game graph \cite{Baier2008}. 

{\definition[Concurrent game graph]A \emph{concurrent game graph} 
$
    TS = \langle \vS, \vA, P, AP, L \rangle,
$ consists of the following components:
\begin{itemize}
    \item $\vS$ is the set of joint states of P1 and P2.
    \item $\vA = A_1 \times A_2$ is a finite set of actions, where $A_1$ is the set of actions P1 can perform and $A_2$ is set of actions P2 can perform. 
    
    \item $P:  \vS\times \vA \rightarrow \dist(\vS)$ is a stochastic transition function. At every state $s \in \vS$, P1   chooses an action $a_1 \in A_1$, and simultaneously and concurrently P2  chooses an action $a_2 \in A_2$. Then, a successor state $s'$ is determined according to the probability distribution $P(s,\va)$, where $\va = (a_1, a_2)$. 
    
    \item $AP$ is a set of atomic propositions. 
    
    \item $L:  \vS\rightarrow 2^{AP}$ is a labeling function. For every state $s \in \vS$, the label of the state $L(s)$ represents a set of atomic propositions that are evaluated true in state $s$. 
\end{itemize} 
}

% \begin{remark}
% In an adversarial game, it is implicitly assumed that P2 knows P1's objective, $\varphi_1$, and P2 plays a counter-strategy to prevent P1 from satisfying $\varphi_1$.
% \end{remark}

The labeling functions are related to the objectives of players. We use \ac{ltl} to represent the players' objectives  in the game. \ac{ltl} provides a succinct way to represent temporally complex specifications such as safety, co-safety, persistence and recurrence or a logical combination of these. The syntax of LTL is given as follows, 
\[ 
    \varphi := \top \mid \bot \mid p \mid \varphi \mid \neg\varphi \mid \varphi_1 \land \varphi_2 \mid \bigcirc \varphi \mid \varphi_1 {\until} \varphi_2, 
\] 
where  $\top,\bot$ are universally true and false, respectively,  $p \in \calAP$ is an atomic proposition,  $\bigcirc$  is a temporal operator called the ``next'' operator. $\bigcirc \phi$ means that the formula $\phi$ will be true in the next state. $\until$ is a temporal operator called the ``until'' operator. $\phi_1\until \phi_2$ means that $\phi_2$ will be true in some future time step, and before that $\phi_1$ holds true for every time steps.

The operators $\Eventually$ (read as eventually) and $\Always$ (read as always) are defined using the operators $\until$ and $\bigcirc$ as follows: $\Eventually \varphi = \truev \until
\varphi$ and $\Always \varphi = \neg \Eventually \neg \varphi$. $\Eventually \phi$ means that $\phi$ will be true at some future time. $\Always \phi$ means that $\phi $ will hold every time step. For details about the syntax and semantics of \ac{ltl}, the readers are referred to \cite{Pnueli1989}. 

In this paper, we restrict the specifications of the players to the class of syntactically co-safe formulas \cite{??}. A syntactically co-safe \ac{ltl} formula  contains only $\Eventually$ and $\until$ temporal operators when
written in positive normal form (i.e., $\neg$ appears only in front
of atomic propositions) \cite{}. A co-safe \ac{ltl} formula $\phi$ has a set of \emph{good prefix} $L$. That is, given a good prefix $w\in L$, the word $ww' \models \phi$ for any $w'\in \Sigma^\omega$.

\begin{definition}{Task \ac{dfa}}
Given P1's objective expressed as a co-safe \ac{ltl} formula $\phi$, the  set of good prefixes of $\phi$ is accepted by a \ac{dfa}  $
    {\cal A} = \langle Q, \Sigma, \delta, q_0, F \rangle
$ with  the following components:
\begin{itemize}
    \item $Q$ is a finite set of states. 
    
    \item $\Sigma = 2^{AP}$ is a finite set of input words to the \ac{dfa}. 
    
    \item $\delta: Q \times \Sigma \rightarrow Q$ is a deterministic transition function. 
    
    \item $I \in Q$ is the unique initial state.
    
    \item $F \subseteq Q$ is a set of final states. 
    \end{itemize}
\end{definition}
A word $w\in \Sigma^\omega$ is accepted by the \ac{dfa} if and only if there exists $k$ such that $\delta (I, w[0,k] )\in F$ where $w[0,k]$ is the prefix of $w$ of length $k+1$.


During the interaction between two players, P1 aims to satisfy his objective in temporal logic, say $\varphi_1$, over the transition system. As the encounter is adversarial, P2's objective is to prevent P1 from satisfying his objective. Hence, P2's objective can symbolically be denoted by $\varphi_2 = \neg \varphi_1$. Next, we give formally the definition of game with Boolean payoffs expressed in temporal logic.

\begin{definition}[Games]
\label{def:games}
Let $\varphi_1$ denote the objective of P1. Then, given a transition system $TS$, a game on graph is a tuple
\[
    \game(\varphi_1, \neg \varphi_1) = \langle TS, \varphi_1, \neg \varphi_1 \rangle.
\]
\end{definition}

 For convenience, we omit P2's objective $\neg \varphi_1$ and simply denote a game by $\game(\varphi_1)$.

% \end{definition}

%  In a game, $\game(\varphi_1)$, each player computes a strategy to satisfy their objective. A finite-memory stochastic strategies defined as $\pi_j: ( \vS\times \vA)^\ast \times  \vS\rightarrow  \dist(A_j)$ where $j = 1, 2$. When games with different specifications are considered,  we may write strategy as $\pi_j(\varphi)$ to denote a strategy of player $j$ in game $\game(\varphi)$.

%  %%todo: include the result of winning region partitions about concurrent games.


% Next, we compose a transition system and an \ac{ltl} specification  to define a game on graph. Every \ac{ltl} specification can be translated to an equivalent automaton \cite{vardi1996automata}. We first define a \ac{dfa} that can represent any co-safe or safe \ac{ltl} formula.

 

% Given the definitions of transition system, \ac{ltl} specification and \ac{dfa}, we now define a game on graph.


% \begin{definition}[Game on Graph]
% Given a transition system $TS$ and \ac{dfa} ${\cal A}$ corresponding to the specifications $\varphi$ of P1, a stochastic concurrent game on graph between P1 and P2 is a tuple
% \[
%     \game = \langle  \vS\times Q, \vA, \Delta_G, {\cal F}, Acc \rangle
% \]
% where the components of a game are as follows
% \begin{itemize}
%     \item $\vS \times Q$ is the set of game states, where $\vS$ is the set of states in $TS$, and $Q$ is the set of states in ${\cal A}$. 
    
%     \item $\vA$ is the set of actions, same as the set of actions in the transition system $TS$.
    
%     \item $\Delta_G:  \vS\times Q \times \vA \rightarrow  \dist( \vS\times Q)$ is a probabilistic transition function. Consider two state $(s, q)$ and  $(s', q')$
%      \begin{align*}
%          \Delta_G((s', q') \mid (s, q), a) = P(s'|s,a) \mathbf{1}(\delta(q, L(s'))\equiv q')
%      \end{align*}
%      where $\mathbf{1}(b)$ is the indicator function, \ie, $\mathbf{1}(b)=1$ if the statement $b$ holds, and $\mathbf{1}(b)=0$ otherwise.
    
%     \item ${\cal F} =  \vS\times F$ is the set of final states for P1. 
    
%     \item $Acc \in \{\text{safety, co-safety}\}$ is the same acceptance condition as that of ${\cal A}$. 
    
% \end{itemize}
% \end{definition}


% In a game on graph with complete information and co-safety acceptance condition, P1 wins the game if no matter which strategy P2 uses, the game ends in one of the states $\cal F$. Otherwise, P2 wins.  If the acceptance condition is safety, then P1 wins the game if no matter which strategy P2 uses, the game stays in $\cal F$. Otherwise, P2 wins.

% P1 assumes, without considering any information about the opponent, that P2 is a \textit{perfect} adversary. This is, P1 assumes that P2 has complete information and complete observation, and her objective is $\varphi_2 = \neg \varphi_1$. This assumption makes P1's strategy in the game very conservative. One approach to weakening this assumption is by allowing information asymmetry, which we introduce in next subsection. 


\subsection{Problem formulation: Planning under Information Asymmetry}
In Def.~\ref{def:games}, the game is a common knowledge to both players. We now consider the case when the information between two players are asymmetrical and potentially incomplete. 
%Information asymmetry exists in an encounter when one player (say P2) has incomplete information about other player's (P1) objective, while the other player has the privileged information \cite{}. 
In the class of games, the asymmetric information between players is introduced as follows.
\begin{itemize}
    \item P1's objective is $\varphi_1 \coloneqq \varphi_{inv}\until \varphi $. $\varphi_{inv}$ is a state formula that specifies some invariant properties. 
    \item P2 knows $\varphi_{inv}$ and the concurrent game graph $TS$, but does not know $\varphi$.
    \item P2 knows that $\varphi_1$ is an \ac{ltl} co-safe formula. 
\end{itemize}


Suppose that, at the beginning of the encounter, P2 hypothesizes P1's objective to be an element $x_0$ from a finite set $\cal X$ of possible objectives. Then, being an adversary, P2 would play a strategy to prevent P1 from satisfying $x_0$. In other words, P2 will play a strategy $\pi_2(x_0)$ based on solution of the game $\game(x_0)$. We note that this strategy may not be optimal due to P2's misperception of P1's true objective. 

We equip P2 with a learning mechanism to update her hypothesis during the game; called as \textit{evolving perceptual game of P2}. That is, when P2 observes P1's behavior in the encounter, if P1's actions diverge from what P2 expects P1 to play based on her hypothesis, then P2 may update her hypothesis and thus evolve her perceptual game. We model this evolution using an inference mechanism defined as follows.


\begin{definition}[Inference Mechanism]
  Given the transition system $TS= \langle S, \vA, T, AP, L \rangle $
  that captures the interaction dynamics between two players.  Let a
  finite set $\cal X$ be P2's hypothesis space about P1's
  objective. Assuming perfect observations, P2's inference mechanism
  is a function
  $\eta: {\cal X} \times ( \vS\times \vA) ^\ast \rightarrow {\cal X}$
  that maps P2's current hypothesis $x \in {\cal X}$ and a finite
  history of state-action sequences $h \in ( \vS\times \vA)^\ast$ to a
  new hypothesis $x' \in {\cal X}$ of P1's objective.
\end{definition}


\begin{remark}
The above definition of inference mechanism assumes that these two players have complete observability in the encounter. When this is not the case, the history may be defined over the set of observations.
\end{remark}

We assume the following knowledge of P1.
\begin{assumption}
\label{assume:p1knowledge} Assume that P1 knows
\begin{enumerate}
    % \item P2 misperceives P1's objective $\varphi_1$ as an objective $x_0 \in \cal X$ at the beginning of the game.
    
    \item P2's initial hypothesis $x_0 \in \cal X$, and
    
    \item P2's inference mechanism $\eta$. 
\end{enumerate}
\end{assumption}
These assumptions can be realized in practice: For example, P2's initial hypothesis can be an objective of P1 in the past interactions. We will show later that even if P1 has incorrect  initial hypothesis of P2, with the knowledge of P2's inference, P1 can perform a sequence of actions to ensure the alignment between P2's current hypothesis and his belief of P2's current hypothesis.

%todo: respond to this statement in the paper.

Given the notion of P2's evolving perceptual game in an adversarial encounter of two players under information asymmetry, we formalize our problem statement. 


\begin{problem}
\label{problem_statement}
Given an adversarial encounter between P1 and P2 under information
asymmetry as defined by Assumptions~\ref{assume:p1knowledge}, compute
a strategy for P1 that maximizes the probability of satisfying
$\varphi_1$.
\end{problem}

==> Archived/subgame.tex <==


Given the hypergame on graph, we can define a sub-hypergame on graph. We define two functions: Function $\pred: V\rightarrow 2^V$   maps a state $v$ in the hypergame to a set of immediate predecessors of $v$, that is $\pred(v)= \{v' \mid \exists a\in A, \Delta(v \mid v',a) >0\}$. 
Function $\succ: V\rightarrow 2^V$ maps a state $v$ to a set of successors of $v$, that is, $\succ(v)= \{v' \mid \exists a\in A, \Delta(v' \mid v, a)>0\}$.

\begin{definition}[Sub-hypergame on a graph]
A \emph{sub-hypergame on a graph} of a dynamic hypergame on a graph $\cal H$ is a subset of hypergames on graphs that satisfy
\begin{itemize}
    \item There is a unique state $v^\ast$ in $\cal H$ such that $\pred(v^\ast) $ is not in the sub-hypergame.
    \item If a state $v$ in the sub-hypergame on graph, then any $v'\in \succ(v)$ is  also in the sub-hypergame.
\end{itemize}
\end{definition}
